Automatic Symmetry Discovery with Lie Algebra Convolutional Network

Existing equivariant neural networks require prior knowledge of the symmetry group and discretization for continuous groups. We propose to work with Lie algebras (infinitesimal generators) instead of Lie groups. Our model, the Lie algebra convolutional network (L-conv) can automatically discover symmetries and does not require discretization of the group. We show that L-conv can serve as a building block to construct any group equivariant feedforward architecture. Both CNNs and Graph Convolutional Networks can be expressed as L-conv with appropriate groups. We discover direct connections between L-conv and physics: (1) group invariant loss generalizes field theory (2) Euler-Lagrange equation measures the robustness, and (3) equivariance leads to conservation laws and Noether current.These connections open up new avenues for designing more general equivariant networks and applying them to important problems in physical sciences

==> secs2/outtakes.tex <==

\section{Outtakes}

\subsection{Tensor with $\vx_0^T g^{-1}$ formulation instead of $\vx_0 g^T$}

\paragraph{Group action}
\nd{Change to $\vx_\mu^T g^T$ for less confusion.}
Any subgroup $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group (invertible $d\times d$ matrices) acts on $\R^d$ and $\mathcal{F}$. 
Since $\vx_\mu \in \R^d$, $g \in G$ also naturally act on $\vx_\mu$. 
The resulting $\vy = g \vx_\mu $ is a linear combination $\vy = c^\nu \vx_\nu$ of elements of the discrete $\mathcal{S}$, not a single element.
The action of $G$ on $\vf$ and $\vx$, can be defined in multiple equivalent ways.
% The most elegant one is if w
We define $f(g \cdot \vx_\mu) = \vx_\mu^T g^{-1}\vf , \forall g\in G$.
% consistent with the lift. 
% This makes the group action on $\vf$ the natural action of $G$, meaning 
For $w\in G$ we have 
\begin{align}
    w\cdot f(\vx_\mu)&= f(w^{-1}\cdot \vx_\mu) = \vx_\mu^T[w^{-1} ]^{-1}\vf = \vx_\mu^T w \vf   
\end{align}
Dropping the position $\vx_\mu$, the transformed features are simply a matrix product $w\vf$. 


\paragraph{G-conv and L-conv in tensor notation} 
Writing G-conv \eqref{eq:G-conv} in the tensor notation we have 
\begin{align}
    [\kappa\star f](g\vx_0) = \int_G \kappa(v)f(gv\vx_0) dv = \vx_0^T \int_G v^{-1} g^{-1} \vf \kappa^T(v) dv \equiv \vx_0^T [\vf \star \kappa](g) 
    \label{eq:G-conv-tensor}
\end{align}
where we moved $\kappa^T(v) \in \R^m \otimes \R^{m'}$ to the right of $\vf$ because it acts as a matrix on the output index of $\vf$.
The equivariance of \eqref{eq:G-conv-tensor} is readily checked with $w\in G$
\begin{align}
    w\cdot [\vf \star \kappa](g) & = [\vf \star \kappa](w^{-1}g) 
    = \int_G v^{-1} [w^{-1}g]^{-1} \vf \kappa^T(v) dv 
    %= \int_G v^{-1} g^{-1} w\vf \kappa^T(v) dv 
    =  [w \vf \star \kappa](g)
\end{align}
where we used $[w^{-1}g]^{-1}\vf = g^{-1} w\vf $.
Similarly, we can rewrite L-conv \eqref{eq:L-conv-def0} in the tensor notation. 
Defining $v_\eps =I+ \ba{\eps}^i L_i $ 
\begin{align}
    Q[\vf](g) 
    &= W^0 f\pa{g\pa{I+ \ba{\eps}^i L_i}} 
    = \vx_0^T \pa{I+ \ba{\eps}^i L_i}^{-1} g^{-1} \vf W^{0T} \cr
    &= \vx_0^T \pa{I- \ba{\eps}^i L_i} g^{-1} \vf W^{0T} 
    % = \br{\vf_\mu + \ba{\eps}^i [L_i \vf]_\mu }W^{0T} 
    % \cr
    \label{eq:L-conv-tensor0}
\end{align}
The equivariance of L-conv in tensor notation is again evident from the $g^{-1} \vf$ part, resulting in $Q[w\vf](g) = Q[\vf](w^{-1}g) = w\cdot Q[\vf](g)$. 
Next, we will discuss how to implement \eqref{eq:L-conv-tensor0} in practice and how to learn symmetries with L-conv.
% means and how it impacts the learning of symmetries using L-conv. 
We will also discuss the relation between L-conv and other neural architectures. 



\subsection{Interpretation of L-conv}
To implement \eqref{eq:L-conv-tensor0} we need to specify the lift and the form of $L_i$. 
We will now discuss the mathematical details leading to and easy to implement form of \eqref{eq:L-conv-tensor0}. 
% $\hat{L}_i$. 

\out{
Recall that $L_i$ reside in the tangent space of the identity. 
Defining the lift via $\vx_\mu= g_\mu \vx_0$, the $d\times d$ matrices $L_i$ are only nonzero in the neighborhood of $\vx_0$. 
L-conv acts on other $\vx_\mu$ via the pushforward $L_i^{(g_\mu)}=g_\mu L_i g_\mu^{-1}$ appearing in $\vx_0^TL_i g_\mu^{-1}= \vx_\mu^T L_i^{(g_\mu)}$ (derived below). 
Thus, the set of $\vx_0^TL_i g_\mu^{-1}$ for all $\mu$, yielding the discrete analogue of the operator $\hat{L}_i$ in \eqref{eq:dfdg-general}, which is defined over the entire tangent bundle $T\mathcal{S}$ instead of only $T_{\vx_0}\mathcal{S}$. 
For example, for image rotation $\hat{L}_i$ is the infinitesimal generator of rotations of the full image, while $L_i$ is a local operator which rotates only the neighborhood of a chosen pixel $\vx_0$. 
When learning symmetries in the tensor notation we can learn the entire $\hat{L}_i$ at once.
We will now discuss the mathematical details leading to $\hat{L}_i$. 
}%%%%%
\out{
% Dropping $\vx_0^T$ we are left with a peculiar equation.
While the group action on $\vf$ is simply $w\vf$, 
% While the normal action of $v_\eps$ would be $v_\eps \vf$, we have a $g^{-1}$ (lift of the input) sitting in $v_\eps g^{-1} \vf$. 
% To realize the oddness, note that 
% unlike the simple linear action $w\vf$ for the features, 
the group action on L-conv is $w\cdot Q[\vf](g) = v_\eps g^{-1} w\vf W^{0T} $.
While $w\cdot Q$ is still a linear action, it is not a simple left matrix product. 
%which is not a simple linear action from the left like $w\vf$.
}%%%%%

\paragraph{Topology}
We introduced the discrete space $\mathcal{S}$ as a set of points. 
In many cases the space has a topology, e.g. when $\mathcal{S}$ are a discretization of a manifold $\mathcal{S}_0$, or vertices on a lattice or a general graph. 
% If the points in $\mathcal{S}$ is a graph, a lattice, or the discretization of a manifold $\mathcal{S}_0$, it has a topology. 
We encode this topology in an undirected graph (i.e. 1-simplex) with adjacency matrix $\mA$, defining the topological space $(\mathcal{S},\mA)$.
% We denote the adjacency matrix of this undirected graph by $\mA$, with 
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
\out{
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
% Thus, $\mathcal{S}$ together with the graph encoded in $\mA$ define a  topological space, which we denote as $(\mathcal{S},\mA)$.
$\mA$ can encode which pixels are adjacent in images, or crystalline structure, or the discretized space-time in physics. 
$\mA$ can be weighted (e.g. the pixel covariance), %matrix between pixels in an image dataset, 
but we use an unweighted $\mA$, with $\mA_{\mu\nu} \in \{0,1\}$.
% In physics, $\mA$ can encode crystalline structure, or the discretized topology of space-time. 
% The existence of a topology on $\mathcal{S}$ via $\mA$ 
% The topology restricts the lift by the group. % that act on the space.
}%%
Define the neighborhood of $\vx_\mu$ to be the set of normalized vectors
\nd{
Neighborhood should be defined using the incidence matrix $\mB$ to ensure the vectors are $\vx_\nu-\vx_\mu \in T_{\vx_\mu}\mathcal{S}$. 
We can do so by picking the set of edges $\{a|\mB_a^\mu =-1\}$.  
}

\begin{align}
    <\mu>=\left\{\vx = \sum_\nu \mA_{\mu\nu} c_\nu \vx_\nu\Bigg| c_\nu \in \R \mbox{ and }\|c\|^2=1 \right\}
    \label{eq:neigh}
\end{align}
For the sum over a neighborhood we write $ \sum_{\nu\in <\mu>} F_\nu \equiv \sum_\nu \mA_{\mu\nu} F_\nu $. 
% $<\mu> = \mathrm{span}\pa{ \{\vx_\nu | \mA_{\mu\nu} \ne 0 \} }$, the space of normalized vectors spanned by neighbors of $\mu$ in $(\mathcal{S},\mA)$. 
Figure \ref{fig:S0S} summarizes some of the aspects of the discretization as well as analogies between $G$, $\mathcal{S}_0$ and $\mathcal{S}$. 
Technically, the group $G_0$ acting on $\mathcal{S}_0$ and $G$ acting on $\mathcal{S}$ are different.
But we can find a group $G$ which closely approximates $G_0$ (see SI \ref{ap:approx}).
% For example, \citet{rao1999learning} used the Shannon-Whittaker Interpolation \citep{whitaker1915functions} to translate discrete 1D signals by arbitrary, continuous amounts as $f'_\mu = g(z)_\mu^\nu f_\nu $.
% Here $g(z)_\mu^\nu = {1\over d} \sum_{p=-d/2}^{d/2} \cos \pa{{2\pi p\over d}(z+\mu -\nu) } $ approximates the shift operator for continuous $z$.
% The $g(z)$ form a group because $g(w)g(z)=q(w+z)$, which is a representation for periodic 1D shifts. 
For instance, \citet{rao1999learning} used Shannon-Whittaker interpolation theorem \citep{whitaker1915functions} to define continuous 1D translation and 2D rotation groups on discrete data. 
We return to this when expressing CNN as L-conv in \ref{sec:approx}. 

\out{

\nd{
% The topology can be encoded using the incidence matrix $\mB: \mathcal{E}\to \mathcal{V}$, where $\mathcal{E}$ and $\mathcal{V}$ are the set of edges and vertices, respectively. 
% The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
In contrast, the adjacency matrix component $\mA_{\mu\nu}$ is the weights of the edge from vertex $\mu$ to vertex $\nu$. 
The incidence matrix defines a 1-simplex, capturing part of the topology. 
* discuss boundary operator $\ro$, Hodge Laplacian, MPNN.  
  }
\nd{developing}
\paragraph{Relation to the Laplace-Beltrami Operator}
$\hat{L}_i$ is nonzero where there is an edge in the graph. 
Instead of writing $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$ 
we may use the incidence matrix $\mB$ to encode this. 
Recall that for a graph with node set  $\mathcal{V}$ and edge set $\mathcal{E}$, the incidence matrix $\mB:\mathcal{V}\times  \mathcal{E}\to \{0,1,-1\}$ encodes which nodes $\mu$ are end points of which edge $a$.
$\mB_{\mu a}=1$ or $-1$ if edge $a$ starts or ends at node $\mu$, respectively, and $\mB_{\mu a}=0$ otherwise. 
For undirected graphs, each pair of connected nodes have one incoming and outgoing edge to each other.
The Laplacian $\mL = \mD-\mA$ becomes $\mL = \mB\mB^T$.
A weighted graph can be encoded using a diagonal weight matrix $\mW_{ab}$ for the edges, with the weighted Laplacian $\mL = \mB \mW\mB^T$. 
Since the Lie algebra basis $\hat{L}_i$ is weighting the edges, we can write $\hat{L}_i = l_i^a\mB_{\mu a} $
}%%%

\paragraph{Lift and group action}
Define the lift via $\vx_\mu = g_\mu \vx_0$. 
Since we chose $\vx_\mu$ to be the canonical basis (one-hot), $\vx_\nu^T\vx_\mu = \delta_\mu^\nu $. 
Thus we can pick $g_\mu$ such that $g_\mu^T= g_\mu^{-1}$, meaning orthogonal matrices.  
Let $(I+\eps L_i) \vx_0 \in <0> $. 
This means that we can write $L_i  \vx_0 = \sum_{\rho \in <0>} 
% \Gamma_{i 0 }^\rho 
[\hat{L}_i]_0^\rho \vx_\rho $ for a set of coefficients $[\hat{L}_i]_0^\rho \in \R$.
%$\Gamma_{i 0 }^\rho \in \R$. 
% for small $\eps \ll 1$. 
% The continuity of $G$ action means that 
We want the $G$-action to preserve the topology of $(\mathcal{S},\mA)$, meaning points which are close remain close after the $G$-action. 
The consequence is that $<\mu>$ can be reached from elements close enough to identity in $<0>$ using $g_\mu$. 
Thus, for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$, meaning for a set of coefficients $ [\hat{L}_i]_\mu^\nu \in \R$ 
%$ \Gamma_{i \mu }^\rho \in \R$ 
we have
\begin{align}
    % <0>\ni&&
    % (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho \in <0>} \Gamma_{i 0 }^\rho \vx_\rho \cr
    % <\mu>\ni&&
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\in <\mu>}  
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu\vx_\nu 
    %= g_\mu \pa{\vx_0+ \eps \sum_{\rho\in <0>} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}
    % \cr
    % &&
    % \Gamma_{i \mu }^\nu &= \sum_{\rho\in <0>} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho = [g_\mu]^\nu_\rho \Gamma_{i 0 }^\rho
\end{align}
Multiplying from the left by $\vx_\nu^T$ to obtain $\vx^T_\nu g_\mu L_i\vx_0 = [g_\mu L_i\vx_0]^\nu $ and  
inserting $I= \sum_\rho \vx_\rho \vx_\rho^T$ we have 
\begin{align}
    [g_\mu L_i\vx_0]^\nu &= 
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu 
    = \sum_{\rho} \vx_\nu^T g_\mu\vx_\rho \vx^T_\rho L_i \vx_0
    \cr & = \sum_{\rho\in <0>}  \vx_\nu^T g_\mu\vx_\rho [\hat{L}_i]_0^\rho
    = [g_\mu]^\nu_\rho [\hat{L}_i]_0^\rho
    \label{eq:hat-L-discrete}
\end{align}
Note that $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$
% $\Gamma_{i \mu }^\nu = \mA_{\mu\nu} \Gamma_{i \mu }^\nu$ 
is only nonzero when $\nu \in <\mu>$. 
This can be rewritten using the ``incidence matrix'' $\mB:\mathcal{S}\to \mathcal{E}$, where $\mathcal{E}$ is the set of edges of the graph \citep{schaub2020random}.
The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
$\hat{L}_i$ become weights for the edges $\alpha$ as 
\nd{ $<\mu>$ as defined above is not $T_{g_\mu}G$ because its vectors do not start from $\vx_\mu$.
We have $\vx_\nu-\vx_\mu \in T_{g_\mu}G$ for $\vx_\nu \in <\mu>$. Does $\hat{L}_i\vf$ have to subtract $\vf_\nu-\vf_\mu$? 
}

\out{
In \eqref{eq:L-conv} we used the vector field $\hat{L}_i$.
Vector fields and partial derivatives $\ro_\alpha$ can be defined on 1-simplexes using the ``incidence matrix'' $\mB:\mathcal{S}\to \mathcal{E}$, where $\mathcal{E}$ is the set of edges of the graph \citep{schaub2020random}.
The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
It yields the graph Laplacian via $\mB^T\mB = \mD-\mA$, where $\mD_{\mu\nu} = \delta_{\mu\nu}\sum_\rho \mA_{\rho\mu}$ is the degree matrix.
The vector field component $[\hat{L}_i]^\nu_\mu$ is putting a weight on the edge from $\mu$ to $\nu$ and can be written as 
$[\hat{L}_i]^\nu_\mu = \sum_{\alpha \in <\mu>} \mL_i^\alpha \mB^\nu_\alpha $

can naturally be written as a matrix product $[\hat{L}_i]^\mu = \mL_i^\alpha \mB_\alpha^\mu$
\nd{Since the Lie algebra basis $\hat{L}_i$ is weighting the edges, we can write $\hat{L}_i = l_i^a\mB_{\mu a} $}
}%
This $\hat{L}_i$ is the discrete $\mathcal{S}$ version of the vector field $\hat{L}_i(\vx) = [g L_i \vx_0]^\alpha \ro_\alpha $ in \eqref{eq:dfdg-general}.
In fact, on a graph $\ro_\alpha f(\vx_\mu)$ becomes $\sum_\nu c_\alpha^\nu  \mA_{\mu\nu}(\vf_\mu - \vf_\nu)$ and most of differential geometry can be defined as usual \citep{schaub2020random,lim2015hodge}. 
Thus, on discrete $\mathcal{S}$, the tangent spaces are $<\mu> = T_{\vx_\mu}\mathcal{S}$. 
In \eqref{eq:hat-L-discrete} $\hat{L}_i$ %which we will call the \textbf{global Lie algebra basis}
is a vector field over the discrete tangent bundle $T\mathcal{S}=\{<\mu>|\mu \in \{0,\dots d\}\}$. 
Taking the transpose of \eqref{eq:hat-L-discrete} and using $g_\mu^T = g_\mu^{-1}$, discussed above, and $[\hat{L}_i^T]^\mu_\nu = [\hat{L}_i]^\nu_\mu$, we can rewrite the $L_i$ term in \eqref{eq:L-conv-tensor0} as 
\begin{align}
    \vx_0^TL_i g_\mu^{-1}\vf &=  [\hat{L}_i]^\nu_\mu \vf_\nu
    \label{eq:}
\end{align}
Thus, L-conv in tensor notation can be written in a simple form as follows.



\paragraph{Lie Algebra Convolutional Layer}
% \begin{figure}
%     \centering
\begin{wrapfigure}{r}{.5\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, this action is analogous to a Graph Convolutional Network with $d$ nodes and $m_l$ features per node. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-30pt}
\end{wrapfigure}
% \end{figure}

In conclusion, the discrete space L-conv \eqref{eq:L-conv-tensor0} can be rewritten using the global Lie algebra basis $\hat{L}_i$
\begin{align}
    % \mbox{L-conv}:\  
    Q[\vf] &=   \pa{\vf + \hat{L}_i\vf \ba{\eps}^i} W^{0T} \cr 
    Q[\vf]_\mu^a &= \vf_\mu^b [W^{0T}]_b^a + 
    [\hat{L}_i]_\mu^\nu \vf_\nu^c \br{W^i}^a_c
    \label{eq:L-conv-tensor}
\end{align}
Where $W^i=W^0\ba{\eps}^i$, $W^0 \in \R^{m_{in}}\otimes \R^{m_{out}}$ and $\ba{\eps}^i \in \R^{m_{in}}\otimes \R^{m_{in}}$ are trainable weights. 
The $\hat{L}_i$ can be either inserted as inductive bias or they can be learned to discover symmetries. % we will be learning $\hat{L}_i$. 
% We will discuss learning symmetries
We derived L-conv from G-conv using kernels around identity. 


\paragraph{Nonlinear activation}
% Regarding nonlinear activation functions, as discussed in \nd{cite prior work}, it depends on whether they commute with the group action. 
% When $G$ is not a Lie group, many point-wise nonlinearities can preserve it. 
% As many nonlinear activation functions are not compatible with equivariance. 
% Note that, similar to discussion in
As noted in \cite{weiler20183d}, an arbitrary nonlinear activation $\sigma $ may not keep the architecture equivariant under $G$, but linear activation remains equivariant.

\nd{Vector field plots of $\hat{L}_i$ in experiments.
Apply orthogonality with $B_{ij} = 2k\Tr{l_il_j}-2\Tr{l_i}\Tr{l_j}=$ }


\out{
In particular, for a fixed $i$ and $\eps\ll 1$, we have 
\begin{align}
    \vx_i &= (I+\eps L_i) \vx_\mu = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu \in <\mu> \\
    [L_i]^\nu_\mu &= \vx_\nu^T L_i \vx_\mu = {1\over \eps }\pa{\vx_\nu^T\vx_i- \delta^\nu_\mu}= \mA_{\mu\nu}\Gamma_{i\mu}^\nu
    % \vx_\nu^T\vx_i &= \delta^\nu_\mu + \eps [L_i]^\nu_\mu = \delta^\nu_\mu + \eps \mA_{\mu\nu}[l_i]^\nu 
\end{align}
Next, we note that writing $g_\mu = P\exp[\int_\gamma dt^iL_i]$ we can use the Lie algebra $[L_i,L_j={c_{ij}}^kL_k$ to pass $L_i$ through

Let $(I+\eps L_i) \vx_0 \in <0> $ for small $\eps \ll 1$. 
The continuity of $G$ action means that for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$. 
Therefore
\begin{align}
    (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho \cr
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu = g_\mu \pa{\vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}\cr
    \mA_{\mu\nu} \Gamma_{i \mu }^\nu   \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho
\end{align}

This means that any small $v_\eps = I+\eps^iL_i \in T_IG$ must move points $\vx_\mu$ within their neighborhood, meaning for $v_\eps = I+\eps^iL_i \in G$ close to identity and $\vx_\mu \in \mathcal{S}$ we have
\begin{align}
    % \forall v_\eps &= I+\eps^iL_i \in G, \quad \forall\vx_\mu \in \mathcal{S},\quad 
    &\exists c\in \R^d, & v_\eps \vx_\mu &= \sum_\nu c^\nu \mA_{0\nu}\vx_\nu \in <\mu >. 
    \label{eq:G-neigh-preserve}
\end{align}
}%%%

% Next, we establish relations between L-conv and other commonly used architectures. 



\subsection{Old}
\begin{proposition}\thlabel{prop:multi-L-conv}
Any G-conv layer on a connected Lie group can be approximated by a multi-layer L-conv  on these groups to arbitrary accuracy. 
\end{proposition}
%
\begin{proof}
To show this we need to take two steps. 
First, we discretize the support of $g(u)$ in \eqref{eq:G-conv} to infinitesimally small sets $ G = \bigcup_k G_k$, each having support around an element $u_k \in G_k$. 
This allows us to write $(f*g)(h)\approx \sum_k\Delta \mu_k g(u_k) f(u_k^{-1}h)$, where $\Delta \mu_k = \int_{G_k} d\mu$.  
Next, we write each $u_k$ as a product. 
On connected groups for any $u_k\in G$, we can write $u_k=\prod_{\alpha=1}^l v_\alpha $ where $v_\alpha = \exp[t_\alpha \cdot L] \approx (I+t_\alpha \cdot L) $ are elements close to identity. 
Then, $f(uh)$ can be written as a composition $l$ G-conv layers, each with weights $g_\alpha(u) = \delta (u-v_\alpha)$ (defined using a faithful representation of $G$)
\begin{align}
    f(u_k^{-1}h) &=f\pa{\prod_\alpha v_\alpha h} = f\pa{ F_{l} \circ \cdots \circ F_{1}(h) }, \cr
    %\qquad 
    F_\alpha(h) &= \int_G d\mu(u) f_\alpha(u_\alpha h) g_\alpha(u) %\cr 
    % & = F\pa{ \prod_\alpha \int_G d\mu(u) f_\alpha(u_\alpha h) g_\alpha(u)} \cr
    % & = \cr
    % g(u) &= \int_G d\mu(v) g(v) \delta(v-u) \approx c\sum_{\{v_i\}} g(v_i) \delta (v_i-u) \label{eq:g-approx}.
    % (f*g)(h) &\approx c\sum_{\{v_\alpha\}} g(v_\alpha) f(v_\alpha^{-1} h) %\cr &
    % \approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{\pa{I+{1\over l}t_\alpha \cdot L}^l h} \cr
    % (f*g)(h) &\approx c\prod_{\{v_\alpha\}} g(v_\alpha) f(v_\alpha^{-1} h) %\cr &
    % \approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{\pa{I+{1\over l}t_\alpha \cdot L}^l h} \cr
    % &\approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{ F_{\alpha,l} \circ \cdots \circ F_{\alpha,1}(h) } 
\end{align}
\out{
% It's sufficient to show that $f(uh)$ can be expressed as L-conv for any $u$, as for each given $u$, the $g(u)$ are the weights. 
% , every group element can be approximated as $u_\alpha \approx (I+{1\over l}t \cdot L)^l$.
Pick a faithful representation for $G$ and express $g_{\alpha}(u)$ in it. 
We may write the kernels %$g(u) = \tilde{g}(t)$
$g_\alpha(u) = \delta (u-v_\alpha)$ 
as an integral over kernels with infinitesimal support around one $u_\alpha$.%, then approximate it as a sum over a set of discrete patches around a set of elements $\{v_\alpha\} $  on $G$ where $g$ has support 
The composition of two G-conv layers with linear $f_\alpha(h) = h$ yields 
\begin{align}
    f(u^{-1}h) &=f\pa{\prod_\alpha v_\alpha h} = f\pa{ F_{l} \circ \cdots \circ F_{1}(h) }  ,\qquad F_\alpha(h) = \int_G d\mu(u) f_\alpha(u_\alpha h) g_\alpha(u) \cr 
    % & = F\pa{ \prod_\alpha \int_G d\mu(u) f_\alpha(u_\alpha h) g_\alpha(u)} \cr
    % & = \cr
    % g(u) &= \int_G d\mu(v) g(v) \delta(v-u) \approx c\sum_{\{v_i\}} g(v_i) \delta (v_i-u) \label{eq:g-approx}.
    % (f*g)(h) &\approx c\sum_{\{v_\alpha\}} g(v_\alpha) f(v_\alpha^{-1} h) %\cr &
    % \approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{\pa{I+{1\over l}t_\alpha \cdot L}^l h} \cr
    (f*g)(h) &\approx c\prod_{\{v_\alpha\}} g(v_\alpha) f(v_\alpha^{-1} h) %\cr &
    \approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{\pa{I+{1\over l}t_\alpha \cdot L}^l h} \cr
    &\approx c\sum_{\{v_\alpha\}} g(v_\alpha) f\pa{ F_{\alpha,l} \circ \cdots \circ F_{\alpha,1}(h) } 
\end{align}
where each $F_{\alpha}$ can be converted to an L-conv layer with linear activation and weights $W = t_\alpha$ and $W^0=1$. 
}%%%%
Since $u_\alpha$ are near identity, each $F_{\alpha}$ can be converted to an L-conv layer with linear activation and weights $W = t_\alpha$ and $W^0=1$. 
Thus, the G-conv layer can be approximated as sum and composition of L-conv layers. 
Each $G_k$ can be considered one output channel for the multi-layer L-conv and $g(u_k)$ are weights of a final aggregation layer. 
%
% Increasing the size of the support set $\{v_\alpha\}$ improves the approximation. 
% But a more systematic estimation for $g(u)$ can be done if $g(u)$ is well approximated as a finite series using basis functions of irreducible representations of $G$, such as the spherical harmonics for $SO(3)$, which generalize the Fourier basis. 
% \ND{Make concrete}%%% 
\end{proof}

% \ND{1. G-conv from composition of L-conv}

% For instance to encode $SO(3)$, instead of discretizing the group and using many group element to cover rotations at different angles, we may simply use the three generators of $SO(3)$. 





\subsection{Symmetries of Linear Regression}
In the case of linear regression we can derive part of the symmetries explicitly, as shown next.
% For brevity, 
We absorb biases into the regression weights $\mA$ as the last row and append a row of $1$ to the input.

\begin{theorem}\thlabel{thm:lin-reg}
% \subsection{Linear Regression}
Consider a linear regression problem on inputs $\mX \in \R^{d\times n}$ and labels $\mY \in \R^{c\times n}$ like above.
We are looking for the linear function $\mY=\mA\mX$.
For this problem is equivariant under a group $G$, %and using the same group element $u$ in 
through two representations $u \in T_d(G)$ and $u_c \in T_c(G)$ acting on $\mX$ and $\mY$, respectively, it is sufficient for $u$ and $u_c$ to satisfy
\begin{align}
    u\mH u^T& = \mH& u_c\mY\mX^Tu^T& = \mY\mX^T. 
    \label{eq:uHu}
\end{align}
where $\mH \equiv {1\over n} \mX\mX^T $ is the covariance matrix of the input. 
\end{theorem}

\begin{proof}
The equivariance condition 
%\eqref{eq:equivariant-group_action}
\eqref{eq:equivariance-steerable}
becomes
\begin{align}
    % R \in G_C \subset GL(C,\R), &\qquad Q \in G_D \subset GL(D,\R)\\
    u_c \mY =& u_c \mA \mX =%= R Ax  
    \mA u \mX 
    & % \label{eq:gy} \\
    \Rightarrow \mA &= u_c \mA u^{-1} \label{eq:lin-reg-equiv0}
\end{align}
%
Assuming that the number of samples is much larger than dimension, $n \gg d$, %and unbiased data \ry{what does this mean?}, 
$\mX^T\mX$ will be full rank $d\times d$ and that its inverse exists. 
The solution to the linear regression $\mY=\mA\mX$ is given by $ \mA = \mY\mX^T(\mX\mX^T)^{-1}$. 
Using the definition of covariance $\mH$ above, the condition \eqref{eq:lin-reg-equiv0} becomes $\mA = u_c\mY\mX^Tu^T (u\mX\mX^T u^T)^{-1}$.
% \begin{align} 
%     \mH &\equiv {1\over n} \mX\mX^T, &
%     \mA & ={1\over n} u_c\mY\mX^Tu^T (u\mH u^T)^{-1} 
%     \label{eq:H,AQ}
% \end{align}
% Instead of the most general solutions to   \eqref{eq:lin-reg-equiv}, let us consider a subset of them which are 
Thus, a sufficient condition for  \eqref{eq:lin-reg-equiv0} to hold is  \eqref{eq:uHu}.
% \begin{align}
%     u\mH u^T& = \mH& u_c\mY\mX^Tu^T& = \mY\mX^T. 
%     \label{eq:uHu}
% \end{align}
\end{proof}
% covers a subset of solutions
% naturally separating %by \eqref{eq:H,AQ} 
% into a supervised and unsupervised part.

The first condition in \eqref{eq:uHu} is about the input features, stating that $u$  preserves the covariance $\mH$, while the second condition also involves labels, stating that $u_c$ and $u$ preserve the cross-correlation of input and labels $\mY\mX^T$.
Next, we show that the group satisfying \eqref{eq:uHu} is related to an orthogonal group. %, as we show below. 

\begin{corollary}
The subgroup of symmetries of linear regression satisfying $u\mH u^T = \mH$ in \eqref{eq:uHu} form an orthogonal group isomorphic to $SO(d)$, with a Lie algebra basis given by 
\begin{align}
    L_i &= \mH^{1/2} L'_i \mH^{-1/2} & L'_i \in so(d) \label{eq:so_H-HLH0}
\end{align}
\end{corollary}

\begin{proof}
multiplying $u\mH u^T = \mH$ by $\mH^{-1/2} $ from both sides, we see that $u'\equiv \mH^{-1/2} u \mH^{1/2} $ satisfies $u' {u'}^T = I$ meaning $u'\in SO(d)$. 
Expanding elements near the identity, we get $u\approx I + \eps \cdot L = \mH^{1/2} (I+ \eps' \cdot L') \mH^{-1/2}$.
Setting $\eps = \eps'$ proves \eqref{eq:so_H-HLH0}. (Details in Supp \ref{ap:lin-reg-algebra})
\end{proof}

% Lastly, we discuss our experimental results. 




% \paragraph{Pooling on L-conv} 
% Pooling operations, such maxpooling, generally yield a significant performance boost in CNN.  
% \cite{cohen2016group} showed a relation between pooling and coset of subgroups. 
% They also state that the strides in CNN pooling are like subsampling the group to a subgroup $H\subset G$, resulting in outputs which are equivariant only under $H$ and not the full $G$. 



% \ND{Training $L$ directly}






\subsection{Further discussion}

\paragraph{Topology}
If the space $\mathcal{S}$ is a grid or discretization of a Riemannian manifold, it has topology. 
We encode this topology in an undirected graph (i.e. 1-simplex) with adjacency matrix $\mA$, defining the topological space $(\mathcal{S},\mA)$.
% We denote the adjacency matrix of this undirected graph by $\mA$, with 
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
% Thus, $\mathcal{S}$ together with the graph encoded in $\mA$ define a  topological space, which we denote as $(\mathcal{S},\mA)$.
$\mA$ can encode which pixels are adjacent in images.  
$\mA$ can be weighted (e.g. the pixel covariance), %matrix between pixels in an image dataset, 
but we use an unweighted $\mA$, with $\mA_{\mu\nu} \in \{0,1\}$.
In physics, $\mA$ can encode crystalline structure, or the discretized topology of space-time. 
% The existence of a topology on $\mathcal{S}$ via $\mA$ 
The topology restricts the lift by the group. % that act on the space.
To preserve the topology of $(S,\mA)$, 
% the action of a group 
the $G$ action must be continuous, meaning preserve the structure of the neighborhoods. 
Denote the neighborhood of a point $\vx_\mu$ by $<\mu> = \{\vx_\nu | \mA_{\mu\nu} \ne 0 \}$. %the ordered set 
% \begin{align}
%     \mbox{neighborhood: } 
%     <\mu> = \{\vx_\nu | \mA_{\mu\nu} \ne 0 \}
% \end{align}
% The ordering is crucial when defining the group action. 
If $g\in G$ swaps two points $\vx_\mu \leftrightarrow \vx_\nu$, it must also swap neighborhoods  $<\mu> \leftrightarrow <\nu >$.
This imposes the constraint on the Lie algebra $L_i \in\mathfrak{g}$ of $G$. 
The components $[L_i]_\mu^\nu\ne 0$ only if $\mA_{\mu\nu}\ne 0$, which also means that $L_i\vx_\mu $ remains within $<\mu>$. 
Hence, $<\mu>$ approximates the tangent space $T_{\vx_\mu}\mathcal{S}_0$ of the continuous space $\mathcal{S}_0 \supset \mathcal{S}$. 
This is important when defining lifts, discussed below.




\out{
\nd{

Graph Attention Networks (GAT) \citep{velivckovic2017graph} also assign different weights to neighbors, but their ansatz for the weighting is different from ours. 
}%
}%%%
\out{
\nd{Discuss Rao's experiments and contrast with ours}

\nd{Add section about pooling and how on the coarse-grained space $\mathcal{S}_i$ a new group $G_i$ is acting, which may not approximate the original $G_0$ well. 
This may also indicate that at different scales different symmetries may exist and we can capture them with coarse-graining.
}
}%%%%%



\out{
The main difference between L-conv and GCN is that L-conv can assign a different weight to each neighbor of the same node. 
As mentioned earlier, this
is similar to GEM-CNN \citep{cohen2019gauge} with a fixed gauge set by $g_\mu $.
% Different weighting of neighbors 
This weighting is similar to Gauge Equivariant Mesh (GEM) CNN \citep{cohen2019gauge}. 
The main difference is that in GEM-CNN the basis of the tangent spaces $<\mu>=T_{\vx_\mu}\mathcal{S}$ are not fixed and are chosen by a gauge. 
In L-conv the lift $\vx_\mu = g_\mu\vx_0$ fixes the gauge, meaning it determines how the basis at $<0>$ maps to the basis at $<\mu>$. 
Changing how the discrete $(\mathcal{S},\mA)$ samples the underlying topological space $\mathcal{S}_0$ 
% is unchanged but the points sampled from it to create $\mathcal{S}$ are moved a bit, 
changes the lift $g_\mu$ and hence the gauge, similar to GEM-CNN. 
}%%%%%


==> secs2/related.tex <==
% The most familiar example of equivariance in ML is translation invariance of features in natural images. % where the same shape may appear in different parts of the image.
% Incorporating this symmetry in the design of artificial neural networks led to the invention of
% Translation symmetry is explicitly encoded in convolutional neural networks (CNN) \cite{lecun1998gradient}. % as we take fixed filters, covering a small area of the image and move them along the whole image. 
% This allows CNN to find patterns matching each filter regardless of where in the image they appear. 
% As results, many other symmetries such as discrete rotations in 2D \cite{veeling2018rotation, marcos2017rotation} and 3D \cite{cohen2018spherical,cohen2016group} as well as permutations \cite{zaheer2017deep} have been incorporated into the architecture of neural networks.
% In \cite{bloem2019probabilistic} the general method for incorporating group equivariance of a probability distribution into the architecture is discussed.
% It is also shown \cite{kondor2018generalization} that the group equivariant action of a neural network layer on an input can be expressed as a convolution defined in the group theoretic sense, which we elaborate below. 
% More generally, steerable CNN \cite{cohen2016steerable} introduce a general way in which group equivariant layers should behave. 

\paragraph{Equivariant Networks}
% Equivariant networks, built upon the principle of equivariance to symmetry transformations, is an emerging field in machine learning. 
% General principles for constructing group equivariant networks were introduced in \citet{cohen2016steerable}, \citet{kondor2018generalization}, and \citet{cohen2019general}.
% Many existing works on equivariant architectures focus on \textit{finite groups} such as permutations \cite{hartford2018deep,ravanbakhsh2017equivariance,zaheer2017deep}, $90$ degree rotations 
% \cite{cohen2018spherical} or dihedral groups $\mathrm{D}_N$ $E(2)$  \cite{weiler2019general}.  
For a continuous group, the number of group elements is infinite.  
To incorporate them into the architecture, existing approaches  either discretize the group \cite{weiler20183d,weiler2018learning,cohen2016group},
or use a truncated sum over irreps \cite{weiler2019general,weiler20183d} via spherical harmonics in \citet{worrall2017harmonic} or more general Clebsch-Gordon coefficients \citep{kondor2018clebsch}.
Another approach taken in \citet{finzi2020generalizing} approximates the integral over the Lie group by Monte Carlo sampling.
However, their approach is quite involved, % It requires ``lifting'' inputs from a vector to an element in the group and 
using the matrix logarithm and exponential to define a distance function used to obtain a sampling neighborhood for each point.
The logarithm needs to be implemented for each group. 
While for low-dimensional groups such as $SO(2)$ or $SO(3)$ there are closed forms, for higher dimensions numerical methods need to be used, further complicating the architecture. 
% approaching the idea of working in the Lie algebra. 
% They use a logarithm map to define the Lie algebra, which requires complex matrix exponential computation.\ry{need double check}
% However, 
% \citet{ravanbakhsh2020universal} Universal MLP: proves a universal approximation theorem for single hidden layer equivariant MLP for Abelian and finite groups.
% The difficulty of designing equivariant networks is the requirement of knowing the symmetry group. 
Our method bypasses the integral over the group manifold. 
We use the Lie algebra to build an equivariant architecture like a Taylor expansion from infinitesimal generators of the group. 
% Our work further complements this by learning the symmetries through optimization from data.
%
% Most of the work in the literature has focused on incorporating known symmetries into the architecture. 
% as well as a new way to build convolutional layers using generators of symmetries. 
% We want to design a more general group convolutional layer potentially capable of learning symmetries in data without imposing inductive biases. 
%
% In \cite{bloem2019probabilistic} the general method for incorporating group equivariance of a probability distribution into the architecture is discussed.
%
\paragraph{Symmetry Discovery}
In addition to simplifying the construction of equivariant architectures, our method can also learn the symmetry generators from data. 
Learning symmetries from data has been studied before, but mostly in restricted settings.
Examples include commutative Lie groups as in \citet{cohen2014learning}, 2D rotations and translations in 
\citet{rao1999learning}, \citet{sohl2010unsupervised} or permutations \citep{anselmi2019symmetry}. 
Perhaps the closest to our work, in spirit, is \citet{zhou2020meta} which uses meta-learning to automatically learn symmetries in the data. 
% \citet{zhou2020meta} is about defining a weight-sharing scheme to decompose the weights of a fully-connected layer and not group convolution as in our work. 
Yet their weight-sharing scheme and the encoding of the symmetry generators is very different from ours (see appendix \ref{ap:compare} for detailed discussion). 
% \ry{do we compare with them?} 
Also their use of Kronecker factorization to sparsify the symmetry matrix restricts the symmetries to be local and, thus, introduces bias.

% Assuming a discrete group $G=\{g_1,\dots, g_n\}$, they decompose the weights $W\in \R^{s\times s}$ of a fully-connected layer, acting on $\vx \in \R^s$ as $\mathrm{vec}(W) = U^Gv$ where $U^G\in \R^{s\times s}$ are the ``symmetry matrices'' and $v\in \R^s$ are the ``filter weights''. 
% Then they use meta-learning to learn $U^G$ and during the main training keep $U^G$ fixed and only learn $v$.
% We may compare MSR to our approach by setting $d=s$. 
% First, note that although the dimensionality of $U\in \R^{nd\times d}$ seems similar to our $L \in \R^{n\times d\times d}$, the $L_i$ are $n$ matrices of shape $d\times d$, whereas $U$ has shape $(nd) \times d$ with many more parameters than $L$. 
% Also, the weights of L-conv $W\in \R^{n\times m_l \times m_{l-1}}$, with $m_l$ being the number of channels, are generally much fewer than MSR filters $v\in \R^d$. 
% Finally, the way in which $Uv$ acts on data is different from L-conv, as the dimensions reveal.
% The prohibitively high dimensionality of $U$ requires MSR to adopt a sparse-coding scheme, mainly Kronecker decomposition.
% Though not necessary, we too choose to use a sparse format for $L_i$, finding that very low-rank $L_i$ often perform best. 
% A Kronecker decomposition may bias the structure of $U^G$ as it introduces a block structure into it.
In a concurrent work, \citep{benton2020learning} propose Augerino, a method to learn equivariance with neural networks. 
Augerino uses data augmentation to transform the input data, which means it is restricting the group to be a subgroup of the augmentation transformations. 
% Augerino learns which subset of the augmentations improved the prediction. 
% This is done by writing 
% The data augmentation is written as $g_\eps = \exp\pa{\sum_i \eps_i \theta_i L_i} $ (equation (9) in \cite{benton2020learning}), with randomly sampled $\eps_i\in [-1,1]$. 
% $\theta_i$ are trainable weights which determine which $L_i$ helped with the learning task. 
Furthermore, their generators are fixed generators of affine transformations in 2D (translations, rotations, scaling and shearing). 
In contrast, our approach is more general.  
We learn the generators directly without restricting them to be a known set of generators.  
Additionally, we do not use the exponential map or matrix logarithm, hence, our method is easy to implement.  
Lastly, Augerino uses sampling to effectively cover the space of group transformations. 
Since we work with the Lie algebra rather the group itself, we do not require sampling and only need to learn a basis for the Lie algebra, which generally a small number of Lie algebra elements.
% The main differences with our approach 
% , which mean they are assuming the group to be a subgroup of their augmentation transformations. 
% Specifically, they assume the group to be affine transformations and learn which sub-group of it is used in the dataset. 
% In eq. 9, the $G_i$ (equivalent to our $L_i$) are the generators of affine transformations and the state below eq. 9 the $G_1,...G_6$ are predefined translations, rotations, scaling and shearing.  
% In contrast, we are learning $L_i$ and do not restrict them to a known set of generators. 



==> secs2/scrap.tex <==
In practice, both the dataset as well as its implementation are discrete.
A feature map $f$ is generally implemented as an array, or tensor, $\f \in \mathcal{F}^d$ where the base space $\mathcal{S}$ is discretized into a set of neighborhoods $\tilde{\mathcal{S}}= \{B_1,\dots B_d \}$.
Here $B_\mu \subset \mathcal{S}$ and $\bigcup_\mu B_\mu = \mathcal{S} $.
For example, $\f$ can be a raster image with resolution $d$. 
The value of $\f$ at a pixel $\mu$ is the $\mu$th component $\f_\mu$ and is a local average of $f(x)$ over a kernel with support mostly on $B_\mu$ (e.g. a Gaussian filter). 
% \out{
% should be the average of $f(\vx)$ over all $\vx\in B_\mu$, meaning 
% \begin{align}
%     \f_\mu &=\frac{\int_{B_\mu} d\vx f(\vx) }{\int_{B_\mu} d\vx}
% \end{align}
% }
With $\mathcal{F}= K^m$ for field $K=\R$ ot $\C$, a group $\tilde{G} \subseteq \mathrm{GL}_d(K)$ naturally acts on $\f$. 
Note that $G$ acted on the space $\mathcal{S}$ and by \eqref{eq:f-G-action} on $f \in \mathcal{F}[\mathcal{S}]$, where $\mathcal{F}[\mathcal{S}]$ denotes the space of all function from $\mathcal{S}$ to $\mathcal{F}$.
Similarly, $\tilde{G}$ acts on $\f\in \mathcal{F}[\tilde{\mathcal{S}}]$ (isomorphic to $\mathcal{F}^d$). 
The groups $\tilde{G}$ and $G$ are not necessarily isomorphic. 
The discretization map taking $f$ to $\f$ may only approximately preserve $G$, e.g. aliasing error (jagged lines) in image rotations. 
Since we only observe symmetries through the discrete dataset, we implement equivariance under the group $\tilde{G}$ instead of $G$.
Note that $\tilde{G}$ is often a continuous Lie group (e.g. arbitrary image rotations). 
\nd{Discuss explicit example of discrete shifts being isomorphic to continuous shifts. 
For example in 1D consider the group $G = (S^1,+)$ on the unit interval mod 1. 
If we discretize the space to only two pixels, a shift by $r\in [0,1]$ can be represented as 
% matrix taking the vector $(1,0)\to(1-r,r)$, and $(0,1)\to(r,1-r)$
}

\paragraph{Discretized Lift}
We want to find the proper definition for the lift $\vx = g\vx_0$ on the discretized space.  
$g\in \tilde{G}$ acts on $\f$ via matrix multiplication from the left $g\f$. 
The discretization replaced the coordinates $\vx \in B_\mu \subset \mathcal{S}$ with neighborhoods $B_\mu$.
To understand the effect of $g\f$ on the coordinates, we will write the components $\f_\mu$ using a matrix product with row vectors.

First, note that $\f\in \mathcal{F}^d = K^d\otimes K^m$. 
Consider a vector $v\in K^d$.
We can define an inner product using dual vectors $u^*: K^d \to K$, meaning $u^* v \in K$.
Let $\{b^\mu\}$ be the $d$ canonical (one-hot) basis vectors for $K^d$.
Define the dual vectors $b_\mu^* = [b^\mu]^*$ such that $b_\mu^* b^\nu =\delta_\mu^\nu $. 
The $*$ denotes going to the dual space (i.e. from column vector $b^\mu$ to the conjugate row vector $b_\mu^*$).
The dual basis can be used to define a dual for each vector $v =\sum_\mu v_\mu b^\mu$ as $v^* = \sum_\mu v^{\mu*}b^*_\mu $. 
The norm of a vector becomes $\|v\| = v^* v = \sum_\mu v^{\mu*}v_\mu$. 
Note that $g\in \tilde{G}$ acts on $v\in K^d$ as $gv$ the same way it acts on $\f$. 
We can define the dual space such that $\tilde{G}$ preserves this norm.
This means that if $u = gv$, we want $\|u\|=\|v\|$. 
Thus for all $g\in \tilde{G}$ and $v\in K^d$, if $u=gv$ we have
\begin{align}
    &\|u\| = [gv]^* gv = v^* v = v^* g^{-1} gv \cr
    &\Rightarrow [gv]^* = v^* g^{-1}.
\end{align}

Using the dual basis we have $\f_\mu %= \f(b_\mu^*) 
= b_\mu^* \f$. 
Hence, $b_\mu^*$ yields the value of $\f$ on the neighborhood $B_\mu$. 
The discretized version of $f(\vx)$ is $b_\mu^* \f$ when $\vx \in B_\mu$. 
The group action $g\cdot f(\vx) = f(g^{-1}\vx)$ in \eqref{eq:f-G-action}, with $g\in G$, becomes $b^*_\mu \tilde{g} \f = [g^{-1}b^\mu]^* \f$, with $\tilde{g}\in \tilde{G}$. 
Thus, the $\tilde{G}$ action on $\f$ by left multiplication is a consistent discrete version of \eqref{eq:f-G-action}.  

% Denote the set of functions $f:\mathcal{S}\to \mathcal{F}$ by $\mathcal{F}[\mathcal{S}]$ and $\f:\tilde{\mathcal{S}}\to \mathcal{F}$ by $\mathcal{F}[\tilde{\mathcal{S}}]$. 
Note that the discretization map $\mathrm{dis}:\mathcal{F}[\mathcal{S}]\to \mathcal{F}[\tilde{\mathcal{S}}]$ is not exactly equivariant, because it introduces estimation error. 
% \nd{Find bounds on group action error}
Recall that we assumed $\mathcal{F} \sim K^m$ over a number field $K$. 
While $\mathcal{S}$ is a discrete space, a continuous subgroup $\tilde{G} \subseteq \mathrm{GL}_d(K)$ acts on $\f\in \mathcal{F}[\tilde{\mathcal{S}}]$. 
In particular, similar to the lift where for any $\vx = g\vx_0$, we can pick a basis vector $b_0 \in K^d$ as the origin.
For any $\mu$ there exists $\tilde{g}_\mu\in \tilde{G}$ s.t. $b_\mu = \tilde{g}_\mu b_0$. 
\nd{We're actually always working with $\tilde{G}$ in practice. So, we don't even need to worry about the aliasing error.
We can simply say we only need to consider $\tilde{G}$ and call it $G$. 
}
The group $\tilde{G}$ may not be isomorphic to $G$ because of the discretization error, but with increasing resolution as $d\to \infty $, any $G$ can be estimated well with a $\tilde{G}$. 
Since in practice we only have access to the discretized data $\f$, the observed symmetries can only be a subgroup of $\mathrm{GL}_d(K)$.
Hence, we assume $G=\tilde{G}$. 



With $\mathcal{F}=K^m$, we have $\f\in K^{d\times m}$ \nd{I think the $K^{d\times m}$ notation is unambiguous, as a convention in ML. It's less cumbersome than $(K^m)^d$ or $K^d \otimes K^m$}.
A group which naturally acts on $\f$ is any subgroup $\tilde{G} \subseteq \mathrm{GL}_d(K)$. 
The group $\tilde{G}$ is not necessarily isomorphic to $G$, which acted on $\mathcal{F}[\mathcal{S}]$
which acts on $\f$, the discretized version of $f$. 
the vectors $b_\mu^*$ are simply one-hot row vectors with components $[b_\mu^*]_i = \delta_{i\mu}$. 
The group that 
\begin{align}
    \vb_\mu &= g \vb_0 & 
    \vb^*_\mu &= \vb^*_0 g^{-1} \cr
    \f_\mu &= \vb^*_\mu \f =  \vb^*_0 g^{-1}\f & &
\end{align}


\begin{align}
    [w\cdot \f]_\mu &= [w^{-1} g \vb_0]^* \f = \vb_0^*[w^{-1} g]^{-1} \f = \vb_0^*g^{-1} w \f = \vb_\mu^* w \f \cr 
    \Rightarrow & w\cdot \f = w \f 
    \label{eq:vec-group-action}
    % \\
    % [w\cdot h]_\mu & = b_\mu^T [w\cdot h] = b_\mu^T \pi[w^{-1}]^{T}h \cr
    % & = b_0^T \pi[g]^T \pi[w^{-1}]^{T}h \cr
    % & = b_0^T \pi[w^{-1} g]^T h = f(w^{-1} g) 
\end{align}



The lift from $\vb_\mu$ to $g$ means simply dropping the $\vb_0^*$ on the left.  
We use \eqref{eq:vec-group-action} to rewrite \eqref{eq:gconv-corrected} in terms of $\f$. 
The group convolution \eqref{eq:gconv-corrected} becomes
\begin{align}
    [\f \star \kappa](g\vb_0) &= \vb_0^*\int v^{-1} \f \kappa(g^{-1}v) dv %\cr & 
    = \vb_0^*\int [gv]^{-1}\f \kappa(v) dv 
    \label{eq:h-gconv-corrected} \cr
    &= \vb_0^* \int v^{-1} g^{-1}\f \kappa(v) dv 
\end{align}
The equivariance of $\kappa \star h$ \eqref{eq:h-gconv-corrected} can be checked readily using \eqref{eq:h-group-action}
\begin{align}
    [ w\cdot \f\star\kappa](g) 
    %&= \int \pi[v]^T h \kappa(g^{-1}v) dv \cr 
    &= \int v^{-1}g^{-1} w \f \kappa(v) dv \cr
    &= \int v^{-1}[w^{-1}g]^{-1} \f \kappa(v) dv \cr
    &= [\f\star\kappa ](w^{-1} g) \cr
    & = w\cdot  [\f\star\kappa](g)
    % \label{eq:kh-equiv}
    \label{eq:h-gconv-equiv}
\end{align}



\paragraph{Lift}
In order for $G$ to lift $\mathcal{S}$, meaning map $\vx_0$ to any other $\vx_\mu$, it must contain the permutation group $S_d$ (e.g. the orthogonal group $G=O(d)$ with $g^Tg=gg^T = I$ contains $S_d$).
We have $\vx_\mu =g_\mu \vx_0$ for $g_\mu \in S_d \subset G$.
Note that $G\subseteq \mathrm{GL}_d(\R)$ induces a $d$ dimensional matrix representation on $S_d \subset G$ such that $g_\mu^T = g_\mu^{-1} $ and $\vx_\mu^T \vx_\mu = \vx_0^T\vx_0 = 1$ and $\vx_\mu^T \vx_\nu = \delta_{\mu\nu}$.
As for the action of the full $G$ on $\vf$ and $\vx$, there are multiple equivalent definitions. 
The most elegant one is if we define $f(g \cdot \vx_\mu) = \vx_\mu^T g^{-1}\vf , \forall g\in G$, consistent with the lift. 
This makes the group action on $\vf$ the natural action of $G$, meaning for $w\in G$ 
\begin{align}
    w\cdot f(\vx_\mu)&= f(w^{-1}\cdot \vx_\mu) = \vx_\mu^T[w^{-1} ]^{-1}\vf = \vx_\mu^T w \vf   
\end{align}
We can also drop the position $\vx_\mu$ and the transformed features simply become a matrix product $w\vf$. 




in the previous formulation, we had the gradient $df(g)/dg$ and the pushforward $gL$. 
In the tensor notation, the pushforward from the origin to $g_\mu$ is already encoded in the $\mu$th row and column of $L$.
$Lg_\mu^{-1}$ is equal to $L$ outside the $2\times 2$ block of $(0,\mu)$. 
Within this block we have 
\begin{align}
    (0,\mu)\mbox{ block: }
    L g_\mu^{-1}\vf& = \mat{L_{00}&L_{0\mu}\\
    L_{\mu0}&L_{\mu\mu}} 
    \mat{0&1\\1&0} 
    \mat{\vf_0\\ \vf_\mu} \cr
    &= \mat{L_{0\mu}&L_{00}\\
    L_{\mu\mu}&L_{\mu0}}
    \mat{\vf_0\\ \vf_\mu} 
    = \mat{L_{0\mu}\vf_0+L_{00}\vf_\mu \\ L_{\mu\mu}\vf_0+L_{\mu0}\vf_\mu
    }
\end{align}
\begin{align}
    (0,\mu,\nu)\mbox{ block: }
    L g_\mu^{-1}\vf& = \mat{L_{00}&L_{0\mu}&L_{0\nu}\\
    L_{\mu0}&L_{\mu\mu}&L_{\mu\nu}\\
    L_{\nu0}&L_{\nu\mu}&L_{\nu\nu}} 
    \mat{0&1&0\\1&0&0\\0&0&1} 
    \mat{\vf_0\\ \vf_\mu\\ \vf_\nu} \cr
    &= \mat{L_{0\mu}&L_{00}&L_{0\nu}\\
    L_{\mu\mu}&L_{\mu0}&L_{\mu\nu}\\
    L_{\nu\mu}&L_{\nu0}&L_{\nu\nu}}
    \mat{\vf_0\\ \vf_\mu\\ \vf_\nu}
    = \mat{L_{0\mu}\vf_0+L_{00}\vf_\mu +L_{0\nu}\vf_\nu \\ L_{\mu\mu}\vf_0+L_{\mu0}\vf_\mu + L_{\mu\nu}\vf_\nu \\
    L_{\nu\mu}\vf_0+L_{\nu0}\vf_\mu + L_{\nu\nu}\vf_\nu 
    }
\end{align}
If we choose the $0$ index to be a dummy index, where $L_{0\mu}=L_{00}=\vf_0=0$, we are left with $Lg_\mu^{-1} \vf = (0,L_{\mu}^\nu f_\nu, \dots L_\nu^\rho f_\rho)$. 
If we now pull out th $\mu$ index to see by how much $\vf_\mu$ is changing, we get $L_\mu^\nu \vf_\nu$. 
But why should we pick index $\mu$? 


Note that $g_\mu = I+s_{\mu0}$ where $s_{\mu0}$ is only nonzero in the $(\mu,0)$ with values 
$\begin{pmatrix}-1&1\\1&-1 \end{pmatrix}$ in that block. 
We can move $g_\mu = g_\mu^{-1} $ past $L$ doing 
\begin{align}
    L_i g_\mu^{-1} &= g_\mu L_i 
    + [L_i,g_\mu ] = g_\mu L_i + [L_i, s_{\mu0}]
\end{align}

\nd{TODO: Explicitly show why $\vx_0^TLg_\mu^{-1}\vf = [Lf]_\mu $}

We want to pull $g_\mu$ through $L$ in $Lg_\mu^{-1}\vf = g_\mu g_\mu Lg_\mu^{-1}\vf$ so that we can read the index $\mu$ of the output. 
Hence, we need to calculate $g_\mu Lg_\mu^{-1}$. 
If $L_i$ is a ``local'' operator, meaning that when the space is a grid, only neighboring grid sites appear in $L_i$, we can represent $L_i$ as a graph over the grid with different weights for each neighbor.
Thus, we are assuming $[L_i]_\mu^\nu$ is nonzero only when $\nu \in <\mu>$, where $<\mu>$ denotes the neighbors of node $\mu$. 
In a 1D grid, the first neighbors would be $<\mu>= \{\mu +1, \mu-1\}$. 
We may also include second neighbors, etc. 
This has an important effect on $g_\mu L_i g_\mu^{-1}$. 
First, recall $g_\mu^{-1} = g_\mu^T = g_\mu$, as they are single permutations of $\vx_0$ to $\vx_\mu$. 
Define the switch operator $s_{\mu\nu}$ as the operator that switches $\mu\leftrightarrow \nu$ and removes their diagonal entries, meaning
\begin{align}
    [s_{\mu\nu }]_a^b & = 
    -\delta_{\mu a}\delta_\mu^b -  \delta_{\nu a}\delta_\nu^b + \delta_{\mu a}\delta_\nu^b +  \delta_{\nu a}\delta_\mu^b \\
    g_\mu &= g_\mu^{-1} = I + s_{\mu0}  \label{eq:g-mu-switch} 
\end{align}
We may insert an identity operator written as $I={1\over d}\sum_\nu g_\nu^{-1}g_\nu $ into \eqref{eq:L-conv-tensor0} to obtain
\begin{align}
    \vx_0^T  L_i g_\mu^{-1} \vf &={1\over d} \sum_\nu \vx_0^T g_\nu^{-1}g_\nu L_i g_\mu^{-1} \vf \cr
    g_\nu L_i g_\mu^{-1} &= (I+s_{\nu0})L_i(I+s_{\mu0}) 
    = L_i + s_{\nu0}L_i + L_i s_{\mu0} +  s_{\nu0}L_i s_{\mu0} \label{eq:L-sLs}
\end{align}
Since $s_{\mu0}$ is zero outside the $2\times2$ block of indices $(0,\mu)$, the terms above can be written as sums over neighbors of $\mu$
\begin{align}
    L_is_{\mu0} &= -L_{00} - \sum_{\nu \in <\mu>} L_i  
\end{align}
What's the most compact way to write this? We know $g_\mu$ only switches $(0,\mu)$ and the rest remains unchanged. 
So $Lg_\mu$ is $L$ for indices outside of $0,\mu$. 
But what is at $0,\mu$? 
Since we have $[\vx_0]_a = \delta_{0,a}$ multiplied from the left, we have  
\begin{align}
    \vx_0^T L g_\mu \vf &=  \delta_0^\rho L^\nu_\rho [g_\mu]^\lambda_\nu \vf_\lambda 
    = L^\nu_0 [g_\mu]^\lambda_\nu \vf_\lambda = \sum_{\nu\in <0>} L^\nu 
\end{align}
\begin{align}
    [Lg_\mu^{-1}]_0^\nu &= \sum_{a} L^\nu_a [g_\mu]^a_0 =\sum_{a} L^\nu_a \delta^a_\mu = L^\nu_\mu
\end{align}

Also what happens when it mapped to $g_\nu$?




\nd{Add to tensor notation}


In the tensor notation $gL \ro_g f = \vb_0^* Lg^{-1}\vf$. 
So $Lg^{-1}= g^{-1} [gLg^{-1}] = g^{-1}L_g$ is the pushforward of $L$ to $T_gG$. 
% To be precise, $Lg^{-1} = g^{-1} [gLg^{-1}] = g^{-1}L_g$. 
We can construct one operator $\hat{L}=\{L_g\}$ containing the set of $L_g\in T_gG$, with $g^{-1}\hat{L} = Lg^{-1}$. 
This way $\hat{L}$ acts on the whole tangent bundle $TG$ and $Lg^{-1}\vf = g^{-1}\hat{L}\vf = [\hat{L}\vf]_g $. 
\out{
So $f(g) = \vb_0^*\vf_g = \vb_0^* g^{-1} \vf $. 
\begin{align}
    [\vf \star \kappa]_g &= [\vf \kappa]_g = %\vb_0^* 
    \pa{g^{-1}+ \eps Lg^{-1}}\vf \kappa\cr &= %\vb_0^* 
    g^{-1} \pa{I+ \eps \hat{L}}\vf \kappa=[(I+\hat{L}) \vf\kappa]_g \cr
    [w\cdot\vf \star \kappa]_g &= %\vb_0^* 
    \pa{g^{-1}+ \eps Lg^{-1}} w\vf \kappa\cr &= %\vb_0^* 
    g^{-1} \pa{I+ \eps \hat{L}}\vf \kappa=[(I+\hat{L}) \vf\kappa]_g 
\end{align}
}

\paragraph{Tensor Notation}
In the fiber bundle formulation,  an $m\times n$ pixel images with $c$ channels was a map $f:\Z_m\times \Z_n\to \R^c$, where $\Z_m = \{1,\dots, m\}$. 
% where the group acts on the base space and the the features are fibers attached to each point. 
The tensor version of the data is $h\in \mathrm{Hom}(\R^{mn},\R^c)$, where the rows are flattened image coordinates and columns are the color channels.
In general, we will be switching from representing the features as $f:\mathcal{S}\to \mathcal{F}$ to tensors $h\in \mathrm{Hom}(\mathbb{R}[\mathcal{S}],\mathcal{F})$. 
The equivariance condition \eqref{eq:equivariance-steerable} becomes 
\begin{align}
    %u\cdot h &= \pi[u]h\rho[u^{-1}]^T, 
    u\cdot h &= \pi[u]^{-1}h\rho[u]^T, 
    \quad \forall u \in G 
    \label{eq:equiv-tensor}
\end{align}
where $\pi$ acts on the $p=mn$ dimensional spatial index and $\rho$ on the channels. 
Again, we will not consider the steerable case and assume $\rho[u]=I$.
Similarly, the group convolution becomes 
\begin{align}
    % \kappa \star h &= \int_G \pi[v]^{-1}h \kappa(v)^T d\mu(v)
    \kappa \star h &= \int_G \pi[v]^{-1}h %\rho[v]^T
    \kappa(v)^T d\mu(v)
\end{align}
where $\kappa(v)$ is moved to the right because they act on the output dimension of $h$. 
and \eqref{eq:G-conv-expand} becomes
\begin{align}
    % (\kappa \star f)(\vx) & 
    % \approx \int_G %{|\eps| <\eta }  
    % \tilde{\kappa}(\eps) f\pa{(I-\eps^i L_i) \vx} d \eps \cr&
    % \approx %\pa{\ba{\eps}_0 I - \ba{\eps}\cdot L }
    \kappa \star h & \approx h {W^0}^T  - \sum_i L_ih {W^i}^T 
    \label{eq:G-conv-expand-tensor}
\end{align}
We will refer to the input dimension of $h$, on which $G$ acts nontrivially, as the spatial dimension. 




\section{For Appendix} 
Explicit example of translation $\tilde{G}$ being isomorphic to $G$


Now we want the linear action of $w\in G$ on $h$ to reproduce $w\cdot f(x) = f(w^{-1}x)$.
Recall, $h$ is a $d\times c$ matrix. 
To obtain row $h_\mu = f(x)$ we can act on $h$ from the left by a one-hot vector $b_\mu \in \R^d$ as $b_\mu^T h = h_\mu$. 
A representation $\pi: H \to \mathrm{GL}_d(\R)$ acts on $b_\mu$ such that $b_\mu = \pi[g_\mu] b_0$. 
One way to get $w\cdot f(x) = f(w^{-1}x)$ is to have $w\cdot h = \pi[w^{-1}]^{T}h$ because 
\begin{align}
    w\cdot h &= \pi[w^{-1}]^{T}h 
    \label{eq:h-group-action}
    \\
    [w\cdot h]_\mu & = b_\mu^T [w\cdot h] = b_\mu^T \pi[w^{-1}]^{T}h \cr
    & = b_0^T \pi[g]^T \pi[w^{-1}]^{T}h \cr
    & = b_0^T \pi[w^{-1} g]^T h = f(w^{-1} g) 
\end{align}
We use \eqref{eq:h-group-action} to rewrite \eqref{eq:gconv-corrected} in terms of $h$. 
First, note that with the lift we do not need the vector $b_0$ and we can directly work with $g_\mu$, meaning 
$f(g) = \pi[g]^T h $. 
The group convolution \eqref{eq:gconv-corrected} becomes
\begin{align}
    [\kappa\star h](g) &= \int \pi[v]^T h \kappa(g^{-1}v) dv \cr &= \int \pi[v]^T\pi[g]^T h \kappa(v) dv 
    \label{eq:h-gconv-corrected}
\end{align}
Note that $\kappa(v)$ is a $c\times c'$ matrix acting on the output index of the $d\times c$ matrix $h$, hence $\kappa$ was appears to the right. 
\nd{We should also write $\kappa\star f$ this way.}
The equivariance of $\kappa \star h$ \eqref{eq:h-gconv-corrected} can be checked readily using \eqref{eq:h-group-action}
\begin{align}
    [\kappa\star w\cdot h](g) 
    %&= \int \pi[v]^T h \kappa(g^{-1}v) dv \cr 
    &= \int \pi[v]^T\pi[g]^T \pi[w^{-1}]^T h \kappa(v) dv \cr
    &= \int \pi[v]^T\pi[w^{-1}g]^T h \kappa(v) dv \cr
    &= [\kappa\star h](w^{-1} g) \cr
    & = w\cdot  [\kappa\star h](g)
    % \label{eq:kh-equiv}
    \label{eq:h-gconv-equiv}
\end{align}
One might ask why $w\cdot h $ acts with the inverse $\pi[w^{-1}]^T h$. 
Indeed, there exists a dual way to define all the above as $w\cdot h = \pi_1[w] h$. 
But to satisfy $w\cdot f(g) = f(w^{-1}g)$ we need to define the lifted vector $b_\mu$ slightly differently as $b_\mu = \pi_1[g_\mu^{-1}]^Tb_0$. 
We can verify that 
\begin{align}
    [w\cdot h]_\mu &= b_\mu^T w\cdot h = b_0^T \pi_1[g_\mu^{-1}] \pi_1[w] h \cr
    & = b_0^T \pi_1[\pa{w^{-1}g_\mu}^{-1}] h \cr
    & = f(w^{-1}g_\mu)
\end{align}
This choice does not yield any different results and is related to the first choice \eqref{eq:h-group-action} by setting $\pi_1[g] = \pi[g^{-1}]^T$. 
In particular, the order in which $w$ and $g$ appear in \eqref{eq:h-gconv-equiv} does not change.
This will be important in L-conv. 






For another group, such as $SO(2)$, the lift will be different
\footnote{Note that the manifold of $SO(2)$ is the circle $S^1$ and the group is isomorphic to periodic 1D translations. 
What is different here is just how the each group acts on the space. 
}
Let the grid be $2n\times 2n$, so that $d=4n^2$ and the origin be at the center node $(n,n)$ with index $\mu=n^2 $ in the discrete $\mathcal{S}$. 
A $G \simeq SO(2)$ can act on circles in this space, and a group $G\simeq \R \otimes SO(2) $ acts on the full space. 
Consider the $SO(2)$ art acting on nodes on at radius $r<n$ units around the origin $(n,n)$. 
An index $\mu$ can be converted to $(x,y)$ using $x=\floor{(\mu-n^2) /(2n)}$ and $x=(\mu-n^2) \mathrm{mod}(2n)$.
The points on this circle satisfy $r^2 \leq x^2+y^2 > (r-1)^2$. 
The lift should then be rotations of points on this circle such that an origin vector $(x_0,y_0) = (r,0)$ is rotated to the $x,y$ of node $\mu$. 
But this lift must also rotate all other points on the circle by the same angle. 
This $g_\mu $ is more difficult to write as an expression like \eqref{eq:gmu-circ-comp}, but it can be specified algorithmically. 


\paragraph{Induced metric}
In \eqref{eq:dfdg-general} $U_i^\alpha = [gL_i\vx_0]^\alpha $ defines a coordinate transformation from a
local basis $\ro_\alpha $ on $T_\vx\mathcal{S}$ to a basis induced by the Lie algebra basis $L_i$. 
Indeed, if $\mathcal{S}$ is endowed with Riemannian metric $\mathbf{g}(\vx):T_\vx \mathcal{S} \times T_\vx \mathcal{S} \to \R $, the lift by $G$ induces a new metric 
$\eta (g):T_gG\times T_gG\to \R$ with components 
$\eta_{ij} = [U^T\mathbf{g}U]_{ij} = U_i^\alpha U_j^\beta \mathbf{g}_{\alpha\beta}$. 
The inverse of this induced metric can be used to define group invariant loss functions. 





\Eqref{eq:G-neigh-preserve} defines a map from $T_IG$ to $<\mu>$. 
Since the lift $\vx_\mu =g_\mu\vx_0 $ maps the tangent spaces $T_{g_\mu} G$ to $T_{\vx_\mu}\mathcal{S}$, the neighborhood is the discrete version of the tangent space $<\mu>=T_{\vx_\mu}\mathcal{S}$.
In fact, partial derivatives $\ro_\alpha \in T_{\vx_\mu}\mathcal{S}$, which form a basis for tangent spaces, get mapped to $ A_{\mu\nu}(\vx_\mu-\vx_\nu)$ and a discrete version of differential geometry applies to $(\mathcal{S},\mA)$ \citep{schaub2020random,lim2015hodge}.
% Let $G$ be a Lie group which acts on $\R^d$ and hence on $\vx_\mu $
% To preserve the topology of $(S,\mA)$, 
% % the action of a group 
% the $G$ action must % be continuous, meaning 
% keep points in $<\mu>$ close to each other. 

In particular, we want the lift $\vx_\mu= g_\mu \vx_0$ to be such that the neighborhood $<\mu>= T_{\vx_\mu}\mathcal{S}$ is a pushforward of $<0>$, meaning
\begin{align}
    % \mbox{if }\vx_\mu &= g_\mu \vx_0, &
    \forall \vx_\nu &\in <\mu >: \quad g_\mu^{-1} \vx_\nu \in <0>
    \label{eq:lift-neigh}
\end{align}
% \begin{align}
%     \mbox{neighborhood: } 
%     <\mu> = \{\vx_\nu | \mA_{\mu\nu} \ne 0 \}
% \end{align}
% The ordering is crucial when defining the group action. 
% If $g\in G$ swaps two points $\vx_\mu \leftrightarrow \vx_\nu$, it must also swap neighborhoods  $<\mu> \leftrightarrow <\nu >$.
This imposes the constraint on the Lie algebra $L_i \in\mathfrak{g}$ of $G$. 
The components $[L_i]_\mu^\nu\ne 0$ only if $\mA_{\mu\nu}\ne 0$. 
Similarly, the pushforward $g_\mu L_i\vx_0 $ should remain within $<\mu>$. 
Hence, $<\mu>$ approximates the tangent space $T_{\vx_\mu}\mathcal{S}_0$ of the continuous space $\mathcal{S}_0 \supset \mathcal{S}$. 
% We clarify this approximation next. 
% This is important when defining lifts, discussed below.


\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figs2/L-conv-3-spaces.pdf}
    \caption{
    \textbf{Lie group and Lie algebra:}
    Illustration of the group manifold of a Lie group $G$ (left).  
    The Lie algebra $\mathfrak{g}=T_IG$ is the tangent space at identity $I$. 
    $L_i$ are a basis for $T_IG$.
    If $G$ is connected, any element $g$ can be written as a path-ordered integral $g=P\exp[\int_\gamma dt^i L_i]$. 
    The tangent space $T_gG$ has a basis $gL_i$, the pushforward by $g$.  
    \textbf{
    Schematic of the effect of coarsening}
    The original base space is  $\mathcal{S}_0$ and $G_0$ is its symmetry group. 
    The coarsening (discretization) produces a space $\mathcal{S}$.  The Lie group $G$ acts on $\mathcal{S}$ and closely approximates $G_0$ ($G\simeq G_0$, e.g. image rotations approximating real rotations).
    The lift takes $\vx\in \mathcal{S}_0$ to $g\in G_0$, and maps the tangent spaces $T_\vx \mathcal{S}_0\to T_gG_0$. 
    Each Lie algebra basis $L_{0i}\in \mathfrak{g}_0=T_IG_0$ generates vector field on the tangent bundle $TG_0$ via the pushforward as $L^{(g)} = gL_{0i}g^{-1}$.
    Due to the lift, each $L_i$ also generates a vector field $\hat{L}_i^\alpha(\vx)\ro_\alpha = [gL_i\vx_0]^\alpha \ro_\alpha$, with $\vx=g\vx_0$ 
    % Since $\mathcal{S}_0$ is lifted to $G$, $L_{0i}$ also generate a flow on $\mathcal{S}_0$, captured by the vector field $\hat{L}_i^\alpha(\vx)\ro_\alpha$. 
    Similarly, the Lie algebra basis $L_i$ of $G\simeq G_0$ generates a flow on $TG$ and a vector field $[\hat{L}_i]_\mu= g_\mu L_i\vx_0$ on $T\mathcal{S}$, with $\vx_\mu=g_\mu\vx_0$. 
    Note that tangent spaces on $\mathcal{S}$ are $T_{\vx_\mu}\mathcal{S}=<\mu>$, the neighborhoods of each $\vx_\mu$, and vector fields are weighted graphs, modifying neighbor weights in the graph $\mA$ encoding the topology of $\mathcal{S}$.
    % tensors flowing from every $\vx_\mu$ within the neighborhood $<\mu>$. 
    Note that depicting $\mathcal{S}$ and $\mathcal{S}_0$ as 2D is only for convenience. 
    They may have any dimensions. 
    }
    \label{fig:4-spaces}
\end{figure}
% \nd{Figure for discretization and tangent bundle}






\paragraph{Lift ...}

% We require the lift $\vx_\mu = g_\mu \vx_0$ to preserve the topology $(\mathcal{S},\mA)$.
% Concretely this means that the map $\mathrm{Lift}:\mathcal{S}\to G$ with $\mathrm{Lift}(\vx_\mu) = g_\mu$ must satisfy 
% \begin{align}
%     \forall \vx_\nu \in <\mu>: \quad
%     \mathrm{Lift}(\vx_\mu) \vx_0 \in <\mu> 
% \end{align}
% , it is important to note that $g_\mu \in G$ restricts the form of $g_\mu$. 
% For instance, 
To see this, we write \eqref{eq:lift-neigh} explicitly with indices. 
Let $\nu \in <0>$ and $\eta \in <\mu>$. 
We have
\begin{align}
    [g_\mu]^\rho_\sigma [\vx_\nu]^\sigma &= \Gamma^\eta_{\mu\nu} [\vx_\eta]^\rho &
    \Gamma_\mu &\in \R^n \otimes \R^n \quad
    (n = |<0>|)
    \label{eq:gauge}
\end{align}
% using a linear map $\Gamma_\mu \in \R^n \otimes \R^n $
The collection of $\Gamma_\mu$ for all $\mu$ is called a ``gauge'', or ``connection'' in differential geometry. 
It relates the basis of $<0>$ to the basis of $<\mu>$. 
The freedom is picking the gauge (i.e. in defining $g_\mu$) can be seen in the fact that $S^{\nu'}_\nu\Gamma^{\eta'}_{\mu \nu'}R^\eta_{\eta'} $ still satisfies \eqref{eq:lift-neigh} for any invertible $S,R$ with $\nu'\in <0>$ and
$\eta'\in<\mu>$. 
% as we show next. % on the tangent bundle $T\mathcal{S}$. 
Gauges have been used in Gauge Equivariant Mesh (GEM) CNN \citet{cohen2019gauge} (see \citet{bronstein2021geometric} for a review). 
Similar to gauges in GEM-CNN, $\Gamma_\mu$ is weighting the neighbors of each node and $\Gamma^\eta_{\mu\nu} = \Gamma^\eta_{\mu\nu} \mA_{0\nu}\mA_{\mu \eta}$ because $\nu\in <0>$ and $\eta \in <\mu>$.
% The continuous version, called gauge fields, is 
Gauge fields are also extensively used in physics
\citep{polyakov2018gauge}, though
% The set of lifts $g_\mu $ also define the pushforward $g_\mu L_i$.
the gauge definition in \eqref{eq:gauge} looks different because it is defined on a discretized space.
We will now use \eqref{eq:gauge} to define the procedure to implement L-conv. 

\paragraph{Gauge and the pushforward}
The freedom in defining the lift does not change the symmetry group that L-conv encodes. 
When $\mathcal{S}$ is a discretization of a continuous manifold $\mathcal{S}_0$, we want the group $G$ acting on $\mathcal{S}$ to approximate a group $G_0$ which acts on $\mathcal{S}_0$.
We will make this notion of approximation $G\simeq G_0$ more precise below. 
Let $G_0$ act transitively, so that $\forall \vx_\mu \in \mathcal{S} \subset \mathcal{S}_0 $, $\exists g_{0\mu}\in G_0$ s.t. $\vx_\nu = g_{0\mu} \vx_\mu$.
% the infinitesimal $G_0$ action on all neighborhoods is a pushforward of the Lie algebra from $T_IG_0 \sim $. 
% Thus, instead of the $d\times d$ basis $L_i$, there exist small matrices $l_i$ with $n\ll d$ which are shared among $<\mu>$ for all $\mu$.
% This is easy to understand 
% If before discretization $\mathcal{S}$ was the group manifold of a group $G_0 \simeq G$. 
Denote the Lie algebra basis of $G_0$ by $L_{0i}\in \mathfrak{g}_0$, which form a basis for $ T_{\vx_0} \mathcal{S}_0\sim T_IG_0 = \mathfrak{g}_0$. 
% at its identity which is isomorphic to the tangent space $ T_{\vx_0} \mathcal{S}$ at the origin $\vx_0$. 
% Pushing $L_{0i}$ forward as $g L_{0i}$ yields a basis for $T_gG_0$.
Let $G\simeq G_0$ be a group acting on $\R^d$ and use it to lift $\vx_\mu = g_\mu \vx_0$. 
Here $g_\mu \in G$ approximates $g_{0\mu}\in G_0$. 
% Since $G_0$ acts transitively on $\mathcal{S}_0 \supset \mathcal{S} $, for every $\vx_\mu \in \mathcal{S}$, $\exists g_\mu \in G$ s.t. $\vx_\mu = g_\mu \vx_0$ 
% (i.e. $\mathcal{S}$ can be lifted to $G$). 
We want to relate $L_i \in \mathfrak{g}$, the Lie algebra of $G$, to  $L_{0i}\in \mathfrak{g}_0$, the Lie algebra of $G_0$. 
Since $\vx_0$ is lifted to the identity, $L_i\vx_0$ approximates the action $L_{0i}\vx_0$. 
Therefore, $L_i\vx_0$ must remain in $<0>$. 
Hence, we have $L_i \vx_0 = \sum_{\nu \in <0>} [l_i]^\nu \vx_\nu  $, where $l_i$ is a vector approximating the action $L_{0i}\vx_0$. 
Using the condition \eqref{eq:lift-neigh} that the lift maps neighborhoods, the pushforward to $T_{g_\mu}G$ becomes 
% This means that there exist a set of vectors $l_i$ defined on $<0> \sim  T_I G_0$ which approximate the $L_{0i}\in \mathfrak{g}_0= T_I G_0$. 
\begin{align}
    % L_i \vx_0& = \sum_{\nu \in <0>} [l_i]^\nu \vx_\nu  
    % \label{eq:A0-li} \\ 
    [g_\mu L_i \vx_0]^\rho & = \sum_{\nu \in <0>} [l_i]^\nu %g_\mu \vx_\nu 
    [g_\mu]^\rho_\sigma [\vx_\nu]^\sigma =
    \sum_{\nu \in <0>} \sum_{\eta \in <\mu>} \Gamma^\eta_{\mu\nu} [l_i]^\nu [\vx_\eta]^\rho
    =  \sum_{\eta \in <\mu>} [\hat{L}_i]_\mu^\eta [\vx_{\eta}]^\rho
    \label{eq:gauge-li}
    % =  \sum_{\mu+\nu \in <\mu>} [l'_i]^\nu \vx_{\mu+\nu} 
\end{align}
% \nd{Using the condition on the lift that it preserves neighborhoods. }
where $[\hat{L}_i]_\mu^\eta = [\Gamma_{\mu} l_i]^\eta $ approximates the pushforward $g_{0\mu} L_{0i} \in T_{g_{0\mu}}G_0 \sim  T_{\vx_\mu}\mathcal{S}_0$.
In fact $\hat{L}_i$ is a collection of bases for all tangent spaces in the tangent bundle $TS$, approximating $TS_0$. 
So, unlike $L_i$ which was nonzero only on $<0>$, $\hat{L}_i$ contains the Lie algebra basis pushed forward to all $<\mu>$. 
Therefore, we will refer to $\hat{L}_i$ as the \textbf{bundle Lie algebra} basis, as it defines a basis for the entire the tangent bundle $T\mathcal{S}$. 
\nd{
Note that, unlike the gauge $\Gamma_\mu$, the $\hat{L}_i$ do not have a gauge freedom. 
Can we prove this?
}
%
%
\out{
Since all $T_g G_0$ are isomorphic and $l_i$ approximates $L_{0i}$, the $l'_i$ for each $\mu$ can be written as 
% For each $\mu$ we have different  $l'_i$ vectors, which can be written in terms of the original $l_i$ encoding $L_{0i}$ 
\begin{align}
    l'_i &=\Gamma_{\mu i}^j l_j, &
    \Gamma_\mu &\in \R^n \otimes \R^n,& 
    n &= |\mathfrak{g}_0 |
\end{align}
% using a linear map $\Gamma_\mu \in \R^n \otimes \R^n $
The collection of $\Gamma_\mu$ for all $\mu$ is called a ``gauge'', or ``connection'' in differential geometry. 
\nd{Talk about 
\begin{itemize}
    % \item how each lift defines a gauge
    \item parallel transport.
    % \item Rao's examples of groups approximating shift and $SO(2)$ 
\end{itemize}
}
}%%%%

Since $\vx_\mu^T\vx_\mu =1 = \vx_0^Tg_\mu^T g_\mu \vx_0$, we have $g_\mu^T = g_\mu^{-1}$. 
Therefore, the transpose of  \eqref{eq:gauge-li} can be used to
rewrite the $L_i$ term in \eqref{eq:L-conv-tensor0} as 
\begin{align}
    \vx_0^TL_i g_\mu^{-1}\vf &= 
    \Gamma^\eta_{\mu\nu} [l_i]^\nu [\vx_\eta]^\rho \vf_\rho = \Gamma^\eta_{\mu\nu} [l_i]^\nu \vf_\eta \equiv [\hat{L}_i]^\eta_\mu \vf_\eta
    \label{eq:}
\end{align}
where we used $[\vx_\eta]^\rho = \delta^\rho_\eta $ from their definition in sec. \ref{sec:tensor}.

If we know the topology, i.e. $\mA$, 
we need to use the ansatz in \eqref{}
we can use the form $[\hat{L}_i]_\mu^\eta = [\Gamma_{\mu} l_i]^\eta $, similar to GEM-CNN. 
When the topology is unknown, we can learn $\hat{L}_i$ as general, possibly low-rank matrices. 
% we redefined $W^{0T}\to W^{0}$ to drop the transpose, for brevity. 
Note that, since $\Gamma_{\mu\nu}^\eta =\Gamma_{\mu\nu}^\eta \mA_{\mu\nu}$ (i.e. only nonzero if $\eta \in <\mu>$, from \eqref{eq:gauge-li} we also have $[\hat{L}_i]^\eta_\mu =[\hat{L}_i]^\eta_\mu \mA_{\mu\eta} $.
So just like GEM-CNN, $\hat{L}_i$ is weighting the neighbors on the graph $\mA$.




\out{
% The lift must move adjacent points together.
% A lift preserving can be achieved using circulant matrices
\begin{align}
    % \mbox{for 1D Translation}&&
    g_\mu & = \sum_{\nu = 0}^{d } \vx_{\mu + \nu } \vx_{\nu}^T \quad (\mu + \nu\  \mathrm{mod}\  d) 
    % \label{eq:gmu-circulant}
    &
    [g_\mu]^\rho_\lambda &=\sum_{\nu} \delta_{\mu+\nu, \lambda} \delta^\rho_\nu %= \delta_{\mu + \rho, \lambda}
    = \delta^\rho_{\lambda-\mu}
    \label{eq:gmu-circ-comp}
\end{align}
with $ g_\mu^{-1}=g_\mu^T$.
}%%%%
% Preserving $<\mu>$ means 
% Note that the only other way we can obtain $\vx_\mu = g_\mu \vx_0$ and preserve the
% Some other $g_\mu $ may still satisfy \eqref{eq:lift-neigh}. 
% For instance, $g_\mu $ can rotate vectors within each $<\nu>$.
\out{
The uniqueness of $g_\mu$ here was because there was a single $L_i$, which generates a unique flow on $\mathcal{S}$. 
For groups with multiple $L_i$, using the path-ordered notation $g_\mu = P\exp[\int_\gamma dt^i L_i]$ we see that at every step along a path $\gamma $ a different $L_i$ step is taken. 
For non-Abelian groups where $[L_i,L_j]\ne 0$, the order of these steps matters and
% What this means is that 
the lift is not uniquely defined.
}%%%%
% for non-Abelian groups. 
% Note that in the tensor notation, $\mathcal{S}$ represents a whole manifold and $g_\mu$ is not moving just one point, but entire neighborhoods.
% Moreover, $g_\mu \in G$ can act on any $\vx_\nu$ and it should again preserve the topology $(\mathcal{S},\mA)$. 
% The Lie algebra basis $L_i$ only moves points $\vx_\nu$ within $<\nu>$. 
% In fact, every choice of the lift defines a ``gauge''.
% $[\vx_0^TL_i]^\nu = [L_i]_0^\nu$ are the components of $L_i$ acting at the origin. 


Using \eqref{eq:gmu-circ-comp} and $g_\mu^{-1} = g_\mu^T$, meaning $[g_\mu^{-1}]^\lambda_\rho = [g_\mu]^\rho_\lambda = \delta^\rho_{\lambda-\mu} = \delta_\rho^{\lambda-\mu}$ and plugging in \eqref{eq:L-conv-tensor0} we get 
\begin{align}
    \vx_0^TL_i g_\mu^{-1}\vf &= [L_i]_0^\rho [g_\mu^{-1}]^\lambda_\rho \vf_\lambda
    = [L_i]_0^\rho 
    % \delta_{\mu+\rho,\lambda}
    \delta_\rho^{\lambda-\mu}
    \vf_\lambda = [L_i]_0^{\lambda-\mu} \vf_\lambda
    \label{eq:xLgf}
\end{align}
If the symmetry is local, meaning only neighboring points mix, $[L_i]_0^\nu$ will only be nonzero when $\nu$ is in the neighborhood of $0$ \nd{on the topology graph $A_{\mu\nu}$}. 
We denote the neighbors of node $\mu$ by $<\mu>$. 
Using this in \eqref{eq:xLgf} we see that it will be nonzero only if $\lambda-\mu \in <0>$. 
This is precisely like the pushforward in our previous formulation. 
The components of $L$ acting on $\vf$ are actually pushed forward from the neighborhood of identity $<0>$. 

\subsection{CNN}

Consider the $k=1$ approximation, where $\hat{L}^\nu_\rho = \pa{\delta^\nu_{\rho+1}-\delta^\nu_{\rho-1}}\hat{L}^0_1 $. 
This is just positive and negative shift by one position. 
Thus, a single layer L-conv yields
\begin{align}
    Q[\vf]^a_\mu&= \vf_\mu^b [W^0]^a_b + \hat{L}_\mu^\nu \vf_\nu^b [\eps W^0]^a_b %\cr &
    = \pa{\vf_\mu^b + \hat{L}_1^0\pa{\vf_{\mu-1}^c- \vf_{\mu+1}^c}\eps_c^b } [W^0]^a_b
\end{align}
which is a 1D CNN with a kernel size $k=3$ and filter weights $V=(-\hat{L}_1^0\eps,I,\hat{L}_1^0\eps) W^0$.
A general CNN with arbitrary kernel size and weights can also be approximated by L-conv layers. 
For weights, note that for $z=\mu \in \Z$, %the sum in $g(z)$ reduces to a delta function and 
$g_\mu=g(z=\mu)$ are circulant matrices that shift by $\mu$ as $ [g_\mu]^\rho_\lambda=\delta^\rho_{\lambda-\mu}$. 
A multi-layer L-conv approximates any $g_\mu$

$\sum_{i=0}^n (\hat{L})^i\vf V_i$
While these is a spacial case of CNN
% $V^a_b= (-\hat{L}_1^0\eps^c_b,\delta^c_b, \hat{L}_1^0\eps^c_b)[W^0]^a_c$. 
Thus, applying $n$ layers of L-conv 
yields a CNN with kernel size $2n+1$. 
\nd{Can the weights be made more general? Right now $V_{-1}=-V_1$. What should we add or change?
If it was two terms this was ok. 
In general if we could add something that shifts $\vf$ by the same amount over the whole kernel size we can create any kernel.}

we get
\begin{align}
    F_n[\vf] &= Q_n\circ\dots Q_1[\vf] =(Q_{n-1}W^0_n +\hat{L}Q_{n-1}W_n) = \sum_{i=0}^n (\hat{L})^i\vf V_i \cr
    [F_n[\vf]]_\rho^a &= \sum_1
\end{align}
where $(\hat{L})^i$ is the $i$th power of $L$ and $V_i$ are expressible in terms of the product of $i$ weights $W^0_a$ and $W_a$ of the $n$ layers. 
Note that for $z=\mu \in \Z$, the sum in $g(z)$ reduces to a delta function and $g_\mu=g(z=\mu)$ become circulant matrices. 
$ [g_\mu]^\rho_\lambda=\delta^\rho_{\lambda-\mu}$ define a lift compatible with $\mA$ and satisfying 
% since $\mA$ is invariant under periodic shifts. 
% This $g_\mu$ also satisfies
\eqref{eq:hat-L-discrete}. 




\paragraph{CNN}
It is also easy to see that  CNN can be encoded as L-conv. 
Note that, generally shift operators used in CNN are thought of as group elements for a discrete permutation group.
However, the same shift operators $L_i$ can be used to create continuous fractional shifts as $(I+\alpha L_i)/(\alpha +1) $.
Since shifts commute with each other, they form a basis for the Lie algebra of an Abelian subgroup of $\mathrm{GL}_d(\R)$.  

\begin{proposition}
    CNN is a special case of L-conv where the generators are shift operators. 
\end{proposition}
\begin{proof}
% In CNN $L_{i}$ are a set of shift operators, which together cover the area of the convolutional kernel.
In 1D CNN, 
for a kernel size $k$ we have $k$ shift operators $L_i$ given by ${L_{i}}_\mu^\nu = \delta_{\mu, \nu -i}$. %index $i\in \{0,1,\cdots k\}$ in \eqref{eq:CNN-general}. 
% Concretely, in 1D CNN, $L^{(i)}$ are 
% \begin{align}
%     {L_{i}}_\mu^\nu = \delta_{\mu, \nu -i}
%     \label{eq:L-CNN-1D}
% \end{align}
Plugging this into \eqref{eq:L-conv} and doing the sum over $\nu$, we recover the convolution formula
\begin{align}
    F(h)_{\mu}^a & = \sigma\pa{\sum_{i,c}  h_{\mu-i}^c W^{i,a}_{c}  +b^a}
    \label{eq:CNN-1D}
\end{align}
In higher dimensional CNN, $i$ covers the relevant flattened indices for the required shifts. 
For instance, a $p\times q$ image, when flattened becomes a vector of length $pq$. 
To cover a $(2,2)$ convolutional kernel, we need shifts to be by $0,1,q,q+1$ pixels. 
Thus, we need four $L_{i}$ given by
\begin{align}
    {L_{i}}_\mu^\nu &= \delta_{\mu, \nu -s_i}, & 
    s_i &= [0,1,q,q+1]_i
    \label{eq:L-CNN-2D}
\end{align}
This means that the number of generators $L_i$ is the size of the convolutional kernel in CNN. 
Generalization to higher dimensions is straightforward. 
\end{proof}

In CNN, covering larger patches is equivalent to the kernels $\kappa(u)$ covering a larger part of the group.
But large convolutional kernels are not generally used. 
Instead, we achieve larger receptive fields by adding more CNN layers, similar to \thref{prop:multi-L-conv}.


\out{
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figs2/L-conv-3-spaces.pdf}
    \caption{
    \textbf{Lie group and Lie algebra:}
    Illustration of the group manifold of a Lie group $G$ (left).  
    The Lie algebra $\mathfrak{g}=T_IG$ is the tangent space at identity $I$. 
    $L_i$ are a basis for $T_IG$.
    If $G$ is connected, any element $g$ can be written as a path-ordered integral $g=P\exp[\int_\gamma dt^i L_i]$. 
    The tangent space $T_gG$ has a basis $gL_ig^{-1}$, the pushforward by $g$.  
    \textbf{
    Manifold vs. discretized Space}
    While real systems can have a continuous manifold  
    $\mathcal{S}_0$ as their base space, often the data collected from is a discrete array $\mathcal{S}$. 
    The discretization (coarsening) will induce some of the topology of $\mathcal{S}_0$ on $\mathcal{S}$ as a graph. 
    Graph neighborhoods $<\mu>$ on the discrete $\mathcal{S}$ represent tangent spaces $T_{\vx_\mu}\mathcal{S}$ and approximate $T_\vx \mathcal{S}_0$.  
    % The coarsening (discretization) produces a space $\mathcal{S}$.  The Lie group $G$ acts on $\mathcal{S}$ and closely approximates $G_0$ ($G\simeq G_0$, e.g. image rotations approximating real rotations).
    The lift takes $\vx\in \mathcal{S}_0$ to $g\in G$, and maps the tangent spaces $T_\vx \mathcal{S}_0\to T_gG$. 
    Each Lie algebra basis $L_{i}\in \mathfrak{g}=T_IG$ generates a vector field on the tangent bundle $TG$ via the pushforward as $L^{(g)} = gL_{i}g^{-1}$. 
    Due to the lift, each $L_i$ also generates a vector field $\hat{L}_i^\alpha(\vx)\ro_\alpha = [gL_i\vx_0]^\alpha \ro_\alpha$, with $\vx=g\vx_0$. 
    Analogously, on $\mathcal{S}$ we get 
    % Since $\mathcal{S}_0$ is lifted to $G$, $L_{0i}$ also generate a flow on $\mathcal{S}_0$, captured by the vector field $\hat{L}_i^\alpha(\vx)\ro_\alpha$. 
    % Similarly, the Lie algebra basis $L_i$ of $G\simeq G_0$ generates a flow on $TG$ and 
    a vector field $[\hat{L}_i]_\mu= g_\mu L_i\vx_0$ on $T\mathcal{S}$, with $\vx_\mu=g_\mu\vx_0$. 
    % Note that tangent spaces on $\mathcal{S}$ are $T_{\vx_\mu}\mathcal{S}=<\mu>$, the neighborhoods of each $\vx_\mu$, and vector fields are weighted graphs, modifying neighbor weights in the graph $\mA$ encoding the topology of $\mathcal{S}$.
    % tensors flowing from every $\vx_\mu$ within the neighborhood $<\mu>$. 
    Note that depicting $\mathcal{S}$ and $\mathcal{S}_0$ as 2D is only for convenience. 
    They may have any dimensions. 
    }
    \label{fig:Lie-group-3-spaces}
\end{figure}
}%%%
% \ry{add summary sentence}




------------

\paragraph{Topology}
\nd{The topology can be encoded using the incidence matrix $\mB: \mathcal{E}\to \mathcal{V}$, where $\mathcal{E}$ and $\mathcal{V}$ are the set of edges and vertices, respectively. 
The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
In contrast, the adjacency matrix component $\mA_{\mu\nu}$ is the weights of the edge from vertex $\mu$ to vertex $\nu$. 
The incidence matrix defines a 1-simplex, capturing part of the topology. 
* discuss boundary operator $\ro$, Hodge Laplacian, MPNN.  
The vector fields $\hat{L}_i$ can naturally be written as a matrix product $[\hat{L}_i]^\mu = \mL_i^\alpha \mB_\alpha^\mu$  }

If the space $\mathcal{S}$ is a grid or discretization of a manifold $\mathcal{S}_0$, it has a topology. 
We encode this topology in an undirected graph (i.e. 1-simplex) with adjacency matrix $\mA$, defining the topological space $(\mathcal{S},\mA)$.
% We denote the adjacency matrix of this undirected graph by $\mA$, with 
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
% Thus, $\mathcal{S}$ together with the graph encoded in $\mA$ define a  topological space, which we denote as $(\mathcal{S},\mA)$.
$\mA$ can encode which pixels are adjacent in images, or crystalline structure, or the discretized space-time in physics. 
$\mA$ can be weighted (e.g. the pixel covariance), %matrix between pixels in an image dataset, 
but we use an unweighted $\mA$, with $\mA_{\mu\nu} \in \{0,1\}$.
% In physics, $\mA$ can encode crystalline structure, or the discretized topology of space-time. 
% The existence of a topology on $\mathcal{S}$ via $\mA$ 
% The topology restricts the lift by the group. % that act on the space.
Define the neighborhood of $\vx_\mu$ to be the set of normalized vectors
\begin{align}
    <\mu>=\left\{\vx = \sum_\nu \mA_{\mu\nu} c_\nu \vx_\nu\Bigg| c_\nu \in \R \mbox{ and }\|c\|^2=1 \right\}
    \label{eq:neigh}
\end{align}
For the sum over a neighborhood we write $ \sum_{\nu\in <\mu>} F_\nu \equiv \sum_\nu \mA_{\mu\nu} F_\nu $. 
% $<\mu> = \mathrm{span}\pa{ \{\vx_\nu | \mA_{\mu\nu} \ne 0 \} }$, the space of normalized vectors spanned by neighbors of $\mu$ in $(\mathcal{S},\mA)$. 
Figure \ref{fig:S0S} summarizes some of the aspects of the discretization as well as analogies between $G$, $\mathcal{S}_0$ and $\mathcal{S}$. 
Technically, the group $G_0$ acting on $\mathcal{S}_0$ and $G$ acting on $\mathcal{S}$ are different.
But we can find a group $G$ which closely approximates $G_0$ (see SI \ref{ap:approx}).
% For example, \citet{rao1999learning} used the Shannon-Whittaker Interpolation \citep{whitaker1915functions} to translate discrete 1D signals by arbitrary, continuous amounts as $f'_\mu = g(z)_\mu^\nu f_\nu $.
% Here $g(z)_\mu^\nu = {1\over d} \sum_{p=-d/2}^{d/2} \cos \pa{{2\pi p\over d}(z+\mu -\nu) } $ approximates the shift operator for continuous $z$.
% The $g(z)$ form a group because $g(w)g(z)=q(w+z)$, which is a representation for periodic 1D shifts. 
For instance, \citet{rao1999learning} used Shannon-Whittaker interpolation theorem \citep{whitaker1915functions} to define continuous 1D translation and 2D rotation groups on discrete data. 
We return to this when expressing CNN as L-conv in \ref{sec:approx}. 

\nd{developing}
\paragraph{Relation to the Laplace-Beltrami Operator}
$\hat{L}_i$ is nonzero where there is an edge in the graph. 
Instead of writing $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$ 
we may use the incidence matrix $\mB$ to encode this. 
Recall that for a graph with node set  $\mathcal{V}$ and edge set $\mathcal{E}$, the incidence matrix $\mB:\mathcal{V}\times  \mathcal{E}\to \{0,1,-1\}$ encodes which nodes $\mu$ are end points of which edge $a$.
$\mB_{\mu a}=1$ or $-1$ if edge $a$ starts or ends at node $\mu$, respectively, and $\mB_{\mu a}=0$ otherwise. 
For undirected graphs, each pair of connected nodes have one incoming and outgoing edge to each other.
The Laplacian $\mL = \mD-\mA$ becomes $\mL = \mB\mB^T$.
A weighted graph can be encoded using a diagonal weight matrix $\mW_{ab}$ for the edges, with the weighted Laplacian $\mL = \mB \mW\mB^T$. 
Since the Lie algebra basis $\hat{L}_i$ is weighting the edges, we can write $\hat{L}_i = l_i^a\mB_{\mu a} $

\paragraph{Lift and group action}
Define the lift via $\vx_\mu = g_\mu \vx_0$. 
Since we chose $\vx_\mu$ to be the canonical basis (one-hot), $\vx_\nu^T\vx_\mu = \delta_\mu^\nu $. 
Thus we can pick $g_\mu$ such that $g_\mu^T= g_\mu^{-1}$, meaning orthogonal matrices.  
Let $(I+\eps L_i) \vx_0 \in <0> $. 
This means that we can write $L_i  \vx_0 = \sum_{\rho \in <0>} 
% \Gamma_{i 0 }^\rho 
[\hat{L}_i]_0^\rho \vx_\rho $ for a set of coefficients $[\hat{L}_i]_0^\rho \in \R$.
%$\Gamma_{i 0 }^\rho \in \R$. 
% for small $\eps \ll 1$. 
% The continuity of $G$ action means that 
We want the $G$-action to preserve the topology of $(\mathcal{S},\mA)$, meaning points which are close remain close after the $G$-action. 
The consequence is that $<\mu>$ can be reached from elements close enough to identity in $<0>$ using $g_\mu$. 
Thus, for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$, meaning for a set of coefficients $ [\hat{L}_i]_\mu^\nu \in \R$ 
%$ \Gamma_{i \mu }^\rho \in \R$ 
we have
\begin{align}
    % <0>\ni&&
    % (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho \in <0>} \Gamma_{i 0 }^\rho \vx_\rho \cr
    % <\mu>\ni&&
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\in <\mu>}  
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu\vx_\nu 
    %= g_\mu \pa{\vx_0+ \eps \sum_{\rho\in <0>} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}
    % \cr
    % &&
    % \Gamma_{i \mu }^\nu &= \sum_{\rho\in <0>} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho = [g_\mu]^\nu_\rho \Gamma_{i 0 }^\rho
\end{align}
Multiplying from the left by $\vx_0^T$ to obtain $\vx^T_\nu g_\mu L_i\vx_0 = [g_\mu L_i\vx_0]^\nu $ we have 
\begin{align}
    [g_\mu L_i\vx_0]^\nu &= 
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu = \sum_{\rho\in <0>} [\hat{L}_i]_0^\rho \vx_\nu^T g_\mu\vx_\rho = [g_\mu]^\nu_\rho [\hat{L}_i]_0^\rho
    \label{eq:hat-L-discrete}
\end{align}
Note that $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$
% $\Gamma_{i \mu }^\nu = \mA_{\mu\nu} \Gamma_{i \mu }^\nu$ 
is only nonzero when $\nu \in <\mu>$. 
This $\hat{L}_i$ is the discrete $\mathcal{S}$ version of the vector field $\hat{L}_i(\vx) = [g L_i \vx_0]^\alpha \ro_\alpha $ in \eqref{eq:dfdg-general}.
In fact, on a graph $\ro_\alpha f(\vx_\mu)$ becomes $\sum_\nu c_\alpha^\nu  \mA_{\mu\nu}(\vf_\mu - \vf_\nu)$ and most of differential geometry can be defined as usual \citep{schaub2020random,lim2015hodge}. 
Thus, on discrete $\mathcal{S}$, the tangent spaces are $<\mu> = T_{\vx_\mu}\mathcal{S}$. 
In \eqref{eq:hat-L-discrete} $\hat{L}_i$ %which we will call the \textbf{global Lie algebra basis}
is a vector field over the discrete tangent bundle $T\mathcal{S}=\{<\mu>|\mu \in \{0,\dots d\}\}$. 
Taking the transpose of \eqref{eq:hat-L-discrete} and using $g_\mu^T = g_\mu^{-1}$, discussed above, and $[\hat{L}_i^T]^\mu_\nu = [\hat{L}_i]^\nu_\mu$, we can rewrite the $L_i$ term in \eqref{eq:L-conv-tensor0} as 
\begin{align}
    \vx_0^TL_i g_\mu^{-1}\vf &=  [\hat{L}_i]^\nu_\mu \vf_\nu
    \label{eq:}
\end{align}
Thus, L-conv in tensor notation can be written in a simple form as follows.



\begin{align}
    \L[W,\eps] &= \sum_n \int_G dg \left\|  W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }\phi_n(g) \right\|^2 
    \cr
    &= \sum_n \int_G dg \br{ 
    \|W^0\phi_n\|^2 + \left\|W^i [\hat{L}_i]^\alpha \ro_\alpha \phi_n \right\|^2 +2\phi_n^T  W^{0T}W^i g [\hat{L}_i]^\alpha \ro_\alpha \phi_n  }
    \label{eq:loss-MSE}\\
    &=\sum_n \int_G dg \br{ M_{ab}\phi_n^a \phi_n^b +\mathbf{h}^{\alpha\beta}_{ab}  \ro_\beta \phi_n^b \ro_\alpha \phi_n^a + [\hat{L}_i]^\alpha \ro_\alpha \pa{\phi_n^T V^i \phi_n}}
    \label{eq:Loss-MSE-simplified}\\
    &= \int d\vx \br{\phi^TM\phi + \ro \phi^T\cdot \mathbf{h}\cdot \ro \phi } + \L_\ro \\
    % \mbox{Invariance: } & u\in G: \quad u^T\mathbf{g}_{ab} u = \mathbf{g}_{ab}
\end{align}
where $W^i = W^0 \ba{\eps}^i$.  
The integration measure can be changed from $\int_G dg$ to $\int d^n\vx/|\det(dg/d\vx)| $ using the Jacobian of $dg/d\vx$. 
We use \eqref{eq:dfdg-general} to replace $gL_i\cdot df/dg = \hat{L}_i^\alpha \ro_\alpha f $. 
\nd{For a compact subgroup $H\subset G$, the $L_i \in T_I H$ may satisfy $\ro_\alpha \hat{L}_i^\alpha =0 $.
Why? $T_n$ is an exception where it is divergence free. 
For scaling it doesn't work, as it's non-compact. 
But for rotations it works. 
Is this related to closed forms being exact? 
}




\paragraph{Relation to physics}
Notice that \eqref{eq:Loss-MSE-simplified} is the MSE loss for the equivariant architecture L-conv. 
We derived it purely using machine learning and equivariance considerations.
But physicists will recognize \eqref{eq:Loss-MSE-simplified} as a generalization of the non-interacting field theory action (integral of a Lagrangian).
In field theory, $f(x)$ is called a field, $M_{ab}$ is the ``mass matrix'' and the second term $\ro^\mu f^a \ro_\mu f_a$ is the ``kinetic'' term. 
% Mass matrices appear in the standard model of particle physics in the Higgs interaction  
The main difference with the ansatz used in physics is that the metrics on $\mathcal{S}$ and $\mathcal{F}$ are fused into a tensor $\mathbf{g}$. 
In physics the ansatz used is much simpler and $\mathbf{g}$ is factorized into a tensor product $\mathbf{g} = \eta \otimes \delta $, where $\eta_{\alpha\beta}$ is a Riemannian metric on $\mathcal{S}$ and $\delta$, usually the Kronecker delta, is the metric on the feature space (internal space or fibers in physics). 


In physics, the loss function \eqref{eq:Loss-MSE-simplified} is used in two ways. 
The primary way is when the parameters $M$ and $\mathbf{g}$ are known, while the features $f(\vx)$ minimizing the loss are not known. 
In this case, the loss lacks the $\sum_n$ and $\L[f]$ is a function of $f$, with $M$ and $\mathbf{g}$ fixed.
Therefore a variational procedure known as the Euler-Lagrange equations is used to find equations for $f(\vx)= \argmin_f\L[f]$. 
However, when $M$ and $\mathbf{g}$ are not known, and instead we have observational data $f_n$, physicists also use \eqref{eq:Loss-MSE-simplified} the same way as ML. 
In this case \eqref{eq:Loss-MSE-simplified} is a variational ansatz used to identify parameters $M$ and $\mathbf{g}$ such that the expected loss for the observed $f_n$ is minimized.
% As noted, \eqref{eq:Loss-MSE-simplified} is in one way more general than the ansatz used in physics.
% We can absorb the mass matrix by defining $\phi = W^0 f$ yielding the integrand $\phi^T \phi + \ro_\alpha \phi^T\gamma^{\alpha \beta}\ro_\beta $, with a new metric $\gamma^{\alpha\beta}_{ab}=[\hat{L}_i^T\ba{\eps}^i\ba{\eps}^j\hat{L}_j]^{\alpha\beta}_{ab} %= \sum_c [\ba{\eps}^i]_{ac}\hat{L}_i^\alpha [\ba{\eps}^j]_{bc}\hat{L}_j^\beta
% $ 
% In physics, usually the mass matrix $M$ is not related to the metrics $\mathbf{g}$. 





% \out
{


\subsection{Absorbing labels into features}
In supervised learning the input is a pair $f_n,y_n$. 
the labels $y_n$ can have their own $G$ action, including being $G$-invariant. 
We can concatenate $[f_n|y_n]\to f'_n$ to define a merged feature which has a well-defined $G$ action.  
\nd{Can we absorb $y$ into $Q[f]$? Maybe as extra dims which are invariant under $G$, until $W^0$ subtracts $y$? 
This can be seen as $W^0Q_0[f](g) - y &= V^0(Q_0[f]|y)$. 
The rest of the $G$ action in L-conv can also work since $dy/dg = 0$ and we only get the $W^0y$ term. 
}

Note the similarity of these with the gradient in polar coordinates. 
In polar coordinates $(r,\theta)$ the gradient is $\del = (\ro_r, r^{-1} \ro_\theta)$, which is $1/r$ times $gL_i\cdot d/dg$. 
This is because of the determinant of $gL_i$. 
Essentially $gL_i$ is the coordinate transformation from whatever basis we chose for $\vx_0$. 
In fact, using $\vu_i = gL_i $
% Thus, in L-conv we get $\eps^i gL_i\cdot df/dg = \eps \cdot \del f$,

}%%%%
%
% \out
{
\nd{
\begin{itemize}
    \item Hamiltonian
    % \item Gauge invariant loss
    \item Conservation Laws
\end{itemize}
Discuss how group invariance of the action functional (loss function) in physics is related to building scalars from L-conv. 
% For exampe, does an MSE loss using L-conv look like the kinetic terms $\ro_\mu \phi \ro^\mu \phi$ in field theory? 

% Right now we have something like $\vx_0^T[gL]^T\ro f$. 
% How do we make a group invariant Loss from this? 
}   
}%%%





\section{Tensor notation \label{ap:tensor} }
If the dataset being analyzed is in the form of $f(\vx)$ for some sample of points $\vx$, together with derivatives $\del f(\vx) $, we can use the formulation above. 
However, in many datasets, such as images, $f(\vx)$ is given as a finite dimensional array or tensor, with $\vx$ taking values over a grid. 
% In this case all the discussions above still hold, as discuss now. 
% In particular, e
Even though the space $\mathcal{S}$ is now discrete, the group which acts on it can still be continuous (e.g. image rotations). 
Let $\mathcal{S}= \{\vx_0,\dots \vx_{d-1}\}$ contain $d$ points. 
Each $\vx_\mu$ represents a coordinate in higher dimensional grid.
For instance, on a $10\times 10$ image, $\vx_0$ is $(x,y)=(0,0)$ point and $ \vx_{99}$ is $(x,y) =(9,9)$.


\paragraph{Feature maps}
To define features $f(\vx_\mu)\in \R^m$ for $\vx_\mu \in \mathcal{S}$, we embed $\vx_\mu \in \R^d$ and 
encode them as the canonical basis (one-hot) vectors with components $[\vx_\mu]^\nu = \delta_\mu^\nu$ (Kronecker delta), e.g. $\vx_0 = (1,0,\dots, 0)$.
The feature space becomes $\mathcal{F}= \R^d \otimes \R^m $, meaning feature maps $\vf \in \mathcal{F}$ are $d\times m$ tensors, with $f(\vx_\mu) = \vx_\mu^T \vf = \vf_\mu $.

\paragraph{Group action}
\nd{Change to $\vx_\mu^T g^T$ for less confusion.}
Any subgroup $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group (invertible $d\times d$ matrices) acts on $\R^d$ and $\mathcal{F}$. 
Since $\vx_\mu \in \R^d$, $g \in G$ also naturally act on $\vx_\mu$. 
The resulting $\vy = g \vx_\mu $ is a linear combination $\vy = c^\nu \vx_\nu$ of elements of the discrete $\mathcal{S}$, not a single element.
The action of $G$ on $\vf$ and $\vx$, can be defined in multiple equivalent ways.
% The most elegant one is if w
We define $f(g \cdot \vx_\mu) = \vx_\mu^T g^{-1}\vf , \forall g\in G$.
% consistent with the lift. 
% This makes the group action on $\vf$ the natural action of $G$, meaning 
For $w\in G$ we have 
\begin{align}
    w\cdot f(\vx_\mu)&= f(w^{-1}\cdot \vx_\mu) = \vx_\mu^T[w^{-1} ]^{-1}\vf = \vx_\mu^T w \vf   
\end{align}
Dropping the position $\vx_\mu$, the transformed features are simply a matrix product $w\vf$. 


\paragraph{G-conv and L-conv in tensor notation} 
Writing G-conv \eqref{eq:G-conv} in the tensor notation we have 
\begin{align}
    [\kappa\star f](g\vx_0) = \int_G \kappa(v)f(gv\vx_0) dv = \vx_0^T \int_G v^{-1} g^{-1} \vf \kappa^T(v) dv \equiv \vx_0^T [\vf \star \kappa](g) 
    \label{eq:G-conv-tensor}
\end{align}
where we moved $\kappa^T(v) \in \R^m \otimes \R^{m'}$ to the right of $\vf$ because it acts as a matrix on the output index of $\vf$.
The equivariance of \eqref{eq:G-conv-tensor} is readily checked with $w\in G$
\begin{align}
    w\cdot [\vf \star \kappa](g) & = [\vf \star \kappa](w^{-1}g) 
    = \int_G v^{-1} [w^{-1}g]^{-1} \vf \kappa^T(v) dv 
    %= \int_G v^{-1} g^{-1} w\vf \kappa^T(v) dv 
    =  [w \vf \star \kappa](g)
\end{align}
where we used $[w^{-1}g]^{-1}\vf = g^{-1} w\vf $.
Similarly, we can rewrite L-conv \eqref{eq:L-conv-def0} in the tensor notation. 
Defining $v_\eps =I+ \ba{\eps}^i L_i $ 
\begin{align}
    Q[\vf](g) 
    &= W^0 f\pa{g\pa{I+ \ba{\eps}^i L_i}} 
    = \vx_0^T \pa{I+ \ba{\eps}^i L_i}^{-1} g^{-1} \vf W^{0T} \cr
    &= \vx_0^T \pa{I- \ba{\eps}^i L_i} g^{-1} \vf W^{0T} 
    % = \br{\vf_\mu + \ba{\eps}^i [L_i \vf]_\mu }W^{0T} 
    % \cr
    \label{eq:L-conv-tensor0}
\end{align}
The equivariance of L-conv in tensor notation is again evident from the $g^{-1} \vf$ part, resulting in $Q[w\vf](g) = Q[\vf](w^{-1}g) = w\cdot Q[\vf](g)$. 
Next, we will discuss how to implement \eqref{eq:L-conv-tensor0} in practice and how to learn symmetries with L-conv.
% means and how it impacts the learning of symmetries using L-conv. 
We will also discuss the relation between L-conv and other neural architectures. 

\subsection{Interpretation of L-conv}
To implement \eqref{eq:L-conv-tensor0} we need to specify the lift and the form of $L_i$. 
We will now discuss the mathematical details leading to and easy to implement form of \eqref{eq:L-conv-tensor0}. 
% $\hat{L}_i$. 

\out{
Recall that $L_i$ reside in the tangent space of the identity. 
Defining the lift via $\vx_\mu= g_\mu \vx_0$, the $d\times d$ matrices $L_i$ are only nonzero in the neighborhood of $\vx_0$. 
L-conv acts on other $\vx_\mu$ via the pushforward $L_i^{(g_\mu)}=g_\mu L_i g_\mu^{-1}$ appearing in $\vx_0^TL_i g_\mu^{-1}= \vx_\mu^T L_i^{(g_\mu)}$ (derived below). 
Thus, the set of $\vx_0^TL_i g_\mu^{-1}$ for all $\mu$, yielding the discrete analogue of the operator $\hat{L}_i$ in \eqref{eq:dfdg-general}, which is defined over the entire tangent bundle $T\mathcal{S}$ instead of only $T_{\vx_0}\mathcal{S}$. 
For example, for image rotation $\hat{L}_i$ is the infinitesimal generator of rotations of the full image, while $L_i$ is a local operator which rotates only the neighborhood of a chosen pixel $\vx_0$. 
When learning symmetries in the tensor notation we can learn the entire $\hat{L}_i$ at once.
We will now discuss the mathematical details leading to $\hat{L}_i$. 
}%%%%%
\out{
% Dropping $\vx_0^T$ we are left with a peculiar equation.
While the group action on $\vf$ is simply $w\vf$, 
% While the normal action of $v_\eps$ would be $v_\eps \vf$, we have a $g^{-1}$ (lift of the input) sitting in $v_\eps g^{-1} \vf$. 
% To realize the oddness, note that 
% unlike the simple linear action $w\vf$ for the features, 
the group action on L-conv is $w\cdot Q[\vf](g) = v_\eps g^{-1} w\vf W^{0T} $.
While $w\cdot Q$ is still a linear action, it is not a simple left matrix product. 
%which is not a simple linear action from the left like $w\vf$.
}%%%%%

\paragraph{Topology}
We introduced the discrete space $\mathcal{S}$ as a set of points. 
In many cases the space has a topology, e.g. when $\mathcal{S}$ are a discretization of a manifold $\mathcal{S}_0$, or vertices on a lattice or a general graph. 
% If the points in $\mathcal{S}$ is a graph, a lattice, or the discretization of a manifold $\mathcal{S}_0$, it has a topology. 
We encode this topology in an undirected graph (i.e. 1-simplex) with adjacency matrix $\mA$, defining the topological space $(\mathcal{S},\mA)$.
% We denote the adjacency matrix of this undirected graph by $\mA$, with 
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
\out{
The components $\mA_{\mu\nu}$ encode the edge between $\mu$ and $\nu$.
% Thus, $\mathcal{S}$ together with the graph encoded in $\mA$ define a  topological space, which we denote as $(\mathcal{S},\mA)$.
$\mA$ can encode which pixels are adjacent in images, or crystalline structure, or the discretized space-time in physics. 
$\mA$ can be weighted (e.g. the pixel covariance), %matrix between pixels in an image dataset, 
but we use an unweighted $\mA$, with $\mA_{\mu\nu} \in \{0,1\}$.
% In physics, $\mA$ can encode crystalline structure, or the discretized topology of space-time. 
% The existence of a topology on $\mathcal{S}$ via $\mA$ 
% The topology restricts the lift by the group. % that act on the space.
}%%
Define the neighborhood of $\vx_\mu$ to be the set of normalized vectors
\nd{
Neighborhood should be defined using the incidence matrix $\mB$ to ensure the vectors are $\vx_\nu-\vx_\mu \in T_{\vx_\mu}\mathcal{S}$. 
We can do so by picking the set of edges $\{a|\mB_a^\mu =-1\}$.  
}

\begin{align}
    <\mu>=\left\{\vx = \sum_\nu \mA_{\mu\nu} c_\nu \vx_\nu\Bigg| c_\nu \in \R \mbox{ and }\|c\|^2=1 \right\}
    \label{eq:neigh}
\end{align}
For the sum over a neighborhood we write $ \sum_{\nu\in <\mu>} F_\nu \equiv \sum_\nu \mA_{\mu\nu} F_\nu $. 
% $<\mu> = \mathrm{span}\pa{ \{\vx_\nu | \mA_{\mu\nu} \ne 0 \} }$, the space of normalized vectors spanned by neighbors of $\mu$ in $(\mathcal{S},\mA)$. 
Figure \ref{fig:S0S} summarizes some of the aspects of the discretization as well as analogies between $G$, $\mathcal{S}_0$ and $\mathcal{S}$. 
Technically, the group $G_0$ acting on $\mathcal{S}_0$ and $G$ acting on $\mathcal{S}$ are different.
But we can find a group $G$ which closely approximates $G_0$ (see SI \ref{ap:approx}).
% For example, \citet{rao1999learning} used the Shannon-Whittaker Interpolation \citep{whitaker1915functions} to translate discrete 1D signals by arbitrary, continuous amounts as $f'_\mu = g(z)_\mu^\nu f_\nu $.
% Here $g(z)_\mu^\nu = {1\over d} \sum_{p=-d/2}^{d/2} \cos \pa{{2\pi p\over d}(z+\mu -\nu) } $ approximates the shift operator for continuous $z$.
% The $g(z)$ form a group because $g(w)g(z)=q(w+z)$, which is a representation for periodic 1D shifts. 
For instance, \citet{rao1999learning} used Shannon-Whittaker interpolation theorem \citep{whitaker1915functions} to define continuous 1D translation and 2D rotation groups on discrete data. 
We return to this when expressing CNN as L-conv in \ref{sec:approx}. 

\out{

\nd{
% The topology can be encoded using the incidence matrix $\mB: \mathcal{E}\to \mathcal{V}$, where $\mathcal{E}$ and $\mathcal{V}$ are the set of edges and vertices, respectively. 
% The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
In contrast, the adjacency matrix component $\mA_{\mu\nu}$ is the weights of the edge from vertex $\mu$ to vertex $\nu$. 
The incidence matrix defines a 1-simplex, capturing part of the topology. 
* discuss boundary operator $\ro$, Hodge Laplacian, MPNN.  
  }
\nd{developing}
\paragraph{Relation to the Laplace-Beltrami Operator}
$\hat{L}_i$ is nonzero where there is an edge in the graph. 
Instead of writing $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$ 
we may use the incidence matrix $\mB$ to encode this. 
Recall that for a graph with node set  $\mathcal{V}$ and edge set $\mathcal{E}$, the incidence matrix $\mB:\mathcal{V}\times  \mathcal{E}\to \{0,1,-1\}$ encodes which nodes $\mu$ are end points of which edge $a$.
$\mB_{\mu a}=1$ or $-1$ if edge $a$ starts or ends at node $\mu$, respectively, and $\mB_{\mu a}=0$ otherwise. 
For undirected graphs, each pair of connected nodes have one incoming and outgoing edge to each other.
The Laplacian $\mL = \mD-\mA$ becomes $\mL = \mB\mB^T$.
A weighted graph can be encoded using a diagonal weight matrix $\mW_{ab}$ for the edges, with the weighted Laplacian $\mL = \mB \mW\mB^T$. 
Since the Lie algebra basis $\hat{L}_i$ is weighting the edges, we can write $\hat{L}_i = l_i^a\mB_{\mu a} $
}%%%

\paragraph{Lift and group action}
Define the lift via $\vx_\mu = g_\mu \vx_0$. 
Since we chose $\vx_\mu$ to be the canonical basis (one-hot), $\vx_\nu^T\vx_\mu = \delta_\mu^\nu $. 
Thus we can pick $g_\mu$ such that $g_\mu^T= g_\mu^{-1}$, meaning orthogonal matrices.  
Let $(I+\eps L_i) \vx_0 \in <0> $. 
This means that we can write $L_i  \vx_0 = \sum_{\rho \in <0>} 
% \Gamma_{i 0 }^\rho 
[\hat{L}_i]_0^\rho \vx_\rho $ for a set of coefficients $[\hat{L}_i]_0^\rho \in \R$.
%$\Gamma_{i 0 }^\rho \in \R$. 
% for small $\eps \ll 1$. 
% The continuity of $G$ action means that 
We want the $G$-action to preserve the topology of $(\mathcal{S},\mA)$, meaning points which are close remain close after the $G$-action. 
The consequence is that $<\mu>$ can be reached from elements close enough to identity in $<0>$ using $g_\mu$. 
Thus, for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$, meaning for a set of coefficients $ [\hat{L}_i]_\mu^\nu \in \R$ 
%$ \Gamma_{i \mu }^\rho \in \R$ 
we have
\begin{align}
    % <0>\ni&&
    % (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho \in <0>} \Gamma_{i 0 }^\rho \vx_\rho \cr
    % <\mu>\ni&&
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\in <\mu>}  
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu\vx_\nu 
    %= g_\mu \pa{\vx_0+ \eps \sum_{\rho\in <0>} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}
    % \cr
    % &&
    % \Gamma_{i \mu }^\nu &= \sum_{\rho\in <0>} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho = [g_\mu]^\nu_\rho \Gamma_{i 0 }^\rho
\end{align}
Multiplying from the left by $\vx_\nu^T$ to obtain $\vx^T_\nu g_\mu L_i\vx_0 = [g_\mu L_i\vx_0]^\nu $ and  
inserting $I= \sum_\rho \vx_\rho \vx_\rho^T$ we have 
\begin{align}
    [g_\mu L_i\vx_0]^\nu &= 
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\nu 
    = \sum_{\rho} \vx_\nu^T g_\mu\vx_\rho \vx^T_\rho L_i \vx_0
    \cr & = \sum_{\rho\in <0>}  \vx_\nu^T g_\mu\vx_\rho [\hat{L}_i]_0^\rho
    = [g_\mu]^\nu_\rho [\hat{L}_i]_0^\rho
    \label{eq:hat-L-discrete}
\end{align}
Note that $[\hat{L}_i]_\mu^\nu = \mA_{\mu\nu}[\hat{L}_i]_\mu^\nu$
% $\Gamma_{i \mu }^\nu = \mA_{\mu\nu} \Gamma_{i \mu }^\nu$ 
is only nonzero when $\nu \in <\mu>$. 
This can be rewritten using the ``incidence matrix'' $\mB:\mathcal{S}\to \mathcal{E}$, where $\mathcal{E}$ is the set of edges of the graph \citep{schaub2020random}.
The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
$\hat{L}_i$ become weights for the edges $\alpha$ as 
\nd{ $<\mu>$ as defined above is not $T_{g_\mu}G$ because its vectors do not start from $\vx_\mu$.
We have $\vx_\nu-\vx_\mu \in T_{g_\mu}G$ for $\vx_\nu \in <\mu>$. Does $\hat{L}_i\vf$ have to subtract $\vf_\nu-\vf_\mu$? 
}

\out{
In \eqref{eq:L-conv} we used the vector field $\hat{L}_i$.
Vector fields and partial derivatives $\ro_\alpha$ can be defined on 1-simplexes using the ``incidence matrix'' $\mB:\mathcal{S}\to \mathcal{E}$, where $\mathcal{E}$ is the set of edges of the graph \citep{schaub2020random}.
The component $\mB^\mu_\alpha$ for node $\mu$ and edge $\alpha$ is $-1$  if $\alpha $ is outgoing from  $\mu$, $+1$ if it's incoming, and $0$ otherwise. 
It yields the graph Laplacian via $\mB^T\mB = \mD-\mA$, where $\mD_{\mu\nu} = \delta_{\mu\nu}\sum_\rho \mA_{\rho\mu}$ is the degree matrix.
The vector field component $[\hat{L}_i]^\nu_\mu$ is putting a weight on the edge from $\mu$ to $\nu$ and can be written as 
$[\hat{L}_i]^\nu_\mu = \sum_{\alpha \in <\mu>} \mL_i^\alpha \mB^\nu_\alpha $

can naturally be written as a matrix product $[\hat{L}_i]^\mu = \mL_i^\alpha \mB_\alpha^\mu$
\nd{Since the Lie algebra basis $\hat{L}_i$ is weighting the edges, we can write $\hat{L}_i = l_i^a\mB_{\mu a} $}
}%
This $\hat{L}_i$ is the discrete $\mathcal{S}$ version of the vector field $\hat{L}_i(\vx) = [g L_i \vx_0]^\alpha \ro_\alpha $ in \eqref{eq:dfdg-general}.
In fact, on a graph $\ro_\alpha f(\vx_\mu)$ becomes $\sum_\nu c_\alpha^\nu  \mA_{\mu\nu}(\vf_\mu - \vf_\nu)$ and most of differential geometry can be defined as usual \citep{schaub2020random,lim2015hodge}. 
Thus, on discrete $\mathcal{S}$, the tangent spaces are $<\mu> = T_{\vx_\mu}\mathcal{S}$. 
In \eqref{eq:hat-L-discrete} $\hat{L}_i$ %which we will call the \textbf{global Lie algebra basis}
is a vector field over the discrete tangent bundle $T\mathcal{S}=\{<\mu>|\mu \in \{0,\dots d\}\}$. 
Taking the transpose of \eqref{eq:hat-L-discrete} and using $g_\mu^T = g_\mu^{-1}$, discussed above, and $[\hat{L}_i^T]^\mu_\nu = [\hat{L}_i]^\nu_\mu$, we can rewrite the $L_i$ term in \eqref{eq:L-conv-tensor0} as 
\begin{align}
    \vx_0^TL_i g_\mu^{-1}\vf &=  [\hat{L}_i]^\nu_\mu \vf_\nu
    \label{eq:}
\end{align}
Thus, L-conv in tensor notation can be written in a simple form as follows.



\paragraph{Lie Algebra Convolutional Layer}
% \begin{figure}
%     \centering
\begin{wrapfigure}{r}{.5\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, this action is analogous to a Graph Convolutional Network with $d$ nodes and $m_l$ features per node. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-30pt}
\end{wrapfigure}
% \end{figure}

In conclusion, the discrete space L-conv \eqref{eq:L-conv-tensor0} can be rewritten using the global Lie algebra basis $\hat{L}_i$
\begin{align}
    % \mbox{L-conv}:\  
    Q[\vf] &=   \pa{\vf + \hat{L}_i\vf \ba{\eps}^i} W^{0T} \cr 
    Q[\vf]_\mu^a &= \vf_\mu^b [W^{0T}]_b^a + 
    [\hat{L}_i]_\mu^\nu \vf_\nu^c \br{W^i}^a_c
    \label{eq:L-conv-tensor}
\end{align}
Where $W^i=W^0\ba{\eps}^i$, $W^0 \in \R^{m_{in}}\otimes \R^{m_{out}}$ and $\ba{\eps}^i \in \R^{m_{in}}\otimes \R^{m_{in}}$ are trainable weights. 
The $\hat{L}_i$ can be either inserted as inductive bias or they can be learned to discover symmetries. % we will be learning $\hat{L}_i$. 
% We will discuss learning symmetries
We derived L-conv from G-conv using kernels around identity. 


\paragraph{Nonlinear activation}
% Regarding nonlinear activation functions, as discussed in \nd{cite prior work}, it depends on whether they commute with the group action. 
% When $G$ is not a Lie group, many point-wise nonlinearities can preserve it. 
% As many nonlinear activation functions are not compatible with equivariance. 
% Note that, similar to discussion in
As noted in \cite{weiler20183d}, an arbitrary nonlinear activation $\sigma $ may not keep the architecture equivariant under $G$, but linear activation remains equivariant.

\nd{Vector field plots of $\hat{L}_i$ in experiments.
Apply orthogonality with $B_{ij} = 2k\Tr{l_il_j}-2\Tr{l_i}\Tr{l_j}=$ }


\out{
In particular, for a fixed $i$ and $\eps\ll 1$, we have 
\begin{align}
    \vx_i &= (I+\eps L_i) \vx_\mu = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu \in <\mu> \\
    [L_i]^\nu_\mu &= \vx_\nu^T L_i \vx_\mu = {1\over \eps }\pa{\vx_\nu^T\vx_i- \delta^\nu_\mu}= \mA_{\mu\nu}\Gamma_{i\mu}^\nu
    % \vx_\nu^T\vx_i &= \delta^\nu_\mu + \eps [L_i]^\nu_\mu = \delta^\nu_\mu + \eps \mA_{\mu\nu}[l_i]^\nu 
\end{align}
Next, we note that writing $g_\mu = P\exp[\int_\gamma dt^iL_i]$ we can use the Lie algebra $[L_i,L_j={c_{ij}}^kL_k$ to pass $L_i$ through

Let $(I+\eps L_i) \vx_0 \in <0> $ for small $\eps \ll 1$. 
The continuity of $G$ action means that for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$. 
Therefore
\begin{align}
    (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho \cr
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu = g_\mu \pa{\vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}\cr
    \mA_{\mu\nu} \Gamma_{i \mu }^\nu   \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho
\end{align}

This means that any small $v_\eps = I+\eps^iL_i \in T_IG$ must move points $\vx_\mu$ within their neighborhood, meaning for $v_\eps = I+\eps^iL_i \in G$ close to identity and $\vx_\mu \in \mathcal{S}$ we have
\begin{align}
    % \forall v_\eps &= I+\eps^iL_i \in G, \quad \forall\vx_\mu \in \mathcal{S},\quad 
    &\exists c\in \R^d, & v_\eps \vx_\mu &= \sum_\nu c^\nu \mA_{0\nu}\vx_\nu \in <\mu >. 
    \label{eq:G-neigh-preserve}
\end{align}
}%%%

% Next, we establish relations between L-conv and other commonly used architectures. 




% \subsection{a}

\out
{
Next, we need to change the integration from $\int_G dg$ to $\int d\vx$.
Since $G$ acts on the vector space $\mathcal{S}\sim \R^n$, we have $G\subset \mathrm{GL}_n(\R)$. 
The Haar measure for $\mathrm{GL}_n(\R)$ is $d\mu(g) = d^{n^2}g/|\det(g)|$, where $d^{n^2}g$ is the Lebesgue integration measure for $n\times n$ matrices. 
We can change the integration variables to $d^n \vx$ using $\vx = g\vx_0$. 
Using \eqref{eq:dgx0-dg} we have 
$dg^\alpha_\beta ={dg^\alpha_\beta\over d\vx^\rho} d\vx^\rho = d\vx^\rho / (\delta^\rho_\beta \vx_0^\alpha)$. 
Since $\vx_0^\alpha = \delta_0^\alpha$ the integration measure simply becomes $d^n x$.
}%
\out{
\nd{Check if invariance yields $ u\in G: \quad u^T\mathbf{g}_{ab} u = \mathbf{g}_{ab}$}
\nd{Linear Sigma Model. Equivariance becomes invariance of metric as 
$u^T\mathbf{g}_{ab} u = \mathbf{g}_ab$
}. 
\ry{create a metric}
\nd{Laplace Beltrami operator via incidence matrix and $L_i$}
\nd{Check
\begin{align}
    \L[W,\eps]
    &=\sum_n \int_G dv \br{ M_{ab}\phi_n^a \phi_n^b +\mathbf{g}^{\alpha\beta}_{ab}  \ro_\beta \phi_n^b \ro_\alpha \phi_n^a} + \L_\ro 
    \label{eq:Loss-MSE-simplified}\\
    &= \int d\vx \br{\phi^TM\phi + \ro \phi^T\cdot \mathbf{g}\cdot \ro \phi } + \L_\ro 
\end{align}
}
\out{
Where, defining  $\hat{L}_i(g) = gL_i\vx_0$ and $W^i= W^0\ba{\eps}^i$,
\begin{align}
    M &\equiv W^{0T}W^0 &
    % \mathbf{g}=[\hat{L}_i^TW^{iT}W^j\hat{L}_j]^{\alpha\beta}_{ab} =
    \mathbf{g}^{\alpha\beta}_{ab} = \sum_c [W^i]_{ac}\hat{L}_i^\alpha [W^j]_{bc}\hat{L}_j^\beta
\end{align}
where $W^i= W^0\ba{\eps}^i$. 
}%
\out{
After some simplification using \eqref{eq:dfdg-general} we find (see SI \ref{ap:Loss-MSE})
\begin{align}
    % \L[W] &= \sum_n \int_G dg \left\|  W^0 \br{I + \ba{\eps}^i U_i^\alpha \ro_\alpha }f_n(g) \right\|^2 + \L_\ro\cr
    % &= \sum_n \int_G dg \br{  \|W^0f_n\|^2 +\|W^iU_i^\alpha \ro_\alpha f_n\|^2   } + \L_\ro \cr
    %  &= \sum_n \int_G dg \br{  f_n^TMf_n +\ro_\alpha f_n^T\mathbf{g}^{\alpha\beta}  \ro_\beta f_n } + \L_\ro \cr
    \L[W]&= \sum_n \int_G dg \br{ M_{ab}f_n^a f_n^b +\mathbf{g}^{\alpha\beta}_{ab}  \ro_\beta f_n^b \ro_\alpha f_n^a} + \L_\ro 
    \label{eq:Loss-MSE-simplified}
\end{align}
}%%%
where %$\L_\ro$ is the third term in \eqref{eq:loss-MSE} and becomes a boundary term 
$\L_\ro = \sum_n {\phi_n}^T[\Sigma \cdot \delta\vx] {\phi_n}$ is a boundary term from partial integration of the single derivative terms. 
Here, $\Sigma$ is the normal to the boundary $\ro \mathcal{S}$ and $\delta \vx$ found from $\ba{\eps}^i gL_i\cdot d\phi/dg = \delta \vx^\alpha \ro_\alpha \phi(\vx)$. 
In the first term in \eqref{eq:Loss-MSE-simplified},  $M=W^{0T}W^0$. 
In the second term $\mathbf{g}^{\alpha\beta}_{ab} = \sum_c [W^i]_{ac}\hat{L}_i^\alpha [W^j]_{bc}\hat{L}_j^\beta $, where
%we have defined 
$\hat{L}_i(g) = gL_i\vx_0$, $W^i= W^0\ba{\eps}^i$ and used \eqref{eq:dfdg-general} (see SI \ref{ap:Loss-MSE}).
$\mathbf{g}^{\alpha\beta}_{ab}$
combines a Riemannian metric $\mathbf{g}^{\alpha\beta}$ on $\mathcal{S}$ with a metric on the feature space $\mathcal{F}$ as $\mathbf{g}_{ab}$.


\paragraph{Learning classical dynamics}
In physics, classical mechanics can be though of as a 1D field theory, meaning the features are $f(\vx) = x(t)\in \mathcal{F}=\R^n$ the position of the object and the base space $\mathcal{S}=\R$ is time. 
The symmetry group is $G=T_1 = (\R,+)$ the 1D (time) translation, with $L=I$. 
The task here is to learn the 

\paragraph{Conservation laws}
Also in physics the boundary term $\L_\ro $ is almost always ignored. 
Instead, for conservation laws in Noether's theorem a different boundary term is extracted by partial integration of the kinetic term, which gives rise to
% $\ro_\alpha f \mathbf{g}^{\alpha\beta} \ro_\beta f$ is the kinetic

This requires the loss to change by at most a constant with zero parameter gradients, meaning 
\begin{align}
    \L[\theta, g\cdot f] &= \L[\theta,f] + \ell, & 
    {\ro \ell \over \ro \theta} &= 0
\end{align}


\nd{
but if it is non-zero it can be a conserved quantity. 
Check its Noether's Theorem.
In normal Noether's theorem, the conserved charge comes only from the kinetic term because that is the only term which contains derivatives and that can produce boundary terms. 
Here we have an additional term, which at the boundary does not have any derivatives and was neglected in physics. 
}
}%%%%



\subsection{Interpretation of L-conv}
To implement \eqref{eq:L-conv-tensor0} we need to specify the lift and the form of $L_i$. 
We will now discuss the mathematical details leading to and easy to implement form of \eqref{eq:L-conv-tensor0}. 

\paragraph{Topology}
Although he discrete space $\mathcal{S}$ is a set of points, in many cases it has a topology.
For instance, $\mathcal{S}$ can be a discretization of a manifold $\mathcal{S}_0$, or vertices on a lattice or a general graph. 
% If the points in $\mathcal{S}$ is a graph, a lattice, or the discretization of a manifold $\mathcal{S}_0$, it has a topology. 
We encode this topology in an undirected graph (i.e. 1-simplex) with vertix set $\mathcal{S}$ edge set $\mathcal{E}$.
Instead of the commonly used graph adjacency matrix $\mA$, we will use the incidence matrix $\mB:\mathcal{S}\times  \mathcal{E}\to \{0,1,-1\}$.
$\mB^\mu_\alpha=1$ or $-1$ if edge $\alpha$ starts or ends at node $\mu$, respectively, and $\mB^\mu_\alpha=0$ otherwise (undirected graphs have pairs of incoming and outgoing edges ).
Similar to the continuous case we will denote the topological space $(\mathcal{S},\mathcal{E},\mB)$ simply by $\mathcal{S}$. 
\out{
The Laplacian $\mL = \mD-\mA$ becomes $\mL = \mB\mB^T$.
A weighted graph can be encoded using a diagonal weight matrix $\mW_{ab}$ for the edges, with the weighted Laplacian $\mL = \mB \mW\mB^T$.
}%

Figure \ref{fig:S0S} summarizes some of the aspects of the discretization as well as analogies between $\mathcal{S}_0$ and $\mathcal{S}$. 
Technically, the group $G_0$ acting on $\mathcal{S}_0$ and $G$ acting on $\mathcal{S}$ are different.
But we can find a group $G$ which closely approximates $G_0$ (see SI \ref{ap:approx}).
% For example, \citet{rao1999learning} used the Shannon-Whittaker Interpolation \citep{whitaker1915functions} to translate discrete 1D signals by arbitrary, continuous amounts as $f'_\mu = g(z)_\mu^\nu f_\nu $.
% Here $g(z)_\mu^\nu = {1\over d} \sum_{p=-d/2}^{d/2} \cos \pa{{2\pi p\over d}(z+\mu -\nu) } $ approximates the shift operator for continuous $z$.
% The $g(z)$ form a group because $g(w)g(z)=q(w+z)$, which is a representation for periodic 1D shifts. 
For instance, \citet{rao1999learning} used Shannon-Whittaker interpolation theorem \citep{whitaker1915functions} to define continuous 1D translation and 2D rotation groups on discrete data. 
We return to this when expressing CNN as L-conv in \ref{sec:approx}. 


\paragraph{Neighborhoods as discrete tangent bundle}
$\mB$ is useful for extending differential geometry to graphs \citep{schaub2020random}. 
% The action $[\mB]_\alpha \vf = \vf_\mu - \vf_\nu$ is a discrete version of $\ro_\alpha \vf $, where $\mu$ and $\nu$ are the endpoints of edge $\alpha$.
% The graph Laplacian $\mL = \mB\mB^T$ generalizes the continuous Euclidean Laplace operator $\del^2 = \ro^\alpha \ro_\alpha $. 
% A discrete version of tangent spaces can be defined using neighborhoods of nodes.
Define the neighborhood $<\mu>=\left\{ \alpha \in \mathcal{E} \big|\mB_\alpha^\mu =-1 \right\}$ of $\vx_\mu$ as the set of outgoing edges. 
\out{
\nd{Should we try to identify $<\mu>$ with a set of vectors instead? Like $\vx_\nu -\vx_\mu$? How can we talk about $L_i\vx_0$ being in $<0>$? 
Or should we think of it as an operator? 
Which acts on a vector and yields a number? 
That is true of the transpose, as $\vx_0^T L_i^T \vf \in \mathcal{F}$. We say that $C \in <\mu>$ if $C\vf = \sum_{\alpha\in <\mu>} c^\alpha \mB_\alpha^\nu \vf_\nu  $
}
}%%%%
$<\mu>$ can be identified with $T_{\vx_\mu} \mathcal{S}$ as for $\alpha \in <\mu>$, $\mB_\alpha \vf = \vf_\mu - \vf_\nu \sim \ro_\alpha \vf $, where $\mu$ and $\nu$ are the endpoints of edge $\alpha$.
This relation becomes exact when $\mathcal{S}$ is an $n$D square lattice with infinitesimal lattice spacing.  
The set of all neighborhoods is $\mB$ itself and encodes the approximate tangent bundle $T\mathcal{S}$.
For some operator $C:\mathcal{S}\otimes\mathcal{F} \to \mathcal{F} $ acting on $\vf $ we will say $C \in <\mu>$ if its action remains within vertices connected to $\mu$, meaning 
\begin{align}
    C \in <\mu>: \qquad C\vf = \sum_{\alpha\in <\mu>} C^\alpha \mB_\alpha^\nu \vf_\nu 
\end{align}
\nd{A bit of abuse of notation... but consistent with the vector field notation $C = C^\alpha \ro_\alpha$}


\paragraph{Lift and group action}
% Define the lift via $\vx_\mu = g_\mu \vx_0$. 
% Since we chose $\vx_\mu$ to be the canonical basis (one-hot), $\vx_\nu^T\vx_\mu = \delta_\mu^\nu $. 
% Thus, we can pick $g_\mu$ such that $g_\mu^T= g_\mu^{-1}$, meaning orthogonal matrices. 
Lie algebra elements $L_i$ by definition take the origin $\vx_0$ to points close to it.
Thus, for small enough $\eta$, 
$(I+\eta L_i) \vx_0 \in <0> $ and so $[L_i  \vx_0]^T\vf=[\hat{L}_i]_0^\rho \vf_\rho = \sum_{\alpha \in <0>} 
% \Gamma_{i 0 }^\rho 
[\hat{L}_i]_0^\alpha \mB^\rho_\alpha \vf_\rho $. 
%for a set of 
The coefficients $[\hat{L}_i]_0^\alpha \in \R$ are in fact the discrete version of $\hat{L}_i$ components from \eqref{eq:dfdg-general}.  
% Define the lift via $\vx_\mu = g_\mu \vx_0$. 
For the pushforward $gL_ig^{-1}$, we define the lift via $\vx_\mu = g_\mu \vx_0$.
We require the $G$-action to preserve the topology of $\mathcal{S}$, meaning points which are close remain close after the $G$-action. 
As a result, $<\mu>$ can be reached by pushing forward elements in $<0>$.
Thus, for each $i$, $\exists \eta \ll 1 $ such that $g_\mu (I+\eta L_i) \vx_0 \in<\mu>$, meaning for a set of coefficients $ [\hat{L}_i]_\mu^\nu \in \R$ 
%$ \Gamma_{i \mu }^\rho \in \R$ 
we have
\begin{align}
    [g_\mu (I+\eta L_i) \vx_0]^T\vf & = \vf_\mu+ \eta \sum_{\alpha\in <\mu>}  
    [\hat{L}_i]_\mu^\alpha \mB_\alpha ^\nu\vf_\nu 
    %= g_\mu \pa{\vx_0+ \eps \sum_{\rho\in <0>} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}
    % \cr
    % &&
    % \Gamma_{i \mu }^\nu &= \sum_{\rho\in <0>} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho = [g_\mu]^\nu_\rho \Gamma_{i 0 }^\rho
\end{align}
where $\vf_\mu = \vx_\mu^T\vf $.
% Multiplying from the left by $\vx_\nu^T$ to obtain $\vx^T_\nu g_\mu L_i\vx_0 = [g_\mu L_i\vx_0]^\nu $ and 
Acting with $[g_\mu L_i \vx_0]^T\vx_\nu $ and 
inserting $I= \sum_\rho \vx_\rho \vx_\rho^T$ we have 
\begin{align}
    [g_\mu L_i\vx_0]^\nu &= 
    % \Gamma_{i \mu }^\nu 
    [\hat{L}_i]_\mu^\alpha \mB_\alpha^\nu  
    = \sum_{\rho} [g_\mu\vx_\rho \vx^T_\rho L_i \vx_0]^T\vx_\nu
    \cr & = \sum_{\rho\in <0>}  [L_i]_0^\rho [\vx_\nu^T g_\mu\vx_\rho]^T
    = [L_i]_0^\rho [g_\mu]^\nu_\rho = [\hat{L}_i]_0^\alpha \mB_\alpha^\rho [g_\mu]^\nu_\rho
    \label{eq:hat-L-discrete}
\end{align}
This $\hat{L}_i \equiv \hat{L}_i^\alpha \mB_\alpha $ is the discrete $\mathcal{S}$ version of the vector field $\hat{L}_i(\vx) = [g L_i \vx_0]^\alpha \ro_\alpha $ in \eqref{eq:dfdg-general}.



\paragraph{Lie Algebra Convolutional Layer}
% \begin{figure}
%     \centering
\begin{wrapfigure}{r}{.45\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, this action is analogous to a Graph Convolutional Network with $d$ nodes and $m_l$ features per node. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-30pt}
\end{wrapfigure}
% \end{figure}

In conclusion, the discrete space L-conv \eqref{eq:L-conv-tensor0} can be rewritten using the global Lie algebra basis $\hat{L}_i$
\begin{align}
    % \mbox{L-conv}:\  
    Q[\vf] &=   \pa{\vf + \hat{L}_i\vf \ba{\eps}^i} W^{0T} \cr 
    Q[\vf]_\mu^a &= \vf_\mu^b [W^{0T}]_b^a + 
    [\hat{L}_i]_\mu^\nu \vf_\nu^c \br{W^i}^a_c
    \label{eq:L-conv-tensor}
\end{align}
Where $W^i=W^0\ba{\eps}^i$, $W^0 \in \R^{m_{in}}\otimes \R^{m_{out}}$ and $\ba{\eps}^i \in \R^{m_{in}}\otimes \R^{m_{in}}$ are trainable weights. 
The $\hat{L}_i$ can be either inserted as inductive bias or they can be learned to discover symmetries. % we will be learning $\hat{L}_i$. 
% We will discuss learning symmetries
We derived L-conv from G-conv using kernels around identity. 


\paragraph{Nonlinear activation}
% Regarding nonlinear activation functions, as discussed in \nd{cite prior work}, it depends on whether they commute with the group action. 
% When $G$ is not a Lie group, many point-wise nonlinearities can preserve it. 
% As many nonlinear activation functions are not compatible with equivariance. 
% Note that, similar to discussion in
As noted in \cite{weiler20183d}, an arbitrary nonlinear activation $\sigma $ may not keep the architecture equivariant under $G$, but linear activation remains equivariant.

\nd{Vector field plots of $\hat{L}_i$ in experiments.
Apply orthogonality with $B_{ij} = 2k\Tr{l_il_j}-2\Tr{l_i}\Tr{l_j}=$ }


\out{
In particular, for a fixed $i$ and $\eps\ll 1$, we have 
\begin{align}
    \vx_i &= (I+\eps L_i) \vx_\mu = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu \in <\mu> \\
    [L_i]^\nu_\mu &= \vx_\nu^T L_i \vx_\mu = {1\over \eps }\pa{\vx_\nu^T\vx_i- \delta^\nu_\mu}= \mA_{\mu\nu}\Gamma_{i\mu}^\nu
    % \vx_\nu^T\vx_i &= \delta^\nu_\mu + \eps [L_i]^\nu_\mu = \delta^\nu_\mu + \eps \mA_{\mu\nu}[l_i]^\nu 
\end{align}
Next, we note that writing $g_\mu = P\exp[\int_\gamma dt^iL_i]$ we can use the Lie algebra $[L_i,L_j={c_{ij}}^kL_k$ to pass $L_i$ through

Let $(I+\eps L_i) \vx_0 \in <0> $ for small $\eps \ll 1$. 
The continuity of $G$ action means that for each $i$, $\exists \eps \ll 1 $ such that $g_\mu (I+\eps L_i) \vx_0 \in<\mu>$. 
Therefore
\begin{align}
    (I+\eps L_i) \vx_0& = \vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho \cr
    g_\mu (I+\eps L_i) \vx_0& = \vx_\mu+ \eps \sum_{\nu\ne \mu} \mA_{\mu\nu} \Gamma_{i \mu }^\nu \vx_\nu = g_\mu \pa{\vx_0+ \eps \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\rho}\cr
    \mA_{\mu\nu} \Gamma_{i \mu }^\nu   \sum_{\rho\ne 0} \mA_{0\rho} \Gamma_{i 0 }^\rho \vx_\nu^T g_\mu\vx_\rho
\end{align}

This means that any small $v_\eps = I+\eps^iL_i \in T_IG$ must move points $\vx_\mu$ within their neighborhood, meaning for $v_\eps = I+\eps^iL_i \in G$ close to identity and $\vx_\mu \in \mathcal{S}$ we have
\begin{align}
    % \forall v_\eps &= I+\eps^iL_i \in G, \quad \forall\vx_\mu \in \mathcal{S},\quad 
    &\exists c\in \R^d, & v_\eps \vx_\mu &= \sum_\nu c^\nu \mA_{0\nu}\vx_\nu \in <\mu >. 
    \label{eq:G-neigh-preserve}
\end{align}
}%%%

% Next, we establish relations between L-conv and other commonly used architectures. 




==> secs2/theory-bkp-2021-07-16.tex <==


% \ry{Show a picture of generation in a set, made with mathematical \href{https://keenan.is/illustrating/2017/03/03/illustrating-lie-groups/}{Illustration}}
% \subsection{Continuous Symmetry, Lie Groups and Lie Algebras}
% \nd{Shorten}
% We will focus on Lie groups that are subsets $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group in $d$ dimensions.
% Our results generalize trivially to other number fields such as $\C$. 
% For any Lie group $G\subset \mathrm{GL}_d(\R)$,

\section{Lie Algebra Convolutional Network}
We now use the Lie algebra to expand G-conv near identity of the group. 
This yields basic building blocks from which an arbitrary G-conv can be constructed.  
% is to instead approximate $\kappa(v)$ utilizing the Lie algebra.
% \subsection{Expanding in G-conv in the Lie algebra}
We consider a G-conv \eqref{eq:G-conv} with a kernel localized near identity $I$. 
Let $\kappa_0 (u) = c \delta_\eta (u)$, with constants $c\in \R^{m'} \otimes \R^{m}$ and a normalized kernel $\delta_\eta(u) \in \R$ %which has 
with support on an $\eta$ neighborhood of $I$, meaning $\delta_\eta(I+\eps^iL_i) \to 0 $ if $\|\eps\|^2>\eta^2$.

\paragraph{L-conv derivation}
Let us consider what happens if the kernel in G-conv \eqref{eq:G-conv} is localized near identity. 
Let $\kappa_I (u) = c \delta_\eta (u)$, with constants $c\in \R^{m'} \otimes \R^{m}$ and kernel $\delta_\eta(u) \in \R$ which has support only on on an $\eta$ neighborhood of identity, meaning $\delta_\eta(I+\eps^iL_i) \to 0 $ if $|\eps|>\eta$.
This allows us to expand G-conv in the Lie algebra of $G$ to linear order. 
With $v_\eps = I+\eps^i L_i $, we have
% $\delta_\eta \star f$ may be expanded  near identity as


\textbf{Lie algebra convolutional (L-conv) layer}
\ry{simplify the notations} We can expand a G-conv whose kernel is $\kappa_0$ in the Lie algebra of $G$ to linear order to obtain the L-conv architecture 
(see SI \ref{ap:theory-extended}, \eqref{eq:L-conv-basic})
\begin{align}
    Q[f](g)&=[\kappa_0 \star f](g) 
    = \int_G dv \kappa_0 (v) f(gv )
    =\int_{\|\eps\| <\eta } dv_\eps  \delta_\eta (v_\eps) f(gv_\eps )\cr
    % &= \int d\eps \delta_\eta (I+\eps^i L_i) f(g(I+\eps^i L_i))\cr
    % &= \int d\eps \delta_\eta (I+\eps^i L_i) f(g+\eps^i gL_i)\cr
    &
    = \int d\eps \kappa_0 (I+\eps^i L_i) \br{f(g)+ \eps^i g L_i \cdot {d\over dg}  f(g) + O(\eps^2) } %\bigg|_{u\to g}
    \cr
    % &\approx \int d\eps \kappa_0 (I+\eps^i L_i) \br{I+ \eps^i g L_i \cdot {d\over dg} } f(g)
    % \cr
    & \approx W^0\br{I + \ba{\eps}^i g L_i\cdot {d\over dg} } f(g)
    \label{eq:L-conv-basic} 
\end{align}

\ry{explain the Taylor expansion in (25)}
% $\delta_\eta \star f$ may be expanded  near identity as
\begin{align}
    Q[f](g)&\equiv c[\delta_\eta \star f](g) 
    = %\approx
    c\int d\eps \delta_\eta (I+\eps^i L_i) \br{I+ \eps^i g L_i \cdot {d\over dg} } f(g) %\bigg|_{u\to g}
    +O(\eta^2)
    \cr
    &= W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }f(g) +O(\eta^2)\cr 
    &= [W^0]_b f^a\pa{g\pa{I+ [\ba{\eps}^i]_a^b L_i}} +O(\eta^2)
    \label{eq:L-conv}
    % = \br{W^0 + W^i g L_i\cdot {d\over dg} } f(g)
    % \label{eq:L-conv-basic} 
\end{align}
where $d\eps $ is the integration measure on the Lie algebra induced by the Haar measure $dv$ on $G$.
% where we used the fact that the Haar measure $dv$ induces an integration measure on the Lie algebra, which we denoted by $d\eps$.
In a matrix representation of $G$, we have $g L_i\cdot {df\over dg} = [g L_i]_\alpha^\beta {df\over dg_\alpha^\beta} = \Tr{[g L_i]^T {df\over dg} }$.
% $g L_i\cdot {df\over dg} = \sum_{a,b}[g L_i]_{ab} {df\over dg_{ab}} = \Tr{[g L_i]^T {df\over dg} }$.
% Note that in $g(I+\eps^iL_i)\vx_0$, the $gL_i\vx_0 = \hat{L}_i(g)\vx$ come from the pushforward $L_i^{(g)}=gL_ig^{-1} \in T_gG$.
%of $L_i\in T_IG$ from the tangent space at $I$ to the tangent space at $g$, meaning $gL_ig^{-1} \in T_gG$. 
% This is seen from the fact that $gv_\eps$ is moving from $g$ by $\eps L_i$, hence in $T_gG$. 
% We will show this explicitly in following examples. 
% \Eqref{eq:L-conv-basic} is the core of the architecture we are proposing, the Lie algebra convolution or \textbf{L-conv}.
\ry{formally define a L-conv layer, put Equation 10 here}



\out{
\textbf{L-conv Layer} 
In general, we define Lie algebra convolution (L-conv) as follows \begin{align}
    Q[f](g)&= \br{W^0 + W^i g L_i\cdot {d\over dg} } f(g) = W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }f(g) \cr 
    &= [W^0]_b f^a\pa{g\pa{I+ [\ba{\eps}^i]_a^b L_i}} +O(\ba{\eps}^2)
    \label{eq:L-conv-def0}
\end{align}
where
}%%%%
% For $f(g)\in \R^m $, 
Here 
\begin{align}
    W^0 &= %\int_G dv \kappa_0(v) = 
    c \int d\eps \delta_\eta (I+\eps^iL_i) \in \R^{m'} \otimes \R^m, &
    \ba{\eps}^i &= \int d\eps \delta_\eta (I+\eps^iL_i) \eps^i \in \R^{m} \otimes \R^m
\end{align}
with $\|\ba{\eps}\|<\eta $.
% For brevity, we define $W^i\equiv W^0 \ba{\eps}^i$.
% , and found using the Moore-Penrose inverse $\tilde{W}_0^{-1} = (W^{0T}W^0)^{-1}W^0$. 
Being an expansion of G-conv, L-conv is also equivariant.

\begin{proposition}[Equivariance of L-conv]\label{prop:L-conv-equiv}
    With assumptions above,
    L-conv is equivariant to  $O(\eta^2)$. 
\end{proposition}
\begin{proof}
    From \eqref{eq:L-conv} it follows that L-conv is equivariant up to $O(\ba{\eps}^2) \sim O(\eta^2)$, as for $w\in G$
\begin{align}
    w\cdot Q[f](g)&= Q[f](w^{-1}g) 
    = W^0 f\pa{w^{-1} g\pa{I+ \ba{\eps}^i L_i}} +O(\eta^2)
    %= W^0 w \cdot f\pa{ g v_\eps} 
    = Q[w\cdot f](g).
    \label{eq:L-conv-equiv}
\end{align}
\end{proof}
% \ry{make this a prop}
% \textbf{Equivariance of L-conv}


\subsection{Interpretation and Examples \label{sec:interpret-continuous} }
% \paragraph{General case} 
The $gL_i\cdot df/dg$ in \eqref{eq:L-conv} can be written in terms of partial derivatives $\ro_\alpha f(\vx) = \ro f/\ro \vx^\alpha$. 
In general, using $\vx^\rho = g^\rho_\sigma \vx_0^\sigma$, we have ${df(g\vx_0)\over dg^\alpha_\beta} =\vx_0^\beta \ro_\alpha f(\vx) $, and so
% \ry{add a cartoon}
\begin{align}
    % \vx^\mu &= g^\rho_\sigma \vx_0^\sigma &
    % {df(g\vx_0)\over dg^\alpha_\beta}
    % &= {d(g^\rho_\sigma \vx_0^\sigma) \over dg^\alpha_\beta}\ro_\rho f(\vx) = \vx_0^\beta \ro_\alpha f(\vx)
    % \label{eq:dgx0-dg}
    % \\
    gL_i\cdot {df\over dg} &= [gL_i]^\alpha_\beta \vx_0^\beta \ro_\alpha f(\vx) = [gL_i\vx_0]\cdot \del f(\vx) = \hat{L}_if(\vx)
    \label{eq:dfdg-general}
\end{align}
Hence, for each $L_i$, the pushforward $gL_i$ generates a flow on $\mathcal{S}$ through the vector field $\hat{L}_i\equiv gL_i\cdot d/dg = [gL_i\vx_0]^\alpha \ro_\alpha$ (Fig. \ref{fig:Lie-group-S}). 
% $\hat{L}_i$ is related to the Maurer-Cartan form $\omega = g^{-1} \ro_\alpha g d\vx^\alpha$, which encodes the pushforward.
% Write $f(gv_\eps) = f(g+ \eta(\eps)^\alpha \ro_\alpha g)$. 
% We have $ \eta^\alpha \ro_\alpha g = \eps^i g L_i$, so $ \eps^i L_i \eta^\alpha g^{-1} \ro_\alpha g = \eta \cdot \omega $.
% The Maurer-Cartan form defines a way to parallel transport (pushforward) and define a basis frame on  
% Vector fields are sections of the tangent bundle $T\mathcal{S}$.
% We will encounter $gL_i\vx_0$ again on a discretized $T\mathcal{S}$ again below. 
Being a vector field $\hat{L}_i\in T\mathcal{S}$ (i.e. 1-tensor), $\hat{L}_i$ is basis independent, meaning 
for $v \in G$, $\hat{L}_i(v\vx) = \hat{L}_i$. 
Its components transform as $[\hat{L}_i(v \vx)]^\alpha =[vgL_i\vx_0]^\alpha = v^\alpha_\beta \hat{L}_i(\vx)^\beta $, while the partial transforms as $\ro / \ro[v\vx]^\alpha = [v^{-1}]^{\gamma}_\alpha \ro_\gamma$. 

\paragraph{Explicit examples}
Using \eqref{eq:dfdg-general} we can calculate the form of L-conv for specific groups (details in SI \ref{ap:examples-continuous}). 
For \textbf{translations} $G=T_n = (\R^n,+)$ we find the generators become simple partial derivatives $\hat{L}_i = \ro_i$ (SI \ref{ap:example-Tn}), yielding $f(\vx) + \eps^\alpha \ro_\alpha f(\vx)$. 
For \textbf{2D rotations} (SI \ref{ap:example-so2}) 
we find $\hat{L} \equiv \pa{x \ro_y - y \ro_x } = \ro_\theta$, which in physics is called the angular momentum operator about the z-axis in quantum mechanics and field theories. %, which generates rotations around the $z$ axis. 
For rotatons with scaling, 
\textbf{Rotation and scaling} $G= SO(2)\times \R^+$, 
we have two $L_i$, one $\hat{L}_\theta=\ro_\theta $ from $so(2)$ and a scaling with $L_r = I$, yielding
$\hat{L}_r = x\ro_x+y\ro_y= r\ro_r $. % (SI \ref{ap:examples-continuous}) 
Next, we discuss the form of L-conv on discrete data. 


\subsection{Approximating G-conv using L-conv \label{sec:G-conv2L-conv} }
\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figs2/G-conv2L-conv.pdf}
    \caption{
    Sketch of the procedure for approximating G-conv using L-conv. 
    First, the kernel is written as the sum of a number of localized kernels $\kappa_k$ with support around $u_k$ (left). 
    Each of the $\kappa_k$ is then moved toward identity by composing multiple L-conv layers $Q_{\eps'}\circ Q_\eps\dots \kappa_k $ (right). 
    % The more layers used, the more accurate the 
    }
    \label{fig:G-conv2L-conv}
\end{figure}

L-conv can be used as a basic building block which can be combined to make more G-conv with more general kernels. 
Figure \ref{fig:G-conv2L-conv} sketches the argument described here (see SI \ref{ap:G-conv2L-conv} for more discussion).
\begin{theorem}[G-conv from L-convs]
    G-conv \eqref{eq:G-conv} can be approximated using L-conv layers.
\end{theorem}
\begin{proof}
    The procedure involves two steps, as illustrated in Fig. \ref{fig:G-conv2L-conv}: 1) approximate the kernel using localized kernels as the $\delta_\eta$ in L-conv; 2) move the kernels towards identity using multiple L-conv layers. 
    The following lemma outline the details.
\end{proof}

% To do so, we first note that any function $\kappa(v)$ can be approximated to arbitrary accuracy using a set of local kernels $\delta_\eta $ (using the universal approximation theorem of neural networks \citep{hornik1989multilayer,cybenko1989approximation}).

\begin{lemma}[Approximating the kernel]
    Any kernel $\kappa$ can be approximated using a set of kernels with $\eta$ support to arbitrary accuracy. 
\end{lemma}
% \textbf{Approximating the kernel}
\begin{proof}
This simply follows from the universal approximation theorem for neural networks \citep{hornik1989multilayer,cybenko1989approximation} and the same approximation errors apply. 
$\delta_\eta(g)$ can be written as the sum of two sigmoid functions 
$\delta_\eta(g) =\mathrm{sig}(v_\eta g)+\mathrm{sig}(v_\eta^{-1}g) $. 
Thus, we can approximate any kernel as $\kappa(g) \approx \sum_k \kappa_k(g)$ where the local kernels $\kappa_k (g) = c_k \delta_\eta (  u_k^{-1}g)$ have
support only on an $\eta$ neighborhood of $u_k \in G $. 
Here $c_k\in \R^{m'} \otimes \R^{m}$ are constants and $\delta_\eta(u)$ is as in \eqref{eq:L-conv}.  
Using this, G-conv \eqref{eq:G-conv} becomes
\begin{align}
    [\kappa \star f](g)
    % & = \sum_k [\kappa_k \star f](g) 
    &= \sum_k c_k \int dv \delta_\eta(u_k^{-1} v) f(gv) 
    % &= \sum_k c_k \int dv \delta_\eta(v ) f(gu_k v) 
    = \sum_k c_k [\delta_\eta \star f] (gu_k).
\end{align}
% As we showed in \eqref{eq:L-conv-basic}, $[\delta_\eta \star f](g)$ is the definition of L-conv. 
% \ry{put this as a theorem, show as an approximation error}
The kernels $\kappa_k$ are localized around $u_k$, whereas in L-conv the kernel is around identity. 
We can compose L-conv layers to move $\kappa_k$ from $u_k$ to identity. 
\end{proof}

\begin{lemma}[Moving kernels to identity]
    The local kernel $\kappa_k$ can be moved near identity. 
\end{lemma}
\begin{proof}
% \textbf{Moving kernels to identity}
The local kernels $\kappa_k(g)=\delta_\eta (gu_k)$ are nonzero around $u_k$.  
An L-conv with $W^0 = I$ performs $G[\kappa_k\star f](g)=\kappa_k\star f(gv_\eps)$, which moves the $\kappa_k$ by $v_\eps=(I+\ba{\eps}^iL_i)$ on $G$.
Thus, by applying multiple L-conv layers we can find $Q_p \circ \dots Q_1\circ \kappa_k\approx c_k\delta_\eta $. 
This can always be done using a set of $v_{\eps_a} = (I+\ba{\eps}_a^iL_i)$ such that $u_k \approx \prod_{a=1}^p v_{\eps_a}$. 
With $\|\eps_a\|<\eta$, the error in $u_k$ is $O(\eta^{p+1})$.
\end{proof}

Thus, we conclude that any G-conv \eqref{eq:G-conv} can be approximated by multilayer L-conv. 
%
% \nd{Mention/review Rao's result and how it demonstrates this theorem for 1D translation.}
We conducted small controlled experiments to verify this (SI \ref{ap:experiments}). 
We briefly discuss them here. 

\paragraph{Learning symmetries using L-conv}
\citet{rao1999learning} introduced a basic version of L-conv and showed that it can learn 1D translation and 2D rotation. 
% They showed that t
The learned 
% infinitesimal generator 
$L_i$ for 1D translation reproduced finite translation well using $(I+\eps L)^N$, which is $N$ recursive L-conv layers. 
Hence, their results prove that L-conv can be used to approximate CNN, as well as $SO(2)$ G-conv. 
We discuss the details of L-conv approximating CNN below in sec. \ref{sec:approx}.
We also conducted more complex experiments using recursive L-conv to learn large rotation angle between two images 
% \nd{revise if experiments moved to SI}
(SI \ref{ap:experiments}).
% These experiments required L-conv to approximate rotations by large angles, which it did successfully. 
% The learned $L$ also has the right structure (Fig. \ref{fig:L-so2-combined}).
\out{
% We can use L-conv for learning the Lie algebra as well. 
% In fact, the architecture used in \citet{rao1999learning} is a basic version of L-conv with $W^0 = 1$. 
They show that with a small fixed $\ba{\eps^i}$ they could learn learn the single $L_i$ for continuous 1D translations and for 2D rotations.
Indeed, the architecture used in \citet{rao1999learning} is a special case of L-conv with $W^0 = 1$ and $\ba{\eps}^i\in \R$. 
We conducted a more advanced experiment with L-conv learning rotation angles in pairs of random images (SI \ref{ap:exp-L-multi})
}%
% experiments for with $G=SO(2)$.
% In the first test, we used fixed small rotation angle $\pi/10$ and used 
Figure \ref{fig:L-so2-combined} shows the learned $L$. 
Left shows $L\in so(2)$ learned using L-conv in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
Middle and right of Fig. \ref{fig:L-so2-combined} are experiments with fixed small rotation angle $\theta = \pi/10$ (SI \ref{ap:exp-L-small}).
Middle is the $L$ learned using L-conv and right is using the exact solution $R = (YX^T)(X^TX)^{-1}$. 
While the middle $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
% Right shows the generator calculated using the exact solution to the linear regression problem with $\theta = \pi/10$. 
% The SGD solutions using L-conv are less noisy and capture more details.
(also see SI \ref{ap:experiments} for a discussion on symmetry discovery literature.)

L-conv can potentially replace other equivariant layers in an architectures.
We conducted limited experiments for this on small image datasets (SI \ref{ap:exp-image}). 
L-conv allows one to look for potential symmetries in data which may have been scrambled or harbors hidden symmetries. 
Next, we will provide some examples of explicit forms of L-conv.

\begin{figure}
    \centering
    \includegraphics[width=.17\linewidth]{figs2/L-conv-recur-3.pdf}
    \includegraphics[width=.82\linewidth]{figs2/L-so2-combined.pdf}
    \caption{
    \textbf{Learning the infinitesimal generator of $SO(2)$} 
    Left shows the architecture for learning rotation angles between pairs of images (SI \ref{ap:exp-L-multi}). 
    Next to it is the $L$ learned using recursive L-conv in this experiment. %to learn rotation angle between pairs of images.  
    %in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
    Middle $L$ is learned using a fixed small rotation angle $\theta = \pi/10$, and
    % While this $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
    right shows $L$ found using the numeric solution from the data. 
    % The SGD solutions using L-conv are less noisy and capture more details.
    }
    \label{fig:L-so2-combined}
\end{figure}

\out{
\nd{Add our own experiments here.}
\paragraph{Symmetry Discovery Literature}
In addition to simplifying the construction of equivariant architectures, our method can also learn the symmetry generators from data. 
Learning symmetries from data has been studied before, but mostly in restricted settings.
Examples include commutative Lie groups as in \citet{cohen2014learning}, 2D rotations and translations in 
\citet{rao1999learning}, \citet{sohl2010unsupervised} or permutations \citep{anselmi2019symmetry}. 
% Perhaps the closest to our work, in spirit, is 
\citet{zhou2020meta} uses meta-learning to automatically learn symmetries in the data. 
% \citet{zhou2020meta} is about defining a weight-sharing scheme to decompose the weights of a fully-connected layer and not group convolution as in our work. 
Yet their weight-sharing scheme and the encoding of the symmetry generators is very different from ours. % (see appendix \ref{ap:compare} for detailed discussion). 
% \ry{do we compare with them?} 
% Also their use of Kronecker factorization to sparsify the symmetry matrix restricts the symmetries to be local and, thus, introduces bias.
% Assuming a discrete group $G=\{g_1,\dots, g_n\}$, they decompose the weights $W\in \R^{s\times s}$ of a fully-connected layer, acting on $\vx \in \R^s$ as $\mathrm{vec}(W) = U^Gv$ where $U^G\in \R^{s\times s}$ are the ``symmetry matrices'' and $v\in \R^s$ are the ``filter weights''. 
% Then they use meta-learning to learn $U^G$ and during the main training keep $U^G$ fixed and only learn $v$.
% We may compare MSR to our approach by setting $d=s$. 
% First, note that although the dimensionality of $U\in \R^{nd\times d}$ seems similar to our $L \in \R^{n\times d\times d}$, the $L_i$ are $n$ matrices of shape $d\times d$, whereas $U$ has shape $(nd) \times d$ with many more parameters than $L$. 
% Also, the weights of L-conv $W\in \R^{n\times m_l \times m_{l-1}}$, with $m_l$ being the number of channels, are generally much fewer than MSR filters $v\in \R^d$. 
% Finally, the way in which $Uv$ acts on data is different from L-conv, as the dimensions reveal.
% The prohibitively high dimensionality of $U$ requires MSR to adopt a sparse-coding scheme, mainly Kronecker decomposition.
% Though not necessary, we too choose to use a sparse format for $L_i$, finding that very low-rank $L_i$ often perform best. 
% A Kronecker decomposition may bias the structure of $U^G$ as it introduces a block structure into it.
% In a concurrent work,
\citep{benton2020learning} propose Augerino, a method to learn equivariance with neural networks, but restricted to
% Augerino uses data augmentation to transform the input data, which means it is restricting the group to be  
a subgroup of the augmentation transformations. 
% Augerino learns which subset of the augmentations improved the prediction. 
% This is done by writing 
% The data augmentation is written as $g_\eps = \exp\pa{\sum_i \eps_i \theta_i L_i} $ (equation (9) in \cite{benton2020learning}), with randomly sampled $\eps_i\in [-1,1]$. 
% $\theta_i$ are trainable weights which determine which $L_i$ helped with the learning task. 
% Furthermore, 
Their Lie algebra is fixed to affine transformations in 2D (translations, rotations, scaling and shearing). 
% In contrast, 
Our approach is more general.  
We learn the $L_i$ directly without restricting to known symmetries. % them to be a known set of generators.  
Additionally, we do not use the exponential map or matrix logarithm, hence, our method is easy to implement.  
Lastly, Augerino uses sampling to effectively cover the space of group transformations. 
Since we work with the Lie algebra rather the group itself, we do not require sampling.
%and only need to learn a basis for the Lie algebra, which generally a small number of Lie algebra elements.
% The main differences with our approach 
% , which mean they are assuming the group to be a subgroup of their augmentation transformations. 
% Specifically, they assume the group to be affine transformations and learn which sub-group of it is used in the dataset. 
% In eq. 9, the $G_i$ (equivalent to our $L_i$) are the generators of affine transformations and the state below eq. 9 the $G_1,...G_6$ are predefined translations, rotations, scaling and shearing.  
% In contrast, we are learning $L_i$ and do not restrict them to a known set of generators. 






Next, we will provide some examples.
% implementation details and relations with physics.
% implementation details of L-conv and how it relates to other architectures such as CNN \citep{lecun1989backpropagation} and graph convolutional networks (GCN) \citep{kipf2016semi}.  
}


\subsection{Interpretation and Examples \label{sec:interpret-continuous} }
% \paragraph{General case} 
The $gL_i\cdot df/dg$ in \eqref{eq:L-conv} can be written in terms of partial derivatives $\ro_\alpha f(\vx) = \ro f/\ro \vx^\alpha$. 
In general, using $\vx^\rho = g^\rho_\sigma \vx_0^\sigma$, we have ${df(g\vx_0)\over dg^\alpha_\beta} =\vx_0^\beta \ro_\alpha f(\vx) $, and so
% \ry{add a cartoon}
\begin{align}
    % \vx^\mu &= g^\rho_\sigma \vx_0^\sigma &
    % {df(g\vx_0)\over dg^\alpha_\beta}
    % &= {d(g^\rho_\sigma \vx_0^\sigma) \over dg^\alpha_\beta}\ro_\rho f(\vx) = \vx_0^\beta \ro_\alpha f(\vx)
    % \label{eq:dgx0-dg}
    % \\
    gL_i\cdot {df\over dg} &= [gL_i]^\alpha_\beta \vx_0^\beta \ro_\alpha f(\vx) = [gL_i\vx_0]\cdot \del f(\vx) = \hat{L}_if(\vx)
    \label{eq:dfdg-general}
\end{align}
Hence, for each $L_i$, the pushforward $gL_i$ generates a flow on $\mathcal{S}$ through the vector field $\hat{L}_i\equiv gL_i\cdot d/dg = [gL_i\vx_0]^\alpha \ro_\alpha$ (Fig. \ref{fig:Lie-group-S}). 
% $\hat{L}_i$ is related to the Maurer-Cartan form $\omega = g^{-1} \ro_\alpha g d\vx^\alpha$, which encodes the pushforward.
% Write $f(gv_\eps) = f(g+ \eta(\eps)^\alpha \ro_\alpha g)$. 
% We have $ \eta^\alpha \ro_\alpha g = \eps^i g L_i$, so $ \eps^i L_i \eta^\alpha g^{-1} \ro_\alpha g = \eta \cdot \omega $.
% The Maurer-Cartan form defines a way to parallel transport (pushforward) and define a basis frame on  
% Vector fields are sections of the tangent bundle $T\mathcal{S}$.
% We will encounter $gL_i\vx_0$ again on a discretized $T\mathcal{S}$ again below. 
Being a vector field $\hat{L}_i\in T\mathcal{S}$ (i.e. 1-tensor), $\hat{L}_i$ is basis independent, meaning 
for $v \in G$, $\hat{L}_i(v\vx) = \hat{L}_i$. 
Its components transform as $[\hat{L}_i(v \vx)]^\alpha =[vgL_i\vx_0]^\alpha = v^\alpha_\beta \hat{L}_i(\vx)^\beta $, while the partial transforms as $\ro / \ro[v\vx]^\alpha = [v^{-1}]^{\gamma}_\alpha \ro_\gamma$. 

\paragraph{Explicit examples}
Using \eqref{eq:dfdg-general} we can calculate the form of L-conv for specific groups (details in SI \ref{ap:examples-continuous}). 
For \textbf{translations} $G=T_n = (\R^n,+)$ we find the generators become simple partial derivatives $\hat{L}_i = \ro_i$ (SI \ref{ap:example-Tn}), yielding $f(\vx) + \eps^\alpha \ro_\alpha f(\vx)$. 
For \textbf{2D rotations} (SI \ref{ap:example-so2}) 
we find $\hat{L} \equiv \pa{x \ro_y - y \ro_x } = \ro_\theta$, which in physics is called the angular momentum operator about the z-axis in quantum mechanics and field theories. %, which generates rotations around the $z$ axis. 
For rotatons with scaling, 
\textbf{Rotation and scaling} $G= SO(2)\times \R^+$, 
we have two $L_i$, one $\hat{L}_\theta=\ro_\theta $ from $so(2)$ and a scaling with $L_r = I$, yielding
$\hat{L}_r = x\ro_x+y\ro_y= r\ro_r $. % (SI \ref{ap:examples-continuous}) 
Next, we discuss the form of L-conv on discrete data. 


\section{Tensor notation \label{sec:tensor} }
% If the dataset being analyzed is in the form of $f(\vx)$ for some sample of points $\vx$, together with derivatives $\del f(\vx) $, we can use the L-conv formulation above. 
% However, i
\begin{wrapfigure}{r}{.45\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \vspace{-40pt}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, L-conv is analogous to a Graph Convolutional Network with $d$ nodes and $m_{in}$ features. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-20pt}
\end{wrapfigure}


In many datasets, such as images, $f(\vx)$ is not given as continuous function, but rather as a discrete array, with %$\vx$ taking values over a grid. 
% In this case all the discussions above still hold, as discuss now. 
% In particular, e
% Let 
$\mathcal{S}= \{\vx_0,\dots \vx_{d-1}\}$ containing $d$ points. 
Each $\vx_\mu$ represents a coordinate in higher dimensional space,
% For instance, 
e.g. on a $10\times 10$ image, $\vx_0$ is $(x,y)=(0,0)$ point and $ \vx_{99}$ is $(x,y) =(9,9)$.

\textbf{Feature maps and group action}
In the tensor notation, we encode $\vx_\mu \in \mathcal{S}$ as the canonical basis (one-hot) vectors in $\vx_\mu \in \R^d$ with 
% To define features $f(\vx_\mu)\in \R^m$ for $\vx_\mu \in \mathcal{S}$, we embed $\vx_\mu \in \R^d$ and 
% encode them as the canonical basis (one-hot) vectors with components 
$[\vx_\mu]_\nu = \delta_{\mu\nu}$ (Kronecker delta), e.g. $\vx_0 = (1,0,\dots, 0)$.
The features become $\vf \in \mathcal{F}= \R^d \otimes \R^m $, meaning 
% feature maps $\vf \in \mathcal{F}$ are 
$d\times m$ tensors, with $f(\vx_\mu) = \vx_\mu^T \vf = \vf_\mu $.
%
% \paragraph{Group action}
% \nd{Change to $\vx_\mu^T g^T$ for less confusion.}
Although $\mathcal{S}$ is discrete, the group acting on $\mathcal{F}$ can be continuous (e.g. image rotations). 
Any $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group (invertible $d\times d$ matrices) acts on $\vx_\mu \in \R^d$ and $\vf\in \mathcal{F}$. 
% Since $\vx_\mu \in \R^d$, $g \in G$ also naturally act on $\vx_\mu$. 
% The resulting 
% Note $\vy = g \vx_\mu \notin  \mathcal{S}$ is a linear combination $\vy = c^\nu \vx_\nu$ of elements in $\mathcal{S}$, not a single element.
% The action of $G$ on $\vf$ and $\vx$, can be defined in multiple equivalent ways.
% The most elegant one is if w
We define $f(g \cdot \vx_\mu) = \vx_\mu^T g^T\vf, \forall g\in G$, so that
% consistent with the lift. 
% This makes the group action on $\vf$ the natural action of $G$, meaning 
for $w\in G$ we have 
\begin{align}
    w\cdot f(\vx_\mu)&= f(w^{-1}\cdot \vx_\mu) = \vx_\mu^T w^{-1T}\vf = %\vx_\mu^T [w^T]^{-1} \vf = 
    [w^{-1}\vx_\mu]^T \vf
    \label{eq:G-action-tensor-T}
\end{align}
Dropping the position $\vx_\mu$, the transformed features are matrix product $w\cdot \vf= w^{-1T}\vf$. 


\paragraph{G-conv and L-conv in tensor notation} 
Writing G-conv \eqref{eq:G-conv} in the tensor notation we have 
\begin{align}
    [\kappa\star f](g\vx_0) = \int_G \kappa(v)f(gv\vx_0) dv = \vx_0^T \int_G v^{T} g^{T} \vf \kappa^T(v) dv 
    \equiv \vx_0^T [\vf \star \kappa](g) 
    \label{eq:G-conv-tensor}
\end{align}
where we moved $\kappa^T(v) \in \R^m \otimes \R^{m'}$ to the right of $\vf$ because it acts as a matrix on the output index of $\vf$.
The equivariance of \eqref{eq:G-conv-tensor} is readily checked with $w\in G$
\begin{align}
    w\cdot [\vf \star \kappa](g) & = [\vf \star \kappa](w^{-1}g) 
    % = \int_G v^{T} [w^{-1}g]^{T} \vf \kappa^T(v) dv %\cr &
    = \vx_0^T \int_G v^{T} g^T w^{-1T} \vf \kappa^T(v) dv %\cr &
    %= \int_G v^{-1} g^{-1} w\vf \kappa^T(v) dv 
    % = [w^{-1T} \vf \star \kappa](g)
    = [(w\cdot\vf) \star \kappa](g)
\end{align}
where we used $[w^{-1}g]^{T}\vf = g^{T} w^{-1T}\vf $.
Similarly, we can rewrite L-conv \eqref{eq:L-conv} in the tensor notation. 
Defining $v_\eps =I+ \ba{\eps}^i L_i $ 
\begin{align}
    Q[\vf](g) 
    &= W^0 f\pa{g\pa{I+ \ba{\eps}^i L_i}} 
    = \vx_0^T \pa{I+ \ba{\eps}^i L_i}^{T} g^{T} \vf W^{0T} \cr
    % &= \vx_0^T \pa{I+ \ba{\eps}^i L_i^T} g^{T} \vf W^{0T} \cr 
    &= \pa{\vx+ \ba{\eps}^i [gL_i\vx_0]}^T \vf W^{0T}.
    % = \br{\vf_\mu + \ba{\eps}^i [gL_i \vf]_\mu }W^{0T} 
    % \cr
    \label{eq:L-conv-tensor}
\end{align}
Here, $\hat{L}_i=gL_i\vx_0$ is eactly the tensor analogue of pushforward vector field $\hat{L}_i$ in \eqref{eq:dfdg-general}. 
We will make this analogy more precise below.
The equivariance of L-conv in tensor notation is again evident from the $g^T \vf$, resulting in 
\begin{align}
    Q[w\cdot \vf](g) &= \vx_0^Tv_\eps^T g^T w^{-1T} \vf W^{0T}= Q[\vf](w^{-1}g) = w\cdot Q[\vf](g)
    \label{eq:L-conv-equiv-tensor}
\end{align}


\paragraph{Lie Algebra Convolutional Layer}
\out{
% \begin{figure}
%     \centering
\begin{wrapfigure}{r}{.45\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, this action is analogous to a Graph Convolutional Network with $d$ nodes and $m_l$ features per node. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-50pt}
\end{wrapfigure}
% \end{figure}
}
In conclusion, the discrete space L-conv \eqref{eq:L-conv-tensor0} can be rewritten using the global Lie algebra basis $\hat{L}_i$
\begin{align}
    % \mbox{L-conv}:\  
    Q[\vf] &=   \pa{\vf + \hat{L}_i\vf \ba{\eps}^i} W^{0T}, & %\cr 
    Q[\vf]_\mu^a &= \vf_\mu^b [W^{0T}]_b^a + 
    [\hat{L}_i]_\mu^\nu \vf_\nu^c \br{W^i}^a_c
    \label{eq:L-conv-tensor-final}
\end{align}
Where $W^i=W^0\ba{\eps}^i$, $W^0 \in \R^{m_{in}}\otimes \R^{m_{out}}$ and $\ba{\eps}^i \in \R^{m_{in}}\otimes \R^{m_{in}}$ are trainable weights. 
The $\hat{L}_i$ can be either inserted as inductive bias or they can be learned to discover symmetries. % we will be learning $\hat{L}_i$. 
% We will discuss learning symmetries
% We derived L-conv from G-conv using kernels around identity. 



\paragraph{Discrete vector field and tangent bundle}
We can show (SI \ref{ap:L-conv-tensor-interpret}) that when $\mathcal{S}$ has a topology $\hat{L}_i= g L_i\vx_0 $ is indeed the discrete version of the $\hat{L}_i$ in \eqref{eq:dfdg-general}. 
The topology, to lowest order, using a graph (1-simplex) is encoded as an
% Instead of the commonly used graph adjacency matrix $\mA$, we will use 
incidence matrix $\mB:\mathcal{S}\times  \mathcal{E}\to \{0,1,-1\}$
with vertices $\mathcal{S}$ and edge set $\mathcal{E}$. 
$\mB^\mu_\alpha=1$ or $-1$ if edge $\alpha$ starts or ends at node $\mu$, respectively, and $\mB^\mu_\alpha=0$ otherwise. % (undirected graphs have pairs of incoming and outgoing edges ).
% Similar to the continuous case we will denote the topological space $(\mathcal{S},\mathcal{E},\mB)$ simply by $\mathcal{S}$.   
$\mB$ is used to extend differential geometry to graphs \citep{schaub2020random}, since for $\alpha $ an outgoing edge from vertex $\mu$, we have 
$\mB_\alpha \vf = \vf_\mu - \vf_\nu \sim \ro_\alpha \vf $. 
We show that for $G$ to preserve the topology, components of $\hat{L}_i$ should act on the local neighborhood of each node and related to each other via the pushforward
\begin{align}
    [\hat{L}_i]_\mu^\nu &= [g_\mu L_i\vx_0]^\nu = [\hat{\ell}_i]_\mu^\alpha \mB_\alpha^\nu 
    = [\hat{\ell}_i]_0^\alpha \mB_\alpha^\rho [g_\mu]^\nu_\rho.
    \label{eq:hat-L-discrete}
\end{align}
$\hat{L}_i \equiv \hat{\ell}_i^\alpha \mB_\alpha $ is the discrete $\mathcal{S}$ version of the vector field $\hat{L}_i(\vx) = [g L_i \vx_0]^\alpha \ro_\alpha $ in \eqref{eq:dfdg-general}.
Here $ [\hat{\ell}_i]_0^\alpha \in \R $ are weightings for edges $\alpha $ connected to $\vx_0$ and capture the action of $L_i$. 
This weighting is similar to Gauge Equivariant Mesh (GEM) CNN \citep{cohen2019gauge}. 
The main difference is that in GEM-CNN the basis of the tangent spaces $T_{\vx_\mu}\mathcal{S}$ are not fixed and are chosen by a gauge. 
In L-conv the lift $\vx_\mu = g_\mu\vx_0$ fixes the gauge by mapping neighbors of $\vx_0$ to neighbors of $\vx_\mu$. 
% , meaning it determines how the basis at $<0>$ maps to the basis at $<\mu>$. 
Changing how the discrete $\mathcal{S}$ samples an underlying continuous space 
% $\mathcal{S}_0$ 
% is unchanged but the points sampled from it to create $\mathcal{S}$ are moved a bit, 
changes $g_\mu$ and hence the gauge, similar to GEM-CNN. 
% have the form $[\hat{L}_i]_\mu^\nu = [\hat{\ell}_i]_\mu^\alpha \mB_\alpha^\nu $. 
% Additionally, we show that the lift $g_\mu$ relates components of $\hat{L}_i$ via the pushforward
% $[\hat{\ell}_i]_\mu^\alpha \mB_\alpha^\nu = [\hat{\ell}_i]_0^\alpha \mB_\alpha^\rho [g_\mu]^\nu_\rho$. 
% Thus, to implement 
% means and how it impacts the learning of symmetries using L-conv. 
Next, we discuss the relation between L-conv and other neural architectures. 



==> secs2/theory-bkp-2021-10-25.tex <==


% \ry{Show a picture of generation in a set, made with mathematical \href{https://keenan.is/illustrating/2017/03/03/illustrating-lie-groups/}{Illustration}}
% \subsection{Continuous Symmetry, Lie Groups and Lie Algebras}
% \nd{Shorten}
% We will focus on Lie groups that are subsets $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group in $d$ dimensions.
% Our results generalize trivially to other number fields such as $\C$. 
% For any Lie group $G\subset \mathrm{GL}_d(\R)$,

\section{Lie Algebra Convolutional Network}
As mentioned above, 
the Lie algebra basis $L_i\in \mathfrak{g}$ can be used to construct the Lie group $G$ using the exponential map. 
Similarly, we show that G-conv layers can be constructed using a more basic architecture utilizing the Lie algebra.
The key idea is to approximate the kernel $\kappa(u)$ using localized kernels which can be constructed using the Lie algebra (Fig. \ref{fig:G-conv2L-conv}).
This is possible because the exponential map is a generalization of a Taylor expansion. 
% This process is closely mimics the universal approximation theorem of neural networks. 
The first step is to show that a G-conv whose kernel is concentrated near identity can be expanded in the Lie algebra.  
% Concretely, we will use the Lie algebra to expand G-conv \eqref{eq:G-conv} near the identity $I$. 
% This yields basic building blocks from which an arbitrary G-conv can be constructed.
% is to instead approximate $\kappa(v)$ utilizing the Lie algebra.
% \subsection{Expanding in G-conv in the Lie algebra}
% We consider a G-conv \eqref{eq:G-conv} with a kernel localized near identity $I$.

Let $\delta_\eta (u)\in \R$ denote a normalized \textit{localized kernel}, meaning $\int_G \delta_\eta(g)dg=1 $, and with support on a small neighborhood of size $\eta$ near $I$ (i.e., $\delta_\eta(I+\eps^iL_i) \to 0 $ if $\|\eps\|^2>\eta^2$).
Let $\kappa_0 (u) = W^0 \delta_\eta (u)$, where $W^0\in \R^{m'} \otimes \R^{m}$ are constants. 
% and $\delta_\eta(u) \in \R$ is a normalized kernel, $\int_G \delta_\eta(g)dg=1 $,
% with support on a small neighborhood of size $\eta$ near $I$, meaning $\delta_\eta(I+\eps^iL_i) \to 0 $ if $\|\eps\|^2>\eta^2$.
The localized kernels $\kappa_0$ can be used to approximate G-conv. 
We first derive the expression for a G-conv whose kernel is $\kappa_0$. 

\out{
Note that with $f(g)\in \R^m$, each $\eps^i \in\R^{m} \otimes \R^m $ is a matrix. 
With indices, $f(gv_\eps) $ is given by 
\begin{align}
    [f(gv_\eps)]^a &= \sum_b f^b(g(\delta^a_b + [\eps^i]^a_b L_i)) 
\end{align}
}%%%%

\textbf{Linear expansion of G-conv with localized kernel}
% \ry{simplify the notations} 
We can expand a G-conv whose kernel is $\kappa_0(u) = W^0 \delta_\eta(u)$ in the Lie algebra of $G$ to linear order. 
With $v_\eps = I+\eps^i L_i $, we have
%to obtain the L-conv architecture.
(see SI \ref{ap:theory-extended}, \eqref{eq:L-conv-basic})
\begin{align}
    Q[f](g)&=[\kappa_0 \star f](g) 
    = \int_G dv \kappa_0 (v) f(gv )
    =\int_{\|\eps\| <\eta } dv_\eps  \kappa_0 (v_\eps) f(gv_\eps )\cr
    % &= \int d\eps \delta_\eta (I+\eps^i L_i) f(g(I+\eps^i L_i))\cr
    % &= \int d\eps \delta_\eta (I+\eps^i L_i) f(g+\eps^i gL_i)\cr
    &
    = W^0\int d\eps \delta_\eta(v_\eps) %(I+\eps^i L_i) 
    \br{f(g)+ \eps^i g L_i \cdot {d\over dg}  f(g) + O(\eps^2) } %\bigg|_{u\to g}
    \cr
    % &\approx \int d\eps \kappa_0 (I+\eps^i L_i) \br{I+ \eps^i g L_i \cdot {d\over dg} } f(g)
    % \cr
    % & \approx W^0\br{I + \ba{\eps}^i g L_i\cdot {d\over dg} } f(g)
    % \label{eq:L-conv-basic} 
    &= W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }f(g) +O(\eta^2) %\cr 
    % \mbox{\nd{out}}
    % &= [W^0]_b f^a\pa{g\pa{\delta^a_b+ [\ba{\eps}^i]_a^b L_i}} +O(\eta^2)
    \label{eq:L-conv}
\end{align}
% where $\delta^a_b$ is the Kronecker delta and, 
where $W^0\in \R^{m'} \otimes \R^m$, and
using  %$\kappa_0(v)=c \delta_\eta(v)$ with $c\in \R^{m'}\otimes \R^m$ 
$\int_G \delta_\eta(g)dg= \int d\eps \delta_\eta(v_\eps)=1 $ and $\eps^i\in \R^{m}\otimes \R^m$, we have defined
\begin{align}
    % W^0 &= %\int_G dv \kappa_0(v) = 
    % \int d\eps\kappa_0 (I+\eps^iL_i) \in \R^{m'} \otimes \R^m, &
    \ba{\eps}^i &= \int d\eps \delta_\eta (v_\eps) %(I+\eps^iL_i) 
    \eps^i \in \R^{m} \otimes \R^m. 
\end{align}
Note that because $\|\eps\|<\eta$ we also have $\|\ba{\eps}\|<\eta $ (SI \ref{ap:theory-extended}, \eqref{eq:O-eta-p}). 
Here $d\eps $ is the integration measure on the Lie algebra $\mathfrak{g}=T_IG$ induced by the Haar measure $dv_\eps $ on $G$.
% where we used the fact that the Haar measure $dv$ induces an integration measure on the Lie algebra, which we denoted by $d\eps$.

\textbf{Interpreting the derivatives}
In a matrix representation of $G$, we have $g L_i\cdot {df\over dg} = [g L_i]_\alpha^\beta {df\over dg_\alpha^\beta} = \Tr{[g L_i]^T {df\over dg} }$.
% $g L_i\cdot {df\over dg} = \sum_{a,b}[g L_i]_{ab} {df\over dg_{ab}} = \Tr{[g L_i]^T {df\over dg} }$.
% Note that in $g(I+\eps^iL_i)\vx_0$, the $gL_i\vx_0 = \hat{L}_i(g)\vx$ come from the pushforward $L_i^{(g)}=gL_ig^{-1} \in T_gG$.
%of $L_i\in T_IG$ from the tangent space at $I$ to the tangent space at $g$, meaning $gL_ig^{-1} \in T_gG$. 
% This is seen from the fact that $gv_\eps$ is moving from $g$ by $\eps L_i$, hence in $T_gG$. 
% We will show this explicitly in following examples. 
% \Eqref{eq:L-conv-basic} is the core of the architecture we are proposing, the Lie algebra convolution or \textbf{L-conv}.
% The $gL_i\cdot df/dg$ in \eqref{eq:L-conv} 
This can be written in terms of partial derivatives $\ro_\alpha f(\vx) = \ro f/\ro \vx^\alpha$ as follows.
% In general, 
Using $\vx^\rho = g^\rho_\sigma \vx_0^\sigma$, we have ${df(g\vx_0)\over dg^\alpha_\beta} =\vx_0^\beta \ro_\alpha f(\vx) $, and so
% \ry{add a cartoon}
\begin{align}
    % \vx^\mu &= g^\rho_\sigma \vx_0^\sigma &
    % {df(g\vx_0)\over dg^\alpha_\beta}
    % &= {d(g^\rho_\sigma \vx_0^\sigma) \over dg^\alpha_\beta}\ro_\rho f(\vx) = \vx_0^\beta \ro_\alpha f(\vx)
    % \label{eq:dgx0-dg}
    % \\
    \hat{L}_if(\vx)\equiv gL_i\cdot {df\over dg} &= [gL_i]^\alpha_\beta \vx_0^\beta \ro_\alpha f(\vx) = [gL_i\vx_0]\cdot \del f(\vx) %= \hat{L}_if(\vx)
    \label{eq:dfdg-general}
\end{align}
Hence, for each $L_i$, the pushforward $gL_ig^{-1}$ generates a flow on $\mathcal{S}$ through the vector field $\hat{L}_i\equiv gL_i\cdot d/dg = [gL_ig^{-1} \vx]^\alpha \ro_\alpha$ (Fig. \ref{fig:Lie-group-S}). 
% $\hat{L}_i$ is related to the Maurer-Cartan form $\omega = g^{-1} \ro_\alpha g d\vx^\alpha$, which encodes the pushforward.
% Write $f(gv_\eps) = f(g+ \eta(\eps)^\alpha \ro_\alpha g)$. 
% We have $ \eta^\alpha \ro_\alpha g = \eps^i g L_i$, so $ \eps^i L_i \eta^\alpha g^{-1} \ro_\alpha g = \eta \cdot \omega $.
% The Maurer-Cartan form defines a way to parallel transport (pushforward) and define a basis frame on  
% Vector fields are sections of the tangent bundle $T\mathcal{S}$.
% We will encounter $gL_i\vx_0$ again on a discretized $T\mathcal{S}$ again below. 
\out{
Being a vector field $\hat{L}_i\in T\mathcal{S}$ (i.e. 1-tensor), $\hat{L}_i$ is basis independent, meaning 
for $v \in G$, $\hat{L}_i(v\vx) = \hat{L}_i$. 
Its components transform as $[\hat{L}_i(v \vx)]^\alpha =[vgL_i\vx_0]^\alpha = v^\alpha_\beta \hat{L}_i(\vx)^\beta $, while the partial transforms as $\ro / \ro[v\vx]^\alpha = [v^{-1}]^{\gamma}_\alpha \ro_\gamma$. 
}%%%
% \ry{formally define a L-conv layer, put Equation 10 here}

\textbf{Lie algebra convolutional (L-conv) layer}
% \out{
% \textbf{L-conv Layer} 
\Eqref{eq:L-conv} states that for a kernel localized near identity the effect of the kernel can be summarized in $W^0$ and $\ba{\eps}^i\hat{L}_i$. 
It is important to note that we do not need to perform the integral over $G$ explicitly anymore. 
Instead of working with a kernel $\kappa_0$, we only need to specify $W^0$ and $\ba{\eps}^i$. 
The construction in \eqref{eq:L-conv} turns out to be the basic building block of G-conv, as we show below. 
Hence, in general, we define the Lie algebra convolution (L-conv) as  
\begin{align}
    Q[f](\vx)%&= \br{W^0 + W^i g L_i\cdot {d\over dg} } f(g) 
    % &= W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }f(g\vx_0) 
    &= W^0\br{I+\ba{\eps}^i\hat{L}_i} f(\vx)\cr 
    &= W^0 \br{I + \ba{\eps}^i  [gL_i\vx_0]^\alpha \ro_\alpha }f(\vx) %\cr 
    % \mbox{\nd{out}}
    % &= [W^0]_b f^a\pa{g\pa{\delta^b_a+ [\ba{\eps}^i]_a^b L_i}\vx_0} +O(\ba{\eps}^2)
    \label{eq:L-conv-def0}
\end{align}
% }%%%%
% For $f(g)\in \R^m $, 
% For brevity, we define $W^i\equiv W^0 \ba{\eps}^i$.
% , and found using the Moore-Penrose inverse $\tilde{W}_0^{-1} = (W^{0T}W^0)^{-1}W^0$. 

Being an expansion of G-conv, L-conv inherits the equivariance of G-conv, as we show next.

\begin{proposition}[Equivariance of L-conv]\label{prop:L-conv-equiv}
    With assumptions above,
    L-conv is equivariant under $G$. % to  $O(\eta^2)$. 
\end{proposition}


% \nd{redo proof with expansion}
\begin{proof}
\out{
    From \eqref{eq:L-conv} it follows that L-conv is equivariant up to $O(\ba{\eps}^2) \sim O(\eta^2)$, as for $w\in G$
\begin{align}
    w\cdot Q[f](g)&= Q[f](w^{-1}g) 
    = W^0 f\pa{w^{-1} g\pa{I+ \ba{\eps}^i L_i}} +O(\eta^2)
    %= W^0 w \cdot f\pa{ g v_\eps} 
    = Q[w\cdot f](g).
    \label{eq:L-conv-equiv}
\end{align}
\nd{2nd way}
}%%%%%
First, note that the components of $\hat{L}_i$ transform as $[\hat{L}_i(v \vx)]^\alpha =[vgL_i\vx_0]^\alpha = v^\alpha_\beta \hat{L}_i(\vx)^\beta $, while the partial transforms as $\ro / \ro[v\vx]^\alpha = [v^{-1}]^{\gamma}_\alpha \ro_\gamma$.
As a result in $\hat{L}_i = [gL_i\vx_0]^\alpha \ro_\alpha $ all factors of $v$ cancel, meaning 
for $v \in G$, $\hat{L}_i(v\vx) = \hat{L}_i(\vx)$. 
% To prove the equivariance of the expanded version of L-conv, 
This is because of the fact that $\hat{L}_i\in T\mathcal{S}$ is a vector field  (i.e. 1-tensor) and, thus, invariant under change of basis. 
% Its components transform as $[\hat{L}_i(v \vx)]^\alpha =[vgL_i\vx_0]^\alpha = v^\alpha_\beta \hat{L}_i(\vx)^\beta $, while the partial transforms as $\ro / \ro[v\vx]^\alpha = [v^{-1}]^{\gamma}_\alpha \ro_\gamma$ resulting in all factors of $v$ cancelling out. 
Plugging into \eqref{eq:L-conv-def0}, for $w\in G$
\begin{align}
    w\cdot Q[f](\vx)&= Q[f](w^{-1}\vx) = W^0\br{I+\ba{\eps}^i \hat{L}_i(w^{-1}\vx)} f(w^{-1}\vx) \cr
    &=  W^0\br{I+\ba{\eps}^i \hat{L}_i(g)} f(w^{-1}\vx) 
    =  W^0\br{I+\ba{\eps}^i \hat{L}_i(g)} w\cdot f(\vx)\cr
    &= Q[w\cdot f](\vx)
    \label{eq:L-conv-equiv}
\end{align}
which proves L-conv is equivariant. 
\end{proof}

% Next, we provide some explicit example of the form of L-conv for familiar continuous symmetries. 

% \ry{make this a prop}
% \textbf{Equivariance of L-conv}

\out{
\ry{explain the Taylor expansion in (25)}
% $\delta_\eta \star f$ may be expanded  near identity as
\begin{align}
    Q[f](g)&\equiv c[\delta_\eta \star f](g) 
    = %\approx
    c\int d\eps \delta_\eta (I+\eps^i L_i) \br{I+ \eps^i g L_i \cdot {d\over dg} } f(g) %\bigg|_{u\to g}
    +O(\eta^2)
    \cr
    &= W^0 \br{I + \ba{\eps}^i g L_i\cdot {d\over dg} }f(g) +O(\eta^2)\cr 
    &= [W^0]_b f^a\pa{g\pa{I+ [\ba{\eps}^i]_a^b L_i}} +O(\eta^2)
    \label{eq:L-conv}
    % = \br{W^0 + W^i g L_i\cdot {d\over dg} } f(g)
    % \label{eq:L-conv-basic} 
\end{align}
}%%%% 
% \subsection{Interpretation and Examples \label{sec:interpret-continuous} }
% \paragraph{General case} 
\paragraph{Examples}
Using \eqref{eq:dfdg-general} we can calculate the form of L-conv for specific groups (details in SI \ref{ap:examples-continuous}). 
For \textbf{translations} $G=T_n = (\R^n,+)$ we find the generators become simple partial derivatives $\hat{L}_i = \ro_i$ (SI \ref{ap:example-Tn}), yielding $f(\vx) + \eps^\alpha \ro_\alpha f(\vx)$. 
For \textbf{2D rotations} (SI \ref{ap:example-so2}) 
we find $\hat{L} \equiv \pa{x \ro_y - y \ro_x } = \ro_\theta$, which in physics is called the angular momentum operator about the z-axis in quantum mechanics and field theories. %, which generates rotations around the $z$ axis. 
For rotations with scaling, 
\textbf{Rotation and scaling} $G= SO(2)\times \R^+$, 
we have two $L_i$, one $\hat{L}_\theta=\ro_\theta $ from $so(2)$ and a scaling with $L_r = I$, yielding
$\hat{L}_r = x\ro_x+y\ro_y= r\ro_r $. % (SI \ref{ap:examples-continuous}) 
Next, we discuss the form of L-conv on discrete data. 


\subsection{Approximating G-conv using L-conv \label{sec:G-conv2L-conv} }
\begin{figure}
    \centering
    \includegraphics[width=.8\linewidth]{figs2/G-conv2L-conv.pdf}
    \caption{
    Sketch of the procedure for approximating G-conv using L-conv. 
    First, the kernel is written as the sum of a number of localized kernels $\kappa_k$ with support around $u_k$ (left). 
    Each of the $\kappa_k$ is then moved toward identity by composing multiple L-conv layers $Q_{\eps'}\circ Q_\eps\dots \kappa_k $ (right). 
    % The more layers used, the more accurate the 
    }
    \label{fig:G-conv2L-conv}
\end{figure}

L-conv can be used as a basic building block which can be combined to make more G-conv with more general kernels. 
Figure \ref{fig:G-conv2L-conv} sketches the argument described here (see also SI \ref{ap:G-conv2L-conv}).
\begin{theorem}[G-conv from L-convs]
    \label{thm:Gconv2Lconv}
    G-conv \eqref{eq:G-conv} can be approximated using L-conv layers.
\end{theorem}
\begin{proof}
    The procedure involves two steps, as illustrated in Fig. \ref{fig:G-conv2L-conv}: 1) approximate the kernel using localized kernels as the $\delta_\eta$ in L-conv; 2) move the kernels towards identity using multiple L-conv layers. 
    The following lemma outline the details.
\end{proof}

% To do so, we first note that any function $\kappa(v)$ can be approximated to arbitrary accuracy using a set of local kernels $\delta_\eta $ (using the universal approximation theorem of neural networks \citep{hornik1989multilayer,cybenko1989approximation}).

\begin{lemma}[Approximating the kernel] 
    \nd{Robin, please check:}
    Let the kernel $\kappa:G\to \mathcal{F}'\otimes \mathcal{F}$ with $\int_G \kappa(g) dg < \infty$ be continuously differentiable with $\|d\kappa(g)/dg\|^2<\xi^2 $, and with compact support over $G_0\subset G$.  
    Let $\kappa_k(g)=c_k\delta_\eta(u_k^{-1}g) $ be a set of kernels with support on an $\eta$ neighborhood of $I\in G$.  
    Then, $\exists c_k \in  \mathcal{F}'\otimes \mathcal{F}$ such that $\tilde{\kappa}$ approximates $\kappa$, meaning
    $\int_G \|\kappa(g)-\tilde{\kappa}(g)\|^2dg < \zeta^2 $ for arbitrary small $\zeta\in \R_+$.
\end{lemma}
% \textbf{Approximating the kernel}
\begin{proof}
The intuition is similar to the universal approximation  theorem for neural networks \citep{hornik1989multilayer,cybenko1989approximation}, only generalized to  a group manifold instead of $\R$. 
Consider a set of non-overlapping neighborhoods $B_k \subset G_0$ of size $\eta \ll 1$, meaning $\int_{B_k}dg =\eta$, and such that
$\bigcup_k B_k = G_0$.
\out{
$\bigcup_k B_k = G_0/\phi$ where $\phi$ is a measure zero set (i.e. $B_k$ make a dense covering of the support of $\kappa$) \nd{precise?}.
}%%
We can show that, for small enough $\eta$, the kernel does not change more than $\xi$ over each $B_k$, allowing us to replace it with a constant localized kernel $\kappa_k$ with support only on $B_k$. 
To see this, consider $g\in B_k$ and $v_\eps= I+\eps^iL_i \in\mathfrak{g} $, such that $v_\eps g \in B_k$.
Let $\gamma$ be a path connecting $g$ to $v_\eps g$, via $u(s) = (I+s\eps^iL_i)g$, with $s\in [0,1]$. 
Using the triangle inequality we have 
\begin{align}
    \|\kappa(g)-\kappa(v_\eps g)\|^2& = \norm{\int_\gamma ds {d\kappa(u(s))\over ds} }^2 \leq
    \int_\gamma ds\norm{ {d\kappa(u(s))\over ds} }^2 \cr &
    < \int_0^1 ds \norm{dg\over ds}^2 \xi^2 = \|\eps\|^2 \xi^2 
\end{align}
where $\|\eps\|^2 \leq \eta^2$ because $v_\eps g\in B_k$. 
This means that if we replace $\kappa(g)$  with $\kappa(u_k)$ for any $u_k\in B_k$, our error in approximating $\kappa$ over $B_k$ is less than $\zeta^2 \eta^2 $. 
Setting $\kappa_k(g) =\kappa(u_k) \delta_\eta(u_k^{-1}g)$ with the localized kernels   $\delta_\eta(g)$ being any continuously differentiable distribution such that $\int_{B_k} dg \delta_\eta(u_k^{-1}g)=1$ on all $B_k$, we get 
% $=1/|B_k|$ if $g\in B_k$ and $0$ otherwise, we get 
\begin{align}
    \int_G dg \|\kappa(g)-\tilde{\kappa}(g)\|^2 = \sum_k \int_{B_k} dg \|\kappa(g)-\kappa_k(g)\|^2 < \sum_{k} {1\over |B_k|} \int_{B_k} dg \eta^2 \xi^2 = \eta^2 \xi^2
\end{align}
% where $|G_0|$ is the size of the support $G_0\subset G$ of $\kappa$.
\out{
This simply follows from the universal approximation theorem for neural networks \citep{hornik1989multilayer,cybenko1989approximation} and the same approximation errors apply. 
$\delta_\eta(g)$ can be written as the sum of two sigmoid functions 
$\delta_\eta(g) =\mathrm{sig}(v_\eta g)+\mathrm{sig}(v_\eta^{-1}g) $. 
}%%%%
\end{proof}

Thus, we can approximate a large class of kernels as $\kappa(g) \approx \sum_k \kappa_k(g)$ where the local kernels $\kappa_k (g) = c_k \delta_\eta (  u_k^{-1}g)$ have
support only on an $\eta$ neighborhood of $u_k \in G $. 
Here $c_k\in \R^{m'} \otimes \R^{m}$ are constants and $\delta_\eta(u)$ is as in \eqref{eq:L-conv}.  
Using this, G-conv \eqref{eq:G-conv} becomes
\begin{align}
    [\kappa \star f](g)
    % & = \sum_k [\kappa_k \star f](g) 
    &= \sum_k c_k \int dv \delta_\eta(u_k^{-1} v) f(gv) 
    % &= \sum_k c_k \int dv \delta_\eta(v ) f(gu_k v) 
    = \sum_k c_k [\delta_\eta \star f] (gu_k).
    \label{eq:c-k-delta}
\end{align}
% As we showed in \eqref{eq:L-conv-basic}, $[\delta_\eta \star f](g)$ is the definition of L-conv. 
% \ry{put this as a theorem, show as an approximation error}
The kernels $\kappa_k$ are localized around $u_k$, whereas in L-conv the kernel is around identity. 
We can compose L-conv layers to move $\kappa_k$ from $u_k$ to identity. 

\out{
Can we write the movement of a $\delta$ on the group explicitly as the action of the exp map on a $\delta$ near identity? 
For a group element it is clear, but for a function over the group? 
Should we use the fact that we have convolution, i.e. integral over the group? 
With $v = P\exp[\int_\gamma dt^i L_i]$ we have 
\begin{align}
    f(g) &= \int_G du f(u)\delta(u^{-1}g) \cr 
    f(vg) &= \int_G du f(u)\delta(u^{-1}vg) = \int_G du' f(v^{-1}u')\delta({u'}^{-1}g) 
\end{align}
Can we use the integral 
}
\begin{lemma}[Moving kernels to identity]
    The local kernel $\kappa_k$ can be moved near identity using a multilayer L-conv.  
\end{lemma}
\begin{proof}
In \Eqref{eq:c-k-delta}, write $u_k = v_\eps u'_k$, with $v_\eps = I+ \eps^i L_i \in \mathfrak{g}$. 
We have  
\begin{align}
    \delta_\eta(u_k^{-1} v) &= \left.\br{I+ \eps^i g L_i \cdot {d\over dg} }\delta_\eta(g)\right|_{g\to {u'}_k^{-1} v} + O(\eps^2) \approx Q_\eps[\delta_\eta]({u'}_k^{-1} v)
\end{align}
where $Q_{\eps} = I-\eps^i \hat{L}_i$ is an L-conv layer with $W^0=I$. 
This means that a applying one L-conv layer with the parameters above moves the localized kernel along $v_\eps $ on $G$.   
Iterating this further, write $u_k$ as the product of a set of small group elements $u_k = \prod_{a=1}^p v_a$, with $v_a = I+ \eps_a^i L_i \in \mathfrak{g}$. 
Defining L-conv layers $Q_a = I-\eps_a^i \hat{L}_i $,
we can write 
\begin{align}
    \kappa_k (g) &\approx c_k Q_p \circ \cdots \circ Q_1 \circ \delta_\eta (g)  
\end{align}
meaning $\kappa_k$ localized around $u_k$ can be written as a $p$ layer L-conv acting on a kernel  $\delta_\eta(g)$, localized around the identity of the group. 
\out{
Thus, by applying multiple L-conv layers we can find $Q_p \circ \dots Q_1\circ \kappa_k\approx c_k\delta_\eta $. 
This can always be done using a set of $v_{\eps_a} = (I+\ba{\eps}_a^iL_i)$ such that $u_k \approx \prod_{a=1}^p v_{\eps_a}$. 
}%%%%
With $\|\eps_a\|<\eta$, the error in $u_k$ is $O(\eta^{p+1})$.
\end{proof}

Thus, we conclude that any G-conv \eqref{eq:G-conv} can be approximated by multilayer L-conv. 
We can take this result even further, following the main theorem in \citet{kondor2018generalization}, and show that any feedforward equivariant neural network can be approximated using multilayer L-conv with nonlinearities. 

\paragraph{Equivariance of nonlinearity}
Point wise nonlinearities will keep an equivariant scalar function equivariant. \nd{ref instead?} 
To see this, 
let $\sigma:\R \to \R $, $f:\mathcal{S}\to \mathcal{F}$ be a scalar (i.e., $g\cdot f(\vx) = f(g^{-1}\vx)$) and $Q:\mathcal{F}\to \mathcal{F}'$ be equivariant (i.e. $g\cdot Q[f]= Q[g\cdot f]$).
Then, $\sigma(Q[f](\vx))$ is still a scalar and for $g\in G$ we have 
\begin{align}
    % g\cdot \sigma\circ f^a(\vx)& = \sigma\circ f^a(g^{-1}\vx) = \sigma\circ g\cdot f^a(\vx) \cr
    g\cdot \sigma\circ Q[f](\vx)& = \sigma\circ Q[f](g^{-1}\vx) = \sigma\circ g\cdot Q[f](\vx) 
\end{align}
meaning, point-wise nonlinearity $\sigma$ is equivariant for scalar $Q[f]$. 
Hence we have the corollary:

\begin{corollary}[Feedforward NN]
    Any equivariant feedforward neural network (FNN) can be approximated using multilayer L-conv with point-wise nonlinearities. 
\end{corollary}
\begin{proof}
This follows from the main theorem in  \citet{kondor2018generalization} and the our Theorem \ref{thm:Gconv2Lconv}. 
A FNN is defined as $\sigma_p \circ F_p(\cdots ( \sigma_1\circ  (F_1  (f)(\vx)$ where $F_k$ are linear and $\sigma_k$ are point-wise nonlinearities.
Any linear equivariant layer has to be G-conv, which can be approximate by multilayer L-conv.
Therefore, multilayer L-conv with nonlinearity can approximate any equivariant FNN.
\end{proof}

As a final note, we should point out that to our knowledge it is not known whether \textit{every equivariant function} can be approximated by equivariant FNN. 
Hence, the corollary above is \textit{not} a universal approximation theorem for equivariant scalar functions in terms of L-conv. 
%
% \nd{Mention/review Rao's result and how it demonstrates this theorem for 1D translation.}
\out{
We conducted small controlled experiments to verify how multilayer L-conv approximates G-conv (SI \ref{ap:experiments}). 
We briefly discuss them here. 

\paragraph{Learning symmetries using L-conv}
\citet{rao1999learning} introduced a basic version of L-conv and showed that it can learn 1D translation and 2D rotation. 
% They showed that t
The learned 
% infinitesimal generator 
$L_i$ for 1D translation reproduced finite translation well using $(I+\eps L)^N$, which is $N$ recursive L-conv layers. 
Hence, their results prove that L-conv can be used to approximate CNN, as well as $SO(2)$ G-conv. 
We discuss the details of L-conv approximating CNN below in sec. \ref{sec:approx}.
We also conducted more complex experiments using recursive L-conv to learn large rotation angle between two images 
% \nd{revise if experiments moved to SI}
(SI \ref{ap:experiments}).
% These experiments required L-conv to approximate rotations by large angles, which it did successfully. 
% The learned $L$ also has the right structure (Fig. \ref{fig:L-so2-combined}).
\out{
% We can use L-conv for learning the Lie algebra as well. 
% In fact, the architecture used in \citet{rao1999learning} is a basic version of L-conv with $W^0 = 1$. 
They show that with a small fixed $\ba{\eps^i}$ they could learn learn the single $L_i$ for continuous 1D translations and for 2D rotations.
Indeed, the architecture used in \citet{rao1999learning} is a special case of L-conv with $W^0 = 1$ and $\ba{\eps}^i\in \R$. 
We conducted a more advanced experiment with L-conv learning rotation angles in pairs of random images (SI \ref{ap:exp-L-multi})
}%
% experiments for with $G=SO(2)$.
% In the first test, we used fixed small rotation angle $\pi/10$ and used 
Figure \ref{fig:L-so2-combined} shows the learned $L$. 
Left shows $L\in so(2)$ learned using L-conv in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
Middle and right of Fig. \ref{fig:L-so2-combined} are experiments with fixed small rotation angle $\theta = \pi/10$ (SI \ref{ap:exp-L-small}).
Middle is the $L$ learned using L-conv and right is using the exact solution $R = (YX^T)(X^TX)^{-1}$. 
While the middle $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
% Right shows the generator calculated using the exact solution to the linear regression problem with $\theta = \pi/10$. 
% The SGD solutions using L-conv are less noisy and capture more details.
(also see SI \ref{ap:experiments} for a discussion on symmetry discovery literature.)

L-conv can potentially replace other equivariant layers in an architectures.
We conducted limited experiments for this on small image datasets (SI \ref{ap:exp-image}). 
L-conv allows one to look for potential symmetries in data which may have been scrambled or harbors hidden symmetries. 
% Next, we will provide some examples of explicit forms of L-conv.
Since many datasets such as images deal with discretized spaces, we first need to derive how L-conv acts on such data, discussed next. 
% Next, we discuss the form of L-conv on discrete data. 


\begin{figure}
    \centering
    \includegraphics[width=.17\linewidth]{figs2/L-conv-recur-3.pdf}
    \includegraphics[width=.82\linewidth]{figs2/L-so2-combined.pdf}
    \caption{
    \textbf{Learning the infinitesimal generator of $SO(2)$} 
    Left shows the architecture for learning rotation angles between pairs of images (SI \ref{ap:exp-L-multi}). 
    Next to it is the $L$ learned using recursive L-conv in this experiment. %to learn rotation angle between pairs of images.  
    %in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
    Middle $L$ is learned using a fixed small rotation angle $\theta = \pi/10$, and
    % While this $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
    right shows $L$ found using the numeric solution from the data. 
    % The SGD solutions using L-conv are less noisy and capture more details.
    }
    \label{fig:L-so2-combined}
\end{figure}
%%
}%%%%

Since many datasets such as images deal with discretized spaces, we first need to derive how L-conv acts on such data, discussed next. 

\section{Discretized space and implementation: the tensor notation \label{sec:tensor} }
% If the dataset being analyzed is in the form of $f(\vx)$ for some sample of points $\vx$, together with derivatives $\del f(\vx) $, we can use the L-conv formulation above. 
% However, i
\out{
\begin{wrapfigure}{r}{.45\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \vspace{-40pt}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, L-conv is analogous to a Graph Convolutional Network with $d$ nodes and $m_{in}$ features. 
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-20pt}
\end{wrapfigure}
}%%%%%%

In many datasets, such as images, $f(\vx)$ is not given as continuous function, but rather as a discrete array, with %$\vx$ taking values over a grid. 
% In this case all the discussions above still hold, as discuss now. 
% In particular, e
% Let 
$\mathcal{S}= \{\vx_0,\dots \vx_{d-1}\}$ containing $d$ points. 
Each $\vx_\mu$ represents a coordinate in higher dimensional space,
% For instance, 
e.g. on a $10\times 10$ image, $\vx_0$ is $(x,y)=(0,0)$ point and $ \vx_{99}$ is $(x,y) =(9,9)$.

\textbf{Feature maps and group action}
In the tensor notation, we encode $\vx_\mu \in \mathcal{S}$ as the canonical basis (one-hot) vectors in $\vx_\mu \in \R^d$ with 
% To define features $f(\vx_\mu)\in \R^m$ for $\vx_\mu \in \mathcal{S}$, we embed $\vx_\mu \in \R^d$ and 
% encode them as the canonical basis (one-hot) vectors with components 
$[\vx_\mu]_\nu = \delta_{\mu\nu}$ (Kronecker delta), e.g. $\vx_0 = (1,0,\dots, 0)$.
The features become $\vf \in \mathcal{F}= \R^d \otimes \R^m $, meaning 
% feature maps $\vf \in \mathcal{F}$ are 
$d\times m$ tensors, with $f(\vx_\mu) = \vx_\mu^T \vf = \vf_\mu $.
%
% \paragraph{Group action}
% \nd{Change to $\vx_\mu^T g^T$ for less confusion.}
Although $\mathcal{S}$ is discrete, the group acting on $\mathcal{F}$ can be continuous (e.g. image rotations). 
Any $G\subseteq \mathrm{GL}_d(\R)$ of the general linear group (invertible $d\times d$ matrices) acts on $\vx_\mu \in \R^d$ and $\vf\in \mathcal{F}$. 
% Since $\vx_\mu \in \R^d$, $g \in G$ also naturally act on $\vx_\mu$. 
% The resulting 
% Note $\vy = g \vx_\mu \notin  \mathcal{S}$ is a linear combination $\vy = c^\nu \vx_\nu$ of elements in $\mathcal{S}$, not a single element.
% The action of $G$ on $\vf$ and $\vx$, can be defined in multiple equivalent ways.
% The most elegant one is if w
We define $f(g \cdot \vx_\mu) = \vx_\mu^T g^T\vf, \forall g\in G$, so that
% consistent with the lift. 
% This makes the group action on $\vf$ the natural action of $G$, meaning 
for $w\in G$ we have 
\begin{align}
    w\cdot f(\vx_\mu)&= f(w^{-1}\cdot \vx_\mu) = \vx_\mu^T w^{-1T}\vf = %\vx_\mu^T [w^T]^{-1} \vf = 
    [w^{-1}\vx_\mu]^T \vf
    \label{eq:G-action-tensor-T}
\end{align}
Dropping the position $\vx_\mu$, the transformed features are matrix product $w\cdot \vf= w^{-1T}\vf$. 


\paragraph{G-conv and L-conv in tensor notation} 
Writing G-conv \eqref{eq:G-conv} in the tensor notation we have 
\begin{align}
    [\kappa\star f](g\vx_0) = \int_G \kappa(v)f(gv\vx_0) dv = \vx_0^T \int_G v^{T} g^{T} \vf \kappa^T(v) dv 
    \equiv \vx_0^T [\vf \star \kappa](g) 
    \label{eq:G-conv-tensor}
\end{align}
where we moved $\kappa^T(v) \in \R^m \otimes \R^{m'}$ to the right of $\vf$ because it acts as a matrix on the output index of $\vf$.
The equivariance of \eqref{eq:G-conv-tensor} is readily checked with $w\in G$
\begin{align}
    w\cdot [\vf \star \kappa](g) & = [\vf \star \kappa](w^{-1}g) 
    % = \int_G v^{T} [w^{-1}g]^{T} \vf \kappa^T(v) dv %\cr &
    = \vx_0^T \int_G v^{T} g^T w^{-1T} \vf \kappa^T(v) dv %\cr &
    %= \int_G v^{-1} g^{-1} w\vf \kappa^T(v) dv 
    % = [w^{-1T} \vf \star \kappa](g)
    = [(w\cdot\vf) \star \kappa](g)
\end{align}
where we used $[w^{-1}g]^{T}\vf = g^{T} w^{-1T}\vf $.
Similarly, we can rewrite L-conv \eqref{eq:L-conv} in the tensor notation. 
Defining $v_\eps =I+ \ba{\eps}^i L_i $ 
\begin{align}
    Q[\vf](g) 
    &= W^0 f\pa{g\pa{I+ \ba{\eps}^i L_i}} 
    = \vx_0^T \pa{I+ \ba{\eps}^i L_i}^{T} g^{T} \vf W^{0T} \cr
    % &= \vx_0^T \pa{I+ \ba{\eps}^i L_i^T} g^{T} \vf W^{0T} \cr 
    &= \pa{\vx+ \ba{\eps}^i [gL_i\vx_0]}^T \vf W^{0T}.
    % = \br{\vf_\mu + \ba{\eps}^i [gL_i \vf]_\mu }W^{0T} 
    % \cr
    \label{eq:L-conv-tensor}
\end{align}
Here, $\hat{L}_i=gL_i\vx_0$ is eactly the tensor analogue of pushforward vector field $\hat{L}_i$ in \eqref{eq:dfdg-general}. 
We will make this analogy more precise below.

The equivariance of L-conv in tensor notation is again evident from the $g^T \vf$, resulting in 
\begin{align}
    Q[w\cdot \vf](g) &= \vx_0^Tv_\eps^T g^T w^{-1T} \vf W^{0T}= Q[\vf](w^{-1}g) = w\cdot Q[\vf](g)
    \label{eq:L-conv-equiv-tensor}
\end{align}


\paragraph{Tensor L-conv  layer implementation}
In conclusion, the discrete space L-conv \eqref{eq:L-conv-tensor} can be rewritten using the global Lie algebra basis $\hat{L}_i$
\begin{align}
    % \mbox{L-conv}:\  
    Q[\vf] &=   \pa{\vf + \hat{L}_i\vf \ba{\eps}^i} W^{0T}, & %\cr 
    Q[\vf]_\mu^a &= \vf_\mu^b [W^{0T}]_b^a + 
    [\hat{L}_i]_\mu^\nu \vf_\nu^c \br{W^i}^a_c
    \label{eq:L-conv-tensor-final}
\end{align}
Where $W^i=W^0\ba{\eps}^i$, $W^0 \in \R^{m_{in}}\otimes \R^{m_{out}}$ and $\ba{\eps}^i \in \R^{m_{in}}\otimes \R^{m_{in}}$ are trainable weights. 
The $\hat{L}_i$ can be either inserted as inductive bias or they can be learned to discover symmetries. % we will be learning $\hat{L}_i$. 
% We will discuss learning symmetries
% We derived L-conv from G-conv using kernels around identity. 

% \out{
% \begin{figure}
%     \centering
\begin{wrapfigure}{r}{.45\textwidth}
    % \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs/L-conv-sketch-2020-10-01.pdf}
    \vspace{-10pt}
    \includegraphics[width = 1\linewidth, trim=0 0 0 20pt]{figs2/L-conv-sketch-2021-05-17.pdf}
    % {figs/L-conv-sketch-2021-02-04.pdf}
    %{figs/L-conv-sketch-2020-11-19.pdf}
    \caption{
    {
    L-conv layer architecture.
    $L_i$ only act on the $d$ flattened spatial dimensions, and $W^i$ only act on the $m_{in}$ input features and returns $m_{out}$ output features.
    For each $i$, L-conv is analogous to a GCN %Graph Convolutional Network 
    with $d$ nodes and $m_{in}$ features.
    }
    }
    \label{fig:L-conv-layer}
    \vspace{-10pt}
\end{wrapfigure}
% \end{figure}
% }
To implement L-conv we we note that the structure of \eqref{eq:L-conv-tensor-final} is quite similar to a Graph Convolutional Network (GCN) \citep{kipf2016semi}. 
For each $i$, the shared convolutional weights are $\ba{\eps}^i W^{0T}$ and the aggregation function of the GCN, a function of the graph adjacency matrix, is $\hat{L}_i$ in L-conv. 
Thus, L-conv can be implemented as GCN modules for each $\hat{L}_i$, plus a residual connection for the $\vf W^{0T}$ term. 
Figure \ref{fig:L-conv-layer} shows the schematic of the structure of such an L-conv layer.   
In a naive implementation,  $\hat{L}_i$ can be general $d\times d $ matrices. 
However, being vector fields generated by the Lie algebra, $\hat{L}_i$ has a more constrained structure which allows them to be encoded and learned using much fewer parameters than a $d\times d $ matrix. 
Specifically, encoding the topology of $\mathcal{S}$ as a graph (see SI \ref{ap:L-conv-tensor-interpret}), the incidence matrix replaces partial derivatives \citep{schaub2020random} in \eqref{eq:dfdg-general} and the $L_i$ become weighting of the edges.
This weighting is similar to Gauge Equivariant Mesh (GEM) CNN \citep{cohen2019gauge}. 
% The main difference is that in GEM-CNN the basis of the tangent spaces $T_{\vx_\mu}\mathcal{S}$ are not fixed and are chosen by a gauge. 
Indeed, in L-conv the lift $\vx_\mu = g_\mu\vx_0$ fixes the gauge by mapping neighbors of $\vx_0$ to neighbors of $\vx_\mu$. 
% , meaning it determines how the basis at $<0>$ maps to the basis at $<\mu>$. 
Changing how the discrete $\mathcal{S}$ samples an underlying continuous space 
% $\mathcal{S}_0$ 
% is unchanged but the points sampled from it to create $\mathcal{S}$ are moved a bit, 
will change $g_\mu$ and hence the gauge, similar to GEM-CNN. 


\textbf{Choosing number of $L_i$} 
Beside the width of $W^0$ and $\ba{\eps}^i$, the number $n_L$ of $L_i$ is a hyperparameter in L-conv. 
For instance, if $\mathcal{S}$ is a discretization of $n$ dimensional space the symmetry group is likely $G\subset \mathrm{GL}_n(\R)\ltimes T_n $, with $n_L \sim O(n^2)$. 
Note that $n_L$ is independent of the size $d$ of the discretized space (e.g. number of pixels) and generally $n^2\ll d$.  
Choosing $n_L$ larger than the true number of $L_i$ only results in an over-complete basis and shouldn't be a problem. 
% \paragraph{Discretizing space vs group} 
% Next, we discuss these constraints. 

We conducted small controlled experiments to verify how multilayer L-conv approximates G-conv (SI \ref{ap:experiments}). 
We briefly discuss them here. 


\paragraph{Learning symmetries using L-conv}
\citet{rao1999learning} introduced a basic version of L-conv and showed that it can learn 1D translation and 2D rotation. 
% They showed that t
The learned 
% infinitesimal generator 
$L_i$ for 1D translation reproduced finite translation well using $(I+\eps L)^N$, which is $N$ recursive L-conv layers. 
Hence, their results prove that L-conv can be used to approximate CNN, as well as $SO(2)$ G-conv. 
We discuss the details of L-conv approximating CNN below in sec. \ref{sec:approx}.
We also conducted more complex experiments using recursive L-conv to learn large rotation angle between two images 
% \nd{revise if experiments moved to SI}
(SI \ref{ap:experiments}).
% These experiments required L-conv to approximate rotations by large angles, which it did successfully. 
% The learned $L$ also has the right structure (Fig. \ref{fig:L-so2-combined}).
\out{
% We can use L-conv for learning the Lie algebra as well. 
% In fact, the architecture used in \citet{rao1999learning} is a basic version of L-conv with $W^0 = 1$. 
They show that with a small fixed $\ba{\eps^i}$ they could learn learn the single $L_i$ for continuous 1D translations and for 2D rotations.
Indeed, the architecture used in \citet{rao1999learning} is a special case of L-conv with $W^0 = 1$ and $\ba{\eps}^i\in \R$. 
We conducted a more advanced experiment with L-conv learning rotation angles in pairs of random images (SI \ref{ap:exp-L-multi})
}%
% experiments for with $G=SO(2)$.
% In the first test, we used fixed small rotation angle $\pi/10$ and used 
Figure \ref{fig:L-so2-combined} shows the learned $L$. 
Left shows $L\in so(2)$ learned using L-conv in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
Middle and right of Fig. \ref{fig:L-so2-combined} are experiments with fixed small rotation angle $\theta = \pi/10$ (SI \ref{ap:exp-L-small}).
Middle is the $L$ learned using L-conv and right is using the exact solution $R = (YX^T)(X^TX)^{-1}$. 
While the middle $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
% Right shows the generator calculated using the exact solution to the linear regression problem with $\theta = \pi/10$. 
% The SGD solutions using L-conv are less noisy and capture more details.
(also see SI \ref{ap:experiments} for a discussion on symmetry discovery literature.)

L-conv can potentially replace other equivariant layers in an architectures.
We conducted limited experiments for this on small image datasets (SI \ref{ap:exp-image}). 
L-conv allows one to look for potential symmetries in data which may have been scrambled or harbors hidden symmetries. 
% Next, we will provide some examples of explicit forms of L-conv.
% Next, we discuss the form of L-conv on discrete data. 


\begin{figure}
    \centering
    \includegraphics[width=.17\linewidth]{figs2/L-conv-recur-3.pdf}
    \includegraphics[width=.82\linewidth]{figs2/L-so2-combined.pdf}
    \caption{
    \textbf{Learning the infinitesimal generator of $SO(2)$} 
    Left shows the architecture for learning rotation angles between pairs of images (SI \ref{ap:exp-L-multi}). 
    Next to it is the $L$ learned using recursive L-conv in this experiment. %to learn rotation angle between pairs of images.  
    %in $3$ recursive layers to learn rotation angles between a pair of $7\times 7$ random images $\vf$ and $R(\theta) \vf$ with $\theta \in [0,\pi/3)$. 
    Middle $L$ is learned using a fixed small rotation angle $\theta = \pi/10$, and
    % While this $L$ is less noisy, it does not capture weights beyond first neighbors of each pixel. 
    right shows $L$ found using the numeric solution from the data. 
    % The SGD solutions using L-conv are less noisy and capture more details.
    }
    \label{fig:L-so2-combined}
\end{figure}
%%

% Next, we discuss the relation between L-conv and other neural architectures. 




==> secs2/theory2-bkp-2021-10-24.tex <==

\section{Relation to other architectures \label{sec:approx} }
% \paragraph{Interpretation}
% Let us interpret this equation.
% In addition to the connection with GEM-CNN, we will now show that other important architectures such as CNN and Graph Convolutional Networks (GCN) \citep{kipf2016semi} are either a subset of L-conv or closely related to it.
L-conv can reproduce some familiar architectures for specific Lie groups, as we discuss now. 

\paragraph{CNN}
% While it is trivial to find permutations taking $\vx_0$ to $\vx_\mu$, most of them won't preserve the topology as \eqref{eq:lift-neigh}. 
% be an element of a given $G$. 
% For instance, 
This is a special case of expressing G-conv as L-conv when the group is continuous 1D translations. 
The arguments here generalize trivially to higher dimensions. 
\citet[sec. 4]{rao1999learning} used the Shannon-Whittaker Interpolation \citep{whitaker1915functions} to define continuous translation on periodic 1D arrays as $\vf'_\rho = g(z)_\rho^\nu \vf_\nu $.
Here $g(z)_\rho^\nu = {1\over d} \sum_{p=-d/2}^{d/2} \cos \pa{{2\pi p\over d}(z+\rho -\nu)} $ approximates the shift operator for continuous $z$.
These $g(z)$ form a 1D translation group $G$ as $g(w)g(z)=g(w+z)$ with $g(0)^\nu_\rho = \delta^\nu_\rho$.
For any $z=\mu \in \Z$,
$g_\mu=g(z=\mu)$ are circulant matrices that shift by $\mu$ as $ [g_\mu]^\rho_\nu=\delta^\rho_{\nu-\mu}$.
Thus, a 1D CNN with kernel size $k$ can be written suing $g_\mu$ as 
\begin{align}
    F(\vf)_{\nu}^a & = \sigma\pa{\sum_{\mu=0}^k  \vf_{\nu-\mu}^c [W^\mu ]^a_{c}  +b^a} = \sigma\pa{\sum_{\mu=0}^k  [g_\mu\vf]_\nu^c [W^\mu ]^a_{c}  +b^a}  
    \label{eq:CNN-1D}
\end{align}
where $W,b$ are the filter weights and biases. 
$g_\mu$ can be approximated using the Lie algebra and written as multi-layer L-conv as in sec. \ref{sec:G-conv2L-conv}. 
Using $g(0)^\nu_\rho \approx \delta(\rho-\nu)$, the single Lie algebra basis $[\hat{L}]_0=\ro_z g(z)|_{z\to0}$, acts as $\hat{L}f(z) \approx -\ro_z f(z)$ (because $\int \ro_z \delta (z-\nu)f(z) =-\ro_\nu f(\nu)$). 
% The Lie algebra has a single basis $[\hat{L}]_0=\ro_z g(z)|_{z\to0}$. 
% Since $g(0)^\nu_\rho \approx \delta(\rho-\nu)$, we have $\hat{L}f(z) \approx -\ro_z f(z)$. 
% , meaning $\hat{L}$ is a Fourier series for $\ro_z$. 
% We have
% \begin{align}
%     [\hat{L}]^\nu_\rho&=\hat{L}(\rho-\nu) = \sum_p {2\pi p \over d^2} \sin \pa{{2\pi p\over d}(\rho -\nu)},&
%     [\hat{L}\vf]_\rho &= \sum_\nu \hat{L}(\rho-\nu)\vf_\nu = [\hat{L}\star \vf]_\nu
% \end{align}
Its components are
$\hat{L}^\nu_\rho={L}(\rho-\nu) = \sum_p {2\pi p \over d^2} \sin \pa{{2\pi p\over d}(\rho -\nu)} $, which are also circulant due to the $(\rho-\nu)$ dependence.
% are approximately 
% ${L}(z)\approx {d\over \pi} \sin(\pi z) \br{z^{-2}+(d-z)^{-2}}$ on $z\in\Z$. 
% \nd{%From sinc form of $g(z)$. 
% What's the exact form?}
Hence, $[\hat{L}\vf]_\rho = \sum_\nu {L}(\rho-\nu)\vf_\nu = [{L}\star \vf]_\nu$ is a convolution. 
\citet{rao1999learning} already showed that this $\hat{L}$ can reproduce finite discrete shifts $g_\mu$ used in CNN.
They used a primitive version of L-conv with $g_\mu = (I+\eps \hat{L})^N$. 
Thus, L-conv can approximate 1D CNN. 
This result generalizes easily to higher dimensions. 
\out{
% $\hat{L}$ is a circulant matrix. 
$\hat{L}^\nu_\rho$ becomes concentrated around small $\rho-\nu$ when $d\gg1$  
% Thus, for large $d$ 
and we can approximate $L$ using $k\ll d$ nearest neighbors of each node.
Here $\mathcal{S}$ is a periodic 1D lattice with 
% $k$ nearest neighbor 
% graph encoding the topology is a circulant matrix
and adjacency matrix
$\mA_{\mu\nu} = \sum_{-k<\nu<k} \delta_{\mu,\mu+i}$ being a circulant matrix.
}%%%%

\paragraph{Relation with Graph Convolutional Networks (GCN)}
Let $\mA$ be the adjacency matrix of a graph. 
% Notice that 
In \eqref{eq:L-conv-tensor-final} if $\hat{L}_i = h(\mA)$, such as $\hat{L}_i =  \mD^{-1/2}\mA\mD^{-1/2}$, we obtain a GCN \citep{kipf2016semi} ($\mD_{\mu\nu} =\delta_{\mu\nu} \sum_\rho \mA_{\mu\rho} $ being the degree matrix). 
% In fact, 
% $[\hat{L}_i]_\mu^\nu=\mA_{\mu\nu}[\hat{L}_i]_\mu^\nu $ is only non-zero where the graph has. 
So in the special case where all neighbors of each node $<\mu>$ have the same edge weight, meaning $[\hat{L}_i]^\nu_\mu = [\hat{L}_i]^\rho_\mu$, $\forall\nu,\rho \in <\mu> $, \eqref{eq:L-conv} is uniformly aggregating over neighbors and L-conv reduces to a GCN. 
Note that this similarity is not just superficial. 
In GCN $h(\mA)= \hat{L}$ is in fact a Lie algebra basis. 
% As discussed above, $\hat{L}_i$ are vector fields on $T\mathcal{S}$.
When 
$\hat{L}= h(\mA)$, the vector field is the flow of isotropic diffusion $d\vf/dt = h(\mA)\vf$ from each node to its neighbors.
This vector field defines one parameter Lie group with elements $g(t) = \exp[h(\mA)t]$. Hence, %the most restricted 
L-conv for flow groups with a single generator are GCN. 
These flow groups include Hamiltonian flows and other linear dynamical systems. The main difference between L-conv and GCN is that L-conv can assign a different weight to each neighbor of the same node. 
As mentioned earlier, this
is similar to GEM-CNN \citep{cohen2019gauge} with a fixed gauge set by $g_\mu $.

\out{
The main difference between L-conv and GCN is that L-conv can assign a different weight to each neighbor of the same node. 
As mentioned earlier, this
is similar to GEM-CNN \citep{cohen2019gauge} with a fixed gauge set by $g_\mu $.
% Different weighting of neighbors 
This weighting is similar to Gauge Equivariant Mesh (GEM) CNN \citep{cohen2019gauge}. 
The main difference is that in GEM-CNN the basis of the tangent spaces $<\mu>=T_{\vx_\mu}\mathcal{S}$ are not fixed and are chosen by a gauge. 
In L-conv the lift $\vx_\mu = g_\mu\vx_0$ fixes the gauge, meaning it determines how the basis at $<0>$ maps to the basis at $<\mu>$. 
Changing how the discrete $(\mathcal{S},\mA)$ samples the underlying topological space $\mathcal{S}_0$ 
% is unchanged but the points sampled from it to create $\mathcal{S}$ are moved a bit, 
changes the lift $g_\mu$ and hence the gauge, similar to GEM-CNN. 
}%%%%%

Next, we discuss the mathematical properties of loss functions for L-conv.




\section{Group invariant loss \label{sec:Loss} }
% \ry{add the example of cycle-consistent loss}
% $G$ being a symmetry of the system means that $f$ and transformed features $g\cdot f$ have similar probability of occurring.
% Hence, 
Loss functions of equivariant architectures are rarely discussed. 
Yet, recent work by \citet{kunin2020neural} showed existence of symmetry directions in the loss landscape. 
To understand how the symmetry generators in L-conv manifest themselves in the loss landscape, we work out the explicit example of a mean square loss (MSE). 
Because $G$ is the symmetry group, $f$ and $g\cdot f$ should result in the same optimal parameters. 
Hence, the minima of the loss function need to be \textit{group invariant}.
One way to satisfy this is for the loss itself to be group invariant, which can be constructed 
% group invariant functions is to 
by integrating over $G$ (global pooling \citep{bronstein2021geometric}). 
A function $I  = \int_G dg F(g)$ is $G$-invariant (SI \ref{ap:invariant-loss}). 
We can also change the integration to $\int_\mathcal{S} d^nx $ by change of variable $dg/d\vx$ (see SI \ref{ap:invariant-loss} for discussion on stabilizers). 
% Next, we discuss the mean square loss (MSE) for a single layer L-conv and its relation to physics. 

\paragraph{MSE loss}
% In \eqref{eq:loss-invariance} $F(g)\in \R$
% is any scalar function of the features $f$ with a defined $G$ action. 
% For example 
% $F(g)$ 
% can be 
% Using \eqref{eq:loss-invariance},
The MSE is given by $I = \sum_n\int _G dg\|Q[f_n](g)\|^2$, where $f_n$ are data samples and $Q[f]$ is L-conv or another $G$-equivariant function. 
In supervised learning the input is a pair $f_n,y_n$. 
$G$ can also act on the labels $y_n$. 
We assme that $y_n$ are either also scalar features $y_n:\mathcal{S}\to \R^{m_y}$ with a group action $g\cdot y_n(\vx)=y_n(g^{-1}\vx)$ (e.g. $f_n$ and $y_n$ are both images), or that $y_n$ are categorical.
In the latter case $g\cdot y_n = y_n$ because the only representations of a continuous $G$ on a discrete set are constant. 
% via some representation $\pi:G\to \mathrm{GL}_c(\R)$.
%have their own $G$ action, 
% including being 
% though in classification $y_n$ is usually $G$-invariant. 
We can concatenate the inputs to 
% \ry{make sure the notation f is consistent} 
$\phi_n \equiv [f_n|y_n]$ % to define a merged feature which has 
with a well-defined $G$ action $g\cdot \phi_n = [g\cdot f_n| g\cdot y_n]$.
% Therefore, in the analysis below we use the combined features $\phi_n$.
% assume the input is a set of $f_n$ and won't distinguish between $f_n$ and $y_n$. 
The collection of combined inputs $\Phi = (\phi_1,\dots, \phi_N)^T$ is an $(m+m_y)\times N$ matrix. 
Using %the combined features $\Phi$, 
equations \ref{eq:L-conv} and  \ref{eq:dfdg-general}, the MSE loss with parameters $W = \{W^0,\ba{\eps}\}$ becomes
% \ry{include a 2d function} 
(SI
\ref{ap:Loss-MSE})
\begin{align}
    I[\Phi;W] &= \int_G dg \L[\Phi;W] = \int_G dg \left\|  W^0 \br{I + \ba{\eps}^i  [\hat{L}_i]^\alpha \ro_\alpha}\Phi(g) \right\|^2 
    \cr
    % &= \int_G dg \br{ 
    % \|W^0\Phi\|^2 + \left\|W^i [\hat{L}_i]^\alpha \ro_\alpha \Phi \right\|^2 +2\Phi^T  W^{0T}W^i [\hat{L}_i]^\alpha \ro_\alpha \Phi}
    % \label{eq:loss-MSE-expand}\\
    % &=\sum_n \int_G dg \br{ M_{ab}\phi_n^a \phi_n^b +\mathbf{h}^{\alpha\beta}_{ab}  \ro_\beta \phi_n^b \ro_\alpha \phi_n^a + [\hat{L}_i]^\alpha \ro_\alpha \pa{\phi_n^T V^i \phi_n}}
    % \label{eq:Loss-MSE-simplified}\\
    &= \int_\mathcal{S} {d^nx\over\left|\ro x\over \ro g\right|} \br{\Phi^T\mathbf{m}_2\Phi + \ro_\alpha \Phi^T \mathbf{h}^{\alpha\beta} \ro_\beta \Phi +[\hat{L}_i]^\alpha \ro_\alpha \pa{\Phi^T \mathbf{v}^i \Phi} }
    \label{eq:Loss-MSE}
    % \mbox{Invariance: } & u\in G: \quad u^T\mathbf{g}_{ab} u = \mathbf{g}_{ab}
 \end{align}
 
% \nd{Discuss stabilizers}
where $\left|\ro x\over \ro g\right|$ is the determinant of the Jacobian, $W^i = W^0 \ba{\eps}^i$ and
\begin{align}
    % \mathbf{m}_2 &=W^{0T}W^0 &
    % \mathbf{h}^{\alpha\beta}(\vx) &= W^{iT}W^j [\hat{L}_i]^\alpha [\hat{L}_i]^\beta &
    % \mathbf{v}^i &= W^{0T}W^i. \\
    \mathbf{m}_2 &=W^{0T}W^0, &
    \mathbf{h}^{\alpha\beta}(\vx) &= \ba{\eps}^{iT} \mathbf{m}_2 \ba{\eps}^j [\hat{L}_i]^\alpha [\hat{L}_j]^\beta, &
    \mathbf{v}^i &= \mathbf{m}_2\ba{\eps}^{i} . 
    \label{eq:MSE-params}
\end{align}
Note that $\mathbf{h}$ has feature space indices via $[\ba{\eps}^{iT} \mathbf{m}_2 \ba{\eps}^j]_{ab}$, with index symmetry
$\mathbf{h}^{\alpha\beta}_{ab}=\mathbf{h}^{\beta\alpha}_{ba} $.
When $\mathcal{F}= \R$ (i.e. $f$ is a 1D scalar), $\mathbf{h}^{\alpha\beta}$ becomes a
a Riemannian metric 
% $\mathbf{h}^{\alpha\beta}$ 
for $\mathcal{S}$.
In general $\mathbf{h}$ combines a 2-tensor $\mathbf{h}_{ab}=\mathbf{h}_{ab}^{\alpha\beta}\ro_\alpha \ro_\beta \in T\mathcal{S} \otimes T\mathcal{S}$ with an inner product $h^T\mathbf{h}^{\alpha\beta}f $ on the feature space $\mathcal{F}$. 
Hence $\mathbf{h}\in T\mathcal{S}\otimes T\mathcal{S}\otimes \mathcal{F}^*\otimes \mathcal{F}^*$ is a $(2,2)$-tensor, with $\mathcal{F}^*$ being the dual space of $\mathcal{F}$.   
% \nd{Is it symmetric?}
% Note that $\mathbf{h}^{\alpha\beta}(\vx)$ is a function of $\vx$ because $\hat{L}_i(\vx)$ depends on $\vx$.
%

A simpler version of the loss function in \eqref{eq:Loss-MSE} is commonly used in field theories in physics \citep{polyakov2018gauge}. 
There too, the motivation is to preserve spatial symmetries for the metric $\mathbf{h}$.
In \eqref{eq:Loss-MSE}, 
$\mathbf{h}$ transforms equivariantly as a 2-tensor $v\cdot \mathbf{h}^{\alpha\beta}=[v^{-1}]^\alpha_\rho [v^{-1}]^\beta_\gamma\mathbf{h}^{\rho\gamma}(\vx)$ for $v\in G$ (SI \ref{ap:invariant-loss}).
In physics the last term in \eqref{eq:Loss-MSE} is absent. 
We can show that for L-conv also when $G$ is translations $T_n$, or rotations $SO(n)$, by partial integration the last term becomes a boundary term and expected to vanish (SI \ref{ap:invariant-loss}).
% For $G=T_n$, the first term in \eqref{eq:Loss-MSE} becomes $\ro_j \phi^T \mathbf{h}^{ji} \ro_i \phi$. 
We discuss the implications of this overlap between physics and equivariant neural networks further below. %in the discussions sec. \ref{sec:discussion}. 
One aspect of the physics theory which may benefit machine learning is that for $\phi_n$ which minimize the loss, the loss function is robust to small perturbations. 
This yields a natural way to probe generalization in equivariant neural networks, discussed next. 

\paragraph{Generalization error}
Equivariant neural networks are expected to be more robust than others, meaning 
equivariance should improve generalization. 
One way to check this is to see how the network would perform for an input $\phi'= \phi + \delta \phi$ which adds a small perturbation $\delta \phi$ to a real data point $\phi$.
Note $\delta \phi $ here s a random noise, not an adversarial attack.
Robustness to such perturbation would mean that, for optimal parameters $W^*$ , the loss function would not change,
i.e. $I [\phi';W^*]=I [\phi;W^*]$. 
This can be cast as a variational equation, requiring $I $ to be minimized around real data points $\phi$. 
Writing $I[\phi;W]= \int d^nx \L[\phi;W]$, we have 
\begin{align}
    % I[\phi;W]&= \int d^nx \L[\phi;W], &
    \delta I [\phi;W^*] &=\int_\mathcal{S} d^nx\br{
    {\ro \L \over \ro \phi^a }\delta \phi^a + {\ro \L \over \ro (\ro_\alpha \phi^a) } \ro_\alpha (\delta \phi^a) 
    }
\end{align}
Doing a partial integration on the second term, we get a vanishing boundary term plus the familiar 
Euler-Lagrange (EL) equation (SI \ref{ap:generalization}), widely used in physics and control theory. 
Thus, requiring good generalization, i.e. $\delta I [\phi;W^*]/\delta \phi=0$ means for optimal parameters $W^*$, real data points $\phi$ satisfy the EL equations
\begin{align}
    \mbox{Generalization Error Minimization} \Longleftrightarrow \mbox{EL: }
    \quad 
    {\ro \L \over \ro \phi^b } - \ro_\alpha {\ro \L \over \ro (\ro_\alpha \phi^b) } = 0 
    \label{eq:loss-Euler-Lagrange}
\end{align}
\out{
Applying this to the MSE loss \eqref{eq:Loss-MSE}, \eqref{eq:loss-Euler-Lagrange} becomes
\begin{align}
    % \mbox{EL:} \quad 
    \mathbf{m}_2 \phi - \ro_\alpha \pa{|J| \mathbf{h}^{\alpha\beta} \ro_\beta \phi } - \ro_\alpha\pa{|\ro_\vx g|\mathbf{v}^i [\hat{L}_i]^\alpha }\phi =0 
    \label{eq:loss-EL-MSE}
\end{align}
where % $|\mathcal{J}| = |\ro g/\ro x|$ 
$|\ro_\vx g|$ is the determinant of the Jacobian.
For the translation group, \eqref{eq:loss-EL-MSE} becomes a Helmholtz equation
\begin{align}
    \ba{\eps}^i\mathbf{m}_2 \ba{\eps}^j \ro_i\ro_j\phi = \mathbf{m}_2 \phi
\end{align}
}%%%%
Another idea which can be transferred from physics to equivariant neural networks is that symmetries produce conserved currents, via Noether's theorem, also discussed in \citet{kunin2020neural}. 
We briefly discuss motivate this below. 

\paragraph{Conservation laws}
The idea is that the equivariance condition \eqref{eq:equivairance-general} can be written for the integrand of the loss $\L[\phi,W]$. 
If we write the equivariance equation for infinitesimal $v_\eps $, we obtain a vector field which is divergence free. 
% For $\delta I [\phi;W^*]/\delta \phi=0$, beside the EL equations, the variations at the boundary should be orthogonal to the normal to the boundary $d^{n-1}\Sigma$. 
Since $G$ is the symmetry of the system, transforming an input $\phi\to w\cdot \phi$ by $w\in G$  the integrand should change equivariantly, meaning $\L[w\cdot \phi]= w\cdot \L[\phi] $. 
% We will now show that 
When generalization error is minimized as in \eqref{eq:loss-Euler-Lagrange}, an infinitesimal $w\approx I+\eta^i L_i$, with $\delta \phi = \eps^i \hat{L}_i \phi$, results in a conserved current (SI \ref{ap:generalization})
% the correct $L_i \in \mathfrak{g}$ appear in $I[\phi;W^*]$.
% Let's see how the Lagrangian $\L$ (integrand of the loss) changes when 
% When the generalization error is minimized (i.e. EL equations are satisfied) the term that produced the vanishing boundary term can
\begin{align}
    \mbox{Noether current: } J^\alpha &= {\ro \L \over \ro (\ro_\alpha \phi^b) } \delta \phi^b - {\ro \L \over \ro \vx^\alpha } \delta \vx^\alpha , & \delta I [\phi;W^*]=0 \quad \Rightarrow \ro_\alpha J^\alpha &= 0
\end{align}
\nd{replace with stress-energy tensor. Discuss why this is narrow and more general symmetries exist.} 
% This is the integrand of the boundary term 
This $J$ is called the Noether current in physics.
It captures the flow of the Lagrangian $\L$ along symmetry direction $\hat{L}_i$.
% and the requirement for the boundary term to vanish is the statement that the Noether current be conserved (i.e. divergence free) or 
% \nd{Becomes Euler-Lagrange equations}
It would be interesting to see if these conserved currents can be used in practice as an alternative way for identifying or discovering symmetries. 
We conclude by remarking on similarity between ML and physics problems. 

\paragraph{Relation to physics} Although \eqref{eq:Loss-MSE} was % is the MSE loss for L-conv, 
derived purely using ML and equivariance,
% But 
physicists will recognize \eqref{eq:Loss-MSE} as a generalization of the non-interacting field theory action (integral of a Lagrangian). 
In field theory, $\phi(x)$ (each input feature $[f|y]$) is called a field.
$\mathbf{m}_2$ is the ``mass matrix'' whose eigenvalues are the squares of masses of the fields.
The second term $\ro\phi^T\cdot \mathbf{h}\cdot\ro\phi = \ro^\mu \phi^a \ro_\mu \phi_a$ is the ``kinetic'' term. 
% Mass matrices appear in the standard model of particle physics in the Higgs interaction  
In physics, the loss in \eqref{eq:Loss-MSE} is used in two ways. 
When the parameters $\mathbf{m}_2$ and $\mathbf{h}$ are known, 
% the features $f(\vx)$ minimizing the loss are not known. 
% In this case, the loss lacks the $\sum_n$ and $I [f]$ is a function of $f$, with $M$ and $\mathbf{g}$ fixed.
% Therefore 
a variational procedure known as the Euler-Lagrange equations is used to find optimal $\phi(\vx)= \argmin_\phi I [\phi]$. 
When $\mathbf{m}_2$ and $\mathbf{h}$ are not known, $\phi_n$ are observational data and physicists use \eqref{eq:Loss-MSE} the same way as ML. %, as an ansatz to estimate $\mathbf{m}_2$ and $\mathbf{h}$. 
In this case \eqref{eq:Loss-MSE} is a variational ansatz used to identify parameters $\mathbf{m}_2$ and $\mathbf{h}$ such that the expected loss for the observed $\phi_n$ is minimized.
The main difference with physics is that % with the ansatz used in physics is that the metrics on $T\mathcal{S}$ and $\mathcal{F}$ are fused into a tensor $\mathbf{h}$. 
physics assumes a simpler form in which 
% the ansatz used is much simpler and 
$\mathbf{h}$ factorizes into a tensor product $\mathbf{h} = \eta \otimes \delta $, where $\eta_{\alpha\beta}$ is a Riemannian metric on $T\mathcal{S}$ and $\delta$, usually the Kronecker delta, is the metric on $\mathcal{F}$. % (internal space or fibers in physics). 
% The other difference is that in field theory the last term in \eqref{eq:Loss-MSE} is usually absent. 
% We now show via examples that this term can be important for conservation laws in ML. 
% \nd{Talk about how L-conv allows us to create more general ansaetze for physics. }
\out{
\textbf{Loss minimization in physics and ML}
In physics, the loss in \eqref{eq:Loss-MSE} is used in two ways. 
When the parameters $\mathbf{m}_2$ and $\mathbf{h}$ are known, 
% the features $f(\vx)$ minimizing the loss are not known. 
% In this case, the loss lacks the $\sum_n$ and $I [f]$ is a function of $f$, with $M$ and $\mathbf{g}$ fixed.
% Therefore 
a variational procedure known as the Euler-Lagrange equations is used to find optimal $\phi(\vx)= \argmin_\phi I [\phi]$. 
When $\mathbf{m}_2$ and $\mathbf{h}$ are not known, $\phi_n$ are observational data and physicists use \eqref{eq:Loss-MSE} the same way as ML. %, as an ansatz to estimate $\mathbf{m}_2$ and $\mathbf{h}$. 
In this case \eqref{eq:Loss-MSE} is a variational ansatz used to identify parameters $\mathbf{m}_2$ and $\mathbf{h}$ such that the expected loss for the observed $\phi_n$ is minimized.
% \nd{Is SGD related to RG and Callan-Symantzik? }

% Next, we will discuss how to implement \eqref{eq:L-conv-tensor0} in practice and how to learn symmetries with L-conv.

% \nd{1) physics; 2) coarse-graining}
}%%%
We conclude with some closing remarks. 

==> secs2/universal.tex <==

\textbf{Todo}
\begin{enumerate}
    \item more intuition 
    \item universal approx
    \item intuition for number of $L_i$
    \item Discretization: Emphasize difference with discretizing group (both have discrete space, but we don't discretize group) 
    \item Comment on good inductive bias and when to use L-conv
    \item real-world potential uses 
    \item concrete discussion of physics and ML uses 
    \item meta-learning paper discussion
    \item LieConv discussion
\end{enumerate}

\textbf{LieConv:}  But as you also mention, the log, product and inverse need to implemented for each group and each representation separately.
 In comparison, our method is similar to GCN. Even when the group is known, we only need to encode $L_i$
 and no group specific functions.
 

\section{Universal Approximation for Group Equivariant Functions}


We say $F$ is \textit{equivariant} under $G$ if $G$ acts on $\mathcal{F}'$ and for $u\in G$
\begin{align}
    u\cdot (F(f)) &= F(u\cdot f).
    \label{eq:equiv-gen-1}
\end{align}

\subsection{Scalar case}
Now we have to define the how the group acts on the features $f(g)$.
We consider the case where the features are ``scalars'' meaning the group action is given by
\begin{align}
    u\cdot f(g)& = f(u^{-1} g)
\end{align}
Similarly, we want the transformed features $F(f)$ to be scalars as well
\begin{align}
    u\cdot F(f)(g)& = F(f)(u^{-1}g)
\end{align}
We want to know what constraint being equivariant puts on the function $F:\mathcal{F}\to \mathcal{F}'$. 
We know that if $F$ is linear, it has to be a group convolution \citep{kondor2018generalization}, with generalizations to the steerable case \citep{cohen2016steerable}.
The proof follows by writing $F(f)=W\cdot f$, where $W$ is a linear operator in the function space.
First, we assume the input of $f:\mathcal{S} \to \mathcal{F}$ is lifted to $G$ so that we have $f(\vx)= f(g\vx_0)$ for $g \in G$. 
Then $F(f):\mathcal{S}\to \mathcal{F}'$
meaning 
\begin{align}
    F(f)(g)&= [W\cdot f](g) = \int_G du W(u,g)f(u) 
\end{align}
The equivariance constraints the form of $W(u,g)$  to $W=\kappa(u^{-1}g)$. 
To see this note
\begin{align}
    v\cdot F(f)(g)&= [v\cdot W\cdot f](g) = \int_G du W(u,v^{-1}g)f(u) \cr 
    = F(v\cdot f)(g)& =  \int_G du W(u,g)f(v^{-1}u) = \int_G du' W(vu',g)f(u')  
\end{align}

which yields 
\begin{align}
    W(u,v^{-1}g)& = W(vu,g) &
    \Rightarrow W(u,g)=\kappa(u^{-1}g).
\end{align}

If we look at the definition of $F(f)$ as a linear function $W\cdot f$, we can try to apply the reasoning behind the universal approximation theorem in neural networks (UAT). 
in UAT, we want to approximate $F(x)$. 
The easiest way to achieve this is by writing $F(x)$ as the sum over a set of localized functions $\delta_\eta(x) \sim \exp[]$ 
\nd{$\delta (f-g)$ the issue is $g$ would be in the function space. It is not clear how it can be }

Can a general equivariant function be approximated with equivariant feedforward G-conv? 
Can we break the function down in terms of its range? 

\subsection{Steerable case}

In the steerable case the action is linear using a representation $\rho_1$  
\begin{align}
    u\cdot f(g)& = \rho(u)f(u^{-1} g)
\end{align}
Similarly, for the transformed features $F(f)$ we can have 
\begin{align}
    u\cdot F(f)(g)& = \rho_2(u)F(f)(u^{-1}g)
\end{align}
Because of equivariance \eqref{eq:equiv-gen-1}, we have
\begin{align}
    u\cdot F(f)(g)& = \rho_2(u)F(f)(u^{-1}g) \cr 
    &= F(u\cdot f)(g) = F(\rho_1(u)f)(u^{-1}g)\cr
    \Rightarrow F(f) &= \rho_2(u^{-1})F(\rho_1(u) f)
\end{align}


We want to know what constraint being equivariant puts on the function $F:\mathcal{F}\to \mathcal{F}'$. 
We know that if $F$ is linear, it has to be a group convolution \citep{kondor2018generalization}, with generalizations to the steerable case \citep{cohen2016steerable}.
The proof follows by writing $F(f)=W\cdot f$, where $W$ is a linear operator in the function space.
First, we assume the input of $f:\mathcal{S} \to \mathcal{F}$ is lifted to $G$ so that we have $f(\vx)= f(g\vx_0)$ for $g \in G$. 
Then $F(f):\mathcal{S}\to \mathcal{F}'$
meaning 
\begin{align}
    F(f)(g)&= [W\cdot f](g) = \int_G du W(u,g)f(u) 
\end{align}
The equivariance constraints the form of $W(u,g)$  to $W=\kappa(u^{-1}g)$. 
To see this note
\begin{align}
    v\cdot F(f)(g)&= [v\cdot W\cdot f](g) = \rho_2 (v) \int_G du W(u,v^{-1}g)f(u) \cr 
    = F(v\cdot f)(g)& =  \int_G du W(u,g)\rho_1 (v)f(v^{-1}u) = \int_G du' W(vu',g)\rho_1 (v)f(u') 
\end{align}
which yields 
\begin{align}
    W(u,v^{-1}g)& =  \rho_2 (v^{-1}) W(vu,g)\rho_1 (v).
\end{align}
On way to satisfy this is the have 
\begin{align}
    W(u,g)& = \rho_2(g) \kappa(g^{-1}u) \rho_1(u^{-1})
\end{align}




\subsection{Steerable case}
% \nd{The parentheses should change to }
\begin{align}
    [u\cdot F(f)](x) &= \rho(u;x) F(u\cdot f)(x),
    % \label{eq:equivairance-general-1}
\end{align}
where $\rho: G\to \mathrm{GL}_{m'}(\R)$ is a representation of the group $G$. 
The more general requirement is to have 
\begin{align}
    [u\cdot F(f)] &= P(u,F)(u\cdot f),\cr
    [v\cdot[u\cdot F(f)]] &= [(vu)\cdot F(f)] \cr 
    \Rightarrow P(vu,F)((vu)\cdot f)&=  P(v,P(u,F))(v\cdot (u\cdot f)) 
    \quad \forall u,v \in G, \ \forall f \in \mathcal{F}\\
    \Rightarrow P(v,P(u,F)) &= P(vu,F), \qquad v\cdot (u\cdot f) = (vu)\cdot f
    % \label{eq:equivairance-general-1}
\end{align}
The first condition on the last line are satisfied if $P(u,F)= \rho(u)F$ for some representation $\rho: G\to \mathrm{GL}_{m'}(\R)$, as 
$P(v,P(u,F)) = \rho(v)\rho(u)F= \rho(vu) F = P(vu,F) $. 
The second condition can also be satisfied if $f$ is also equivariant or alternatively if $u\cdot f= \pi(u)f$ with $\pi: G\to \mathrm{GL}_{m}(\R)$.
Note, we do not claim a linear representation of the group is the unique solution, but rather that it is one way to have equivariance under group action.


% The main assumption for the proof is that the input (i.e., $f$) can be lifted to the group. 





%
\textbf{Group Convolution}
\citet{kondor2018generalization} showed that $F$ is a linear equivariant map if and only if it performs a group convolution (G-conv).
To define G-conv, we first lift $\vx$ to elements in $G$ \citep{kondor2018generalization}.
% This requires that the map $\mathrm{Lift}:\mathcal{S}\to G$ be injective. 
% This puts the condition on $G$ that $\forall \vx,\vy \in \mathcal{S}$, $\exists g\in G$ such that $\vy = g\vx$ (e.g. $G$ can be 2D translation on images). 
% For example, when $\mathcal{S} = \R$, the group of 1D translations (i.e. addition by a real number $G=(\R,+)$) satisfies this condition.
To do the lift, we pick an origin $\vx_0 \in \mathcal{S}$ and replace each point $\vx = g\vx_0$ by $g$. 
% With a slight abuse of notation, 
We will often drop $\vx_0$ for brevity and write
% The feature maps then become 
$f(g)\equiv f(g\vx_0)$. 
% Lift $x\to g\in G$ and let $dv\equiv d\mu(v)$. 
% From \cite{cohen2018intertwiners} Eq (41) 
Let $\kappa: G\to %\mathrm{Hom}( \mathcal{F}', \mathcal{F}) \sim 
\R^{m'} \otimes \R^{m}$ %, meaning $\kappa(g)$ is 
be a linear transformation from $\mathcal{F}$ to $\mathcal{F}'$.
G-conv is defined as 
% As shown in \cite{kondor2018generalization}, the following G-conv is equivariant  
\begin{align}
    [\kappa\star f](g) = \int_G \kappa(g^{-1}v)f(v) dv = \int_G \kappa(v)f(gv) dv,
    \label{eq:G-conv-1}
\end{align}
where for brevity, we are denoting the Haar measure on $G$ as $dv\equiv d\mu(v)$.

\textbf{Equivariance of G-conv}
As shown in \cite{kondor2018generalization}, G-conv is equivariant. 
The equivariance of \eqref{eq:G-conv-1} can be readily checked using \eqref{eq:f-G-action}.
For $w\in G$ we have
\begin{align}
    [\kappa\star w\cdot f](g) 
    &= \int_G \kappa(v)w\cdot f(gv) dv 
    %\cr & 
    = \int_G \kappa(v)f(w^{-1}gv) dv\cr
    & = [\kappa\star f](w^{-1}g)
    = w\cdot [\kappa\star f](g) 
    % = \int \kappa(v)f(gv) dv 
    \label{eq:G-conv-equiv-1}
\end{align}


\section{Formal Statement}


Let $G$ be a compact Lie group.  Let 
\[ X =  \lbrace f \colon G \to \mathbb{R} : \text{{\color{red}some conditions}}  \rbrace.
\]

Consider $K \subset X$ compact with $g K = K$.  {\color{red} Possibly additional restrictions on $K$.}  Let $Q \colon X \to X$ which is $G$-equivariant.  Assume $Q$ {\color{red} satisfies some regularity hypothesis.}  

Let $\mathrm{MLLconv} = \lbrace  \hat{Q} \colon X \to X : \hat{Q} =  L_1 \circ \sigma \circ \ldots \circ L_k, L_i: X^{k_i} \to X^{k_i} \text{ $L$-conv layer}, \  \sigma = \mathtt{ReLU} \rbrace$

For $f \in X$, define
\[
\| f \|_X = \int_{g \in G} |f(g)| dg.
\]

\begin{theorem}
Let $\epsilon > 0$.  There exists a $\hat{Q} \in \mathrm{MLLconv}$ such that 
\[
\mathrm{sup}_{f \in K} \| \hat{Q}(f) - Q(f) \|_X < \epsilon.
\]
\end{theorem}



